Determination of jet calibration and energy resolution in proton-proton collisions at $\sqrt{s}$ = 8 TeV using the ATLAS detector

The jet energy scale, jet energy resolution, and their systematic uncertainties are measured for jets reconstructed with the ATLAS detector in 2012 using proton-proton data produced at a centre-of-mass energy of 8 TeV with an integrated luminosity of 20 fb$^{-1}$. Jets are reconstructed from clusters of energy depositions in the ATLAS calorimeters using the anti-$k_t$ algorithm. A jet calibration scheme is applied in multiple steps, each addressing specific effects including mitigation of contributions from additional proton-proton collisions, loss of energy in dead material, calorimeter non-compensation, angular biases and other global jet effects. The final calibration step uses several \textit{in situ} techniques and corrects for residual effects not captured by the initial calibration. These analyses measure both the jet energy scale and resolution by exploiting the transverse momentum balance in $\gamma$+jet, $Z$+jet, dijet, and multijet events. A statistical combination of these measurements is performed. In the central detector region, the derived calibration has a precision better than 1% for jets with transverse momentum 150 GeV $< p_{\mathrm{T}}<$ 1500 GeV, and the relative energy resolution is $(8.4\pm 0.6)$% for $p_{\mathrm{T}}=$ 100 GeV and $(23\pm 2)$% for $p_{\mathrm{T}}=$ 20 GeV. The calibration scheme for jets with radius parameter $R=1.0$, for which jets receive a dedicated calibration of the jet mass, is also discussed.

==> flattened/atlas_authlist.tex <==
% ATLAS Collaboration author list
% Reference date of PERF-2014-02 is 2017-12-18
% Author list last updated on date 08-OCT-19
% Data extracted on 28-Feb-2020 for paper reference PERF-2014-02
% at 5:28pm
 
\begin{flushleft}
{\Large The ATLAS Collaboration}

\bigskip

M.~Aaboud$^\textrm{\scriptsize 35d}$,    
G.~Aad$^\textrm{\scriptsize 101}$,    
B.~Abbott$^\textrm{\scriptsize 128}$,    
O.~Abdinov$^\textrm{\scriptsize 13,*}$,    
B.~Abeloos$^\textrm{\scriptsize 64}$,    
S.H.~Abidi$^\textrm{\scriptsize 167}$,    
O.S.~AbouZeid$^\textrm{\scriptsize 145}$,    
N.L.~Abraham$^\textrm{\scriptsize 155}$,    
H.~Abramowicz$^\textrm{\scriptsize 161}$,    
H.~Abreu$^\textrm{\scriptsize 160}$,    
Y.~Abulaiti$^\textrm{\scriptsize 6}$,    
B.S.~Acharya$^\textrm{\scriptsize 66a,66b,p}$,    
S.~Adachi$^\textrm{\scriptsize 163}$,    
C.~Adam~Bourdarios$^\textrm{\scriptsize 64}$,    
L.~Adamczyk$^\textrm{\scriptsize 83a}$,    
J.~Adelman$^\textrm{\scriptsize 120}$,    
M.~Adersberger$^\textrm{\scriptsize 113}$,    
T.~Adye$^\textrm{\scriptsize 143}$,    
A.A.~Affolder$^\textrm{\scriptsize 145}$,    
Y.~Afik$^\textrm{\scriptsize 160}$,    
C.~Agheorghiesei$^\textrm{\scriptsize 27c}$,    
J.A.~Aguilar-Saavedra$^\textrm{\scriptsize 139f,139a}$,    
F.~Ahmadov$^\textrm{\scriptsize 79,ai}$,    
G.~Aielli$^\textrm{\scriptsize 73a,73b}$,    
S.~Akatsuka$^\textrm{\scriptsize 85}$,    
T.P.A.~{\AA}kesson$^\textrm{\scriptsize 96}$,    
E.~Akilli$^\textrm{\scriptsize 53}$,    
A.V.~Akimov$^\textrm{\scriptsize 110}$,    
G.L.~Alberghi$^\textrm{\scriptsize 23b,23a}$,    
J.~Albert$^\textrm{\scriptsize 176}$,    
P.~Albicocco$^\textrm{\scriptsize 50}$,    
M.J.~Alconada~Verzini$^\textrm{\scriptsize 88}$,    
S.~Alderweireldt$^\textrm{\scriptsize 118}$,    
M.~Aleksa$^\textrm{\scriptsize 36}$,    
I.N.~Aleksandrov$^\textrm{\scriptsize 79}$,    
C.~Alexa$^\textrm{\scriptsize 27b}$,    
G.~Alexander$^\textrm{\scriptsize 161}$,    
T.~Alexopoulos$^\textrm{\scriptsize 10}$,    
M.~Alhroob$^\textrm{\scriptsize 128}$,    
B.~Ali$^\textrm{\scriptsize 141}$,    
G.~Alimonti$^\textrm{\scriptsize 68a}$,    
J.~Alison$^\textrm{\scriptsize 37}$,    
S.P.~Alkire$^\textrm{\scriptsize 147}$,    
C.~Allaire$^\textrm{\scriptsize 64}$,    
B.M.M.~Allbrooke$^\textrm{\scriptsize 155}$,    
B.W.~Allen$^\textrm{\scriptsize 131}$,    
P.P.~Allport$^\textrm{\scriptsize 21}$,    
A.~Aloisio$^\textrm{\scriptsize 69a,69b}$,    
A.~Alonso$^\textrm{\scriptsize 40}$,    
F.~Alonso$^\textrm{\scriptsize 88}$,    
C.~Alpigiani$^\textrm{\scriptsize 147}$,    
A.A.~Alshehri$^\textrm{\scriptsize 56}$,    
M.I.~Alstaty$^\textrm{\scriptsize 101}$,    
B.~Alvarez~Gonzalez$^\textrm{\scriptsize 36}$,    
D.~\'{A}lvarez~Piqueras$^\textrm{\scriptsize 174}$,    
M.G.~Alviggi$^\textrm{\scriptsize 69a,69b}$,    
B.T.~Amadio$^\textrm{\scriptsize 18}$,    
Y.~Amaral~Coutinho$^\textrm{\scriptsize 80b}$,    
L.~Ambroz$^\textrm{\scriptsize 134}$,    
C.~Amelung$^\textrm{\scriptsize 26}$,    
D.~Amidei$^\textrm{\scriptsize 105}$,    
S.P.~Amor~Dos~Santos$^\textrm{\scriptsize 139a,139c}$,    
S.~Amoroso$^\textrm{\scriptsize 36}$,    
C.S.~Amrouche$^\textrm{\scriptsize 53}$,    
C.~Anastopoulos$^\textrm{\scriptsize 148}$,    
L.S.~Ancu$^\textrm{\scriptsize 53}$,    
N.~Andari$^\textrm{\scriptsize 21}$,    
T.~Andeen$^\textrm{\scriptsize 11}$,    
C.F.~Anders$^\textrm{\scriptsize 60b}$,    
J.K.~Anders$^\textrm{\scriptsize 20}$,    
K.J.~Anderson$^\textrm{\scriptsize 37}$,    
A.~Andreazza$^\textrm{\scriptsize 68a,68b}$,    
V.~Andrei$^\textrm{\scriptsize 60a}$,    
S.~Angelidakis$^\textrm{\scriptsize 38}$,    
I.~Angelozzi$^\textrm{\scriptsize 119}$,    
A.~Angerami$^\textrm{\scriptsize 39}$,    
A.V.~Anisenkov$^\textrm{\scriptsize 121b,121a}$,    
A.~Annovi$^\textrm{\scriptsize 71a}$,    
C.~Antel$^\textrm{\scriptsize 60a}$,    
M.T.~Anthony$^\textrm{\scriptsize 148}$,    
M.~Antonelli$^\textrm{\scriptsize 50}$,    
D.J.A.~Antrim$^\textrm{\scriptsize 171}$,    
F.~Anulli$^\textrm{\scriptsize 72a}$,    
M.~Aoki$^\textrm{\scriptsize 81}$,    
L.~Aperio~Bella$^\textrm{\scriptsize 36}$,    
G.~Arabidze$^\textrm{\scriptsize 106}$,    
Y.~Arai$^\textrm{\scriptsize 81}$,    
J.P.~Araque$^\textrm{\scriptsize 139a}$,    
V.~Araujo~Ferraz$^\textrm{\scriptsize 80b}$,    
R.~Araujo~Pereira$^\textrm{\scriptsize 80b}$,    
A.T.H.~Arce$^\textrm{\scriptsize 48}$,    
R.E.~Ardell$^\textrm{\scriptsize 93}$,    
F.A.~Arduh$^\textrm{\scriptsize 88}$,    
J-F.~Arguin$^\textrm{\scriptsize 109}$,    
S.~Argyropoulos$^\textrm{\scriptsize 77}$,    
A.J.~Armbruster$^\textrm{\scriptsize 36}$,    
L.J.~Armitage$^\textrm{\scriptsize 92}$,    
O.~Arnaez$^\textrm{\scriptsize 167}$,    
H.~Arnold$^\textrm{\scriptsize 119}$,    
M.~Arratia$^\textrm{\scriptsize 32}$,    
O.~Arslan$^\textrm{\scriptsize 24}$,    
A.~Artamonov$^\textrm{\scriptsize 123,*}$,    
G.~Artoni$^\textrm{\scriptsize 134}$,    
S.~Artz$^\textrm{\scriptsize 99}$,    
S.~Asai$^\textrm{\scriptsize 163}$,    
N.~Asbah$^\textrm{\scriptsize 45}$,    
A.~Ashkenazi$^\textrm{\scriptsize 161}$,    
E.M.~Asimakopoulou$^\textrm{\scriptsize 172}$,    
L.~Asquith$^\textrm{\scriptsize 155}$,    
K.~Assamagan$^\textrm{\scriptsize 29}$,    
R.~Astalos$^\textrm{\scriptsize 28a}$,    
R.J.~Atkin$^\textrm{\scriptsize 33a}$,    
M.~Atkinson$^\textrm{\scriptsize 173}$,    
N.B.~Atlay$^\textrm{\scriptsize 150}$,    
K.~Augsten$^\textrm{\scriptsize 141}$,    
G.~Avolio$^\textrm{\scriptsize 36}$,    
R.~Avramidou$^\textrm{\scriptsize 59a}$,    
B.~Axen$^\textrm{\scriptsize 18}$,    
M.K.~Ayoub$^\textrm{\scriptsize 15a}$,    
G.~Azuelos$^\textrm{\scriptsize 109,ax}$,    
A.E.~Baas$^\textrm{\scriptsize 60a}$,    
M.J.~Baca$^\textrm{\scriptsize 21}$,    
H.~Bachacou$^\textrm{\scriptsize 144}$,    
K.~Bachas$^\textrm{\scriptsize 67a,67b}$,    
M.~Backes$^\textrm{\scriptsize 134}$,    
P.~Bagnaia$^\textrm{\scriptsize 72a,72b}$,    
M.~Bahmani$^\textrm{\scriptsize 84}$,    
H.~Bahrasemani$^\textrm{\scriptsize 151}$,    
A.J.~Bailey$^\textrm{\scriptsize 174}$,    
J.T.~Baines$^\textrm{\scriptsize 143}$,    
M.~Bajic$^\textrm{\scriptsize 40}$,    
O.K.~Baker$^\textrm{\scriptsize 183}$,    
P.J.~Bakker$^\textrm{\scriptsize 119}$,    
D.~Bakshi~Gupta$^\textrm{\scriptsize 95}$,    
E.M.~Baldin$^\textrm{\scriptsize 121b,121a}$,    
P.~Balek$^\textrm{\scriptsize 180}$,    
F.~Balli$^\textrm{\scriptsize 144}$,    
W.K.~Balunas$^\textrm{\scriptsize 136}$,    
E.~Banas$^\textrm{\scriptsize 84}$,    
A.~Bandyopadhyay$^\textrm{\scriptsize 24}$,    
Sw.~Banerjee$^\textrm{\scriptsize 181,j}$,    
A.A.E.~Bannoura$^\textrm{\scriptsize 182}$,    
L.~Barak$^\textrm{\scriptsize 161}$,    
W.M.~Barbe$^\textrm{\scriptsize 38}$,    
E.L.~Barberio$^\textrm{\scriptsize 104}$,    
D.~Barberis$^\textrm{\scriptsize 54b,54a}$,    
M.~Barbero$^\textrm{\scriptsize 101}$,    
T.~Barillari$^\textrm{\scriptsize 114}$,    
M-S.~Barisits$^\textrm{\scriptsize 36}$,    
J.~Barkeloo$^\textrm{\scriptsize 131}$,    
T.~Barklow$^\textrm{\scriptsize 152}$,    
N.~Barlow$^\textrm{\scriptsize 32}$,    
R.~Barnea$^\textrm{\scriptsize 160}$,    
S.L.~Barnes$^\textrm{\scriptsize 59c}$,    
B.M.~Barnett$^\textrm{\scriptsize 143}$,    
R.M.~Barnett$^\textrm{\scriptsize 18}$,    
Z.~Barnovska-Blenessy$^\textrm{\scriptsize 59a}$,    
A.~Baroncelli$^\textrm{\scriptsize 74a}$,    
G.~Barone$^\textrm{\scriptsize 26}$,    
A.J.~Barr$^\textrm{\scriptsize 134}$,    
L.~Barranco~Navarro$^\textrm{\scriptsize 174}$,    
F.~Barreiro$^\textrm{\scriptsize 98}$,    
J.~Barreiro~Guimar\~{a}es~da~Costa$^\textrm{\scriptsize 15a}$,    
R.~Bartoldus$^\textrm{\scriptsize 152}$,    
A.E.~Barton$^\textrm{\scriptsize 89}$,    
P.~Bartos$^\textrm{\scriptsize 28a}$,    
A.~Basalaev$^\textrm{\scriptsize 137}$,    
A.~Bassalat$^\textrm{\scriptsize 64,ar}$,    
R.L.~Bates$^\textrm{\scriptsize 56}$,    
S.J.~Batista$^\textrm{\scriptsize 167}$,    
S.~Batlamous$^\textrm{\scriptsize 35e}$,    
J.R.~Batley$^\textrm{\scriptsize 32}$,    
M.~Battaglia$^\textrm{\scriptsize 145}$,    
M.~Bauce$^\textrm{\scriptsize 72a,72b}$,    
F.~Bauer$^\textrm{\scriptsize 144}$,    
K.T.~Bauer$^\textrm{\scriptsize 171}$,    
H.S.~Bawa$^\textrm{\scriptsize 31,n}$,    
J.B.~Beacham$^\textrm{\scriptsize 126}$,    
M.D.~Beattie$^\textrm{\scriptsize 89}$,    
T.~Beau$^\textrm{\scriptsize 135}$,    
P.H.~Beauchemin$^\textrm{\scriptsize 170}$,    
P.~Bechtle$^\textrm{\scriptsize 24}$,    
H.C.~Beck$^\textrm{\scriptsize 52}$,    
H.P.~Beck$^\textrm{\scriptsize 20,s}$,    
K.~Becker$^\textrm{\scriptsize 51}$,    
M.~Becker$^\textrm{\scriptsize 99}$,    
C.~Becot$^\textrm{\scriptsize 124}$,    
A.~Beddall$^\textrm{\scriptsize 12d}$,    
A.J.~Beddall$^\textrm{\scriptsize 12a}$,    
V.A.~Bednyakov$^\textrm{\scriptsize 79}$,    
M.~Bedognetti$^\textrm{\scriptsize 119}$,    
C.P.~Bee$^\textrm{\scriptsize 154}$,    
T.A.~Beermann$^\textrm{\scriptsize 36}$,    
M.~Begalli$^\textrm{\scriptsize 80b}$,    
M.~Begel$^\textrm{\scriptsize 29}$,    
A.~Behera$^\textrm{\scriptsize 154}$,    
J.K.~Behr$^\textrm{\scriptsize 45}$,    
A.S.~Bell$^\textrm{\scriptsize 94}$,    
G.~Bella$^\textrm{\scriptsize 161}$,    
L.~Bellagamba$^\textrm{\scriptsize 23b}$,    
A.~Bellerive$^\textrm{\scriptsize 34}$,    
M.~Bellomo$^\textrm{\scriptsize 160}$,    
K.~Belotskiy$^\textrm{\scriptsize 111}$,    
N.L.~Belyaev$^\textrm{\scriptsize 111}$,    
O.~Benary$^\textrm{\scriptsize 161,*}$,    
D.~Benchekroun$^\textrm{\scriptsize 35a}$,    
M.~Bender$^\textrm{\scriptsize 113}$,    
N.~Benekos$^\textrm{\scriptsize 10}$,    
Y.~Benhammou$^\textrm{\scriptsize 161}$,    
E.~Benhar~Noccioli$^\textrm{\scriptsize 183}$,    
J.~Benitez$^\textrm{\scriptsize 77}$,    
D.P.~Benjamin$^\textrm{\scriptsize 48}$,    
M.~Benoit$^\textrm{\scriptsize 53}$,    
J.R.~Bensinger$^\textrm{\scriptsize 26}$,    
S.~Bentvelsen$^\textrm{\scriptsize 119}$,    
L.~Beresford$^\textrm{\scriptsize 134}$,    
M.~Beretta$^\textrm{\scriptsize 50}$,    
D.~Berge$^\textrm{\scriptsize 45}$,    
E.~Bergeaas~Kuutmann$^\textrm{\scriptsize 172}$,    
N.~Berger$^\textrm{\scriptsize 5}$,    
L.J.~Bergsten$^\textrm{\scriptsize 26}$,    
J.~Beringer$^\textrm{\scriptsize 18}$,    
S.~Berlendis$^\textrm{\scriptsize 57}$,    
N.R.~Bernard$^\textrm{\scriptsize 102}$,    
G.~Bernardi$^\textrm{\scriptsize 135}$,    
C.~Bernius$^\textrm{\scriptsize 152}$,    
F.U.~Bernlochner$^\textrm{\scriptsize 24}$,    
T.~Berry$^\textrm{\scriptsize 93}$,    
P.~Berta$^\textrm{\scriptsize 99}$,    
C.~Bertella$^\textrm{\scriptsize 15a}$,    
G.~Bertoli$^\textrm{\scriptsize 44a,44b}$,    
I.A.~Bertram$^\textrm{\scriptsize 89}$,    
C.~Bertsche$^\textrm{\scriptsize 45}$,    
G.J.~Besjes$^\textrm{\scriptsize 40}$,    
O.~Bessidskaia~Bylund$^\textrm{\scriptsize 44a,44b}$,    
M.~Bessner$^\textrm{\scriptsize 45}$,    
N.~Besson$^\textrm{\scriptsize 144}$,    
A.~Bethani$^\textrm{\scriptsize 100}$,    
S.~Bethke$^\textrm{\scriptsize 114}$,    
A.~Betti$^\textrm{\scriptsize 24}$,    
A.J.~Bevan$^\textrm{\scriptsize 92}$,    
J.~Beyer$^\textrm{\scriptsize 114}$,    
R.M.~Bianchi$^\textrm{\scriptsize 138}$,    
O.~Biebel$^\textrm{\scriptsize 113}$,    
D.~Biedermann$^\textrm{\scriptsize 19}$,    
R.~Bielski$^\textrm{\scriptsize 100}$,    
K.~Bierwagen$^\textrm{\scriptsize 99}$,    
N.V.~Biesuz$^\textrm{\scriptsize 71a,71b}$,    
M.~Biglietti$^\textrm{\scriptsize 74a}$,    
T.R.V.~Billoud$^\textrm{\scriptsize 109}$,    
M.~Bindi$^\textrm{\scriptsize 52}$,    
A.~Bingul$^\textrm{\scriptsize 12d}$,    
C.~Bini$^\textrm{\scriptsize 72a,72b}$,    
S.~Biondi$^\textrm{\scriptsize 23b,23a}$,    
T.~Bisanz$^\textrm{\scriptsize 52}$,    
C.~Bittrich$^\textrm{\scriptsize 47}$,    
D.M.~Bjergaard$^\textrm{\scriptsize 48}$,    
J.E.~Black$^\textrm{\scriptsize 152}$,    
K.M.~Black$^\textrm{\scriptsize 25}$,    
R.E.~Blair$^\textrm{\scriptsize 6}$,    
T.~Blazek$^\textrm{\scriptsize 28a}$,    
I.~Bloch$^\textrm{\scriptsize 45}$,    
C.~Blocker$^\textrm{\scriptsize 26}$,    
A.~Blue$^\textrm{\scriptsize 56}$,    
U.~Blumenschein$^\textrm{\scriptsize 92}$,    
S.~Blunier$^\textrm{\scriptsize 146a}$,    
G.J.~Bobbink$^\textrm{\scriptsize 119}$,    
V.S.~Bobrovnikov$^\textrm{\scriptsize 121b,121a}$,    
S.S.~Bocchetta$^\textrm{\scriptsize 96}$,    
A.~Bocci$^\textrm{\scriptsize 48}$,    
C.~Bock$^\textrm{\scriptsize 113}$,    
D.~Boerner$^\textrm{\scriptsize 182}$,    
D.~Bogavac$^\textrm{\scriptsize 113}$,    
A.G.~Bogdanchikov$^\textrm{\scriptsize 121b,121a}$,    
C.~Bohm$^\textrm{\scriptsize 44a}$,    
V.~Boisvert$^\textrm{\scriptsize 93}$,    
P.~Bokan$^\textrm{\scriptsize 172,52}$,    
T.~Bold$^\textrm{\scriptsize 83a}$,    
A.S.~Boldyrev$^\textrm{\scriptsize 112}$,    
A.E.~Bolz$^\textrm{\scriptsize 60b}$,    
M.~Bomben$^\textrm{\scriptsize 135}$,    
M.~Bona$^\textrm{\scriptsize 92}$,    
J.S.~Bonilla$^\textrm{\scriptsize 131}$,    
M.~Boonekamp$^\textrm{\scriptsize 144}$,    
A.~Borisov$^\textrm{\scriptsize 122}$,    
G.~Borissov$^\textrm{\scriptsize 89}$,    
J.~Bortfeldt$^\textrm{\scriptsize 36}$,    
D.~Bortoletto$^\textrm{\scriptsize 134}$,    
V.~Bortolotto$^\textrm{\scriptsize 73a,62b,62c,73b}$,    
D.~Boscherini$^\textrm{\scriptsize 23b}$,    
M.~Bosman$^\textrm{\scriptsize 14}$,    
J.D.~Bossio~Sola$^\textrm{\scriptsize 30}$,    
J.~Boudreau$^\textrm{\scriptsize 138}$,    
E.V.~Bouhova-Thacker$^\textrm{\scriptsize 89}$,    
D.~Boumediene$^\textrm{\scriptsize 38}$,    
S.K.~Boutle$^\textrm{\scriptsize 56}$,    
A.~Boveia$^\textrm{\scriptsize 126}$,    
J.~Boyd$^\textrm{\scriptsize 36}$,    
I.R.~Boyko$^\textrm{\scriptsize 79}$,    
A.J.~Bozson$^\textrm{\scriptsize 93}$,    
J.~Bracinik$^\textrm{\scriptsize 21}$,    
N.~Brahimi$^\textrm{\scriptsize 101}$,    
A.~Brandt$^\textrm{\scriptsize 8}$,    
G.~Brandt$^\textrm{\scriptsize 182}$,    
O.~Brandt$^\textrm{\scriptsize 60a}$,    
F.~Braren$^\textrm{\scriptsize 45}$,    
U.~Bratzler$^\textrm{\scriptsize 164}$,    
B.~Brau$^\textrm{\scriptsize 102}$,    
J.E.~Brau$^\textrm{\scriptsize 131}$,    
W.D.~Breaden~Madden$^\textrm{\scriptsize 56}$,    
K.~Brendlinger$^\textrm{\scriptsize 45}$,    
A.J.~Brennan$^\textrm{\scriptsize 104}$,    
L.~Brenner$^\textrm{\scriptsize 45}$,    
R.~Brenner$^\textrm{\scriptsize 172}$,    
S.~Bressler$^\textrm{\scriptsize 180}$,    
B.~Brickwedde$^\textrm{\scriptsize 99}$,    
D.L.~Briglin$^\textrm{\scriptsize 21}$,    
T.M.~Bristow$^\textrm{\scriptsize 49}$,    
D.~Britton$^\textrm{\scriptsize 56}$,    
D.~Britzger$^\textrm{\scriptsize 60b}$,    
I.~Brock$^\textrm{\scriptsize 24}$,    
R.~Brock$^\textrm{\scriptsize 106}$,    
G.~Brooijmans$^\textrm{\scriptsize 39}$,    
T.~Brooks$^\textrm{\scriptsize 93}$,    
W.K.~Brooks$^\textrm{\scriptsize 146c}$,    
E.~Brost$^\textrm{\scriptsize 120}$,    
J.H~Broughton$^\textrm{\scriptsize 21}$,    
P.A.~Bruckman~de~Renstrom$^\textrm{\scriptsize 84}$,    
D.~Bruncko$^\textrm{\scriptsize 28b}$,    
A.~Bruni$^\textrm{\scriptsize 23b}$,    
G.~Bruni$^\textrm{\scriptsize 23b}$,    
L.S.~Bruni$^\textrm{\scriptsize 119}$,    
S.~Bruno$^\textrm{\scriptsize 73a,73b}$,    
B.H.~Brunt$^\textrm{\scriptsize 32}$,    
M.~Bruschi$^\textrm{\scriptsize 23b}$,    
N.~Bruscino$^\textrm{\scriptsize 138}$,    
P.~Bryant$^\textrm{\scriptsize 37}$,    
L.~Bryngemark$^\textrm{\scriptsize 45}$,    
T.~Buanes$^\textrm{\scriptsize 17}$,    
Q.~Buat$^\textrm{\scriptsize 36}$,    
P.~Buchholz$^\textrm{\scriptsize 150}$,    
A.G.~Buckley$^\textrm{\scriptsize 56}$,    
I.A.~Budagov$^\textrm{\scriptsize 79}$,    
M.K.~Bugge$^\textrm{\scriptsize 133}$,    
F.~B\"uhrer$^\textrm{\scriptsize 51}$,    
O.~Bulekov$^\textrm{\scriptsize 111}$,    
D.~Bullock$^\textrm{\scriptsize 8}$,    
T.J.~Burch$^\textrm{\scriptsize 120}$,    
S.~Burdin$^\textrm{\scriptsize 90}$,    
C.D.~Burgard$^\textrm{\scriptsize 119}$,    
A.M.~Burger$^\textrm{\scriptsize 5}$,    
B.~Burghgrave$^\textrm{\scriptsize 120}$,    
S.~Burke$^\textrm{\scriptsize 143}$,    
I.~Burmeister$^\textrm{\scriptsize 46}$,    
J.T.P.~Burr$^\textrm{\scriptsize 134}$,    
D.~B\"uscher$^\textrm{\scriptsize 51}$,    
V.~B\"uscher$^\textrm{\scriptsize 99}$,    
E.~Buschmann$^\textrm{\scriptsize 52}$,    
P.J.~Bussey$^\textrm{\scriptsize 56}$,    
J.M.~Butler$^\textrm{\scriptsize 25}$,    
C.M.~Buttar$^\textrm{\scriptsize 56}$,    
J.M.~Butterworth$^\textrm{\scriptsize 94}$,    
P.~Butti$^\textrm{\scriptsize 36}$,    
W.~Buttinger$^\textrm{\scriptsize 36}$,    
A.~Buzatu$^\textrm{\scriptsize 157}$,    
A.R.~Buzykaev$^\textrm{\scriptsize 121b,121a}$,    
G.~Cabras$^\textrm{\scriptsize 23b,23a}$,    
S.~Cabrera~Urb\'an$^\textrm{\scriptsize 174}$,    
D.~Caforio$^\textrm{\scriptsize 141}$,    
H.~Cai$^\textrm{\scriptsize 173}$,    
V.M.M.~Cairo$^\textrm{\scriptsize 2}$,    
O.~Cakir$^\textrm{\scriptsize 4a}$,    
N.~Calace$^\textrm{\scriptsize 53}$,    
P.~Calafiura$^\textrm{\scriptsize 18}$,    
A.~Calandri$^\textrm{\scriptsize 101}$,    
G.~Calderini$^\textrm{\scriptsize 135}$,    
P.~Calfayan$^\textrm{\scriptsize 65}$,    
G.~Callea$^\textrm{\scriptsize 41b,41a}$,    
L.P.~Caloba$^\textrm{\scriptsize 80b}$,    
S.~Calvente~Lopez$^\textrm{\scriptsize 98}$,    
D.~Calvet$^\textrm{\scriptsize 38}$,    
S.~Calvet$^\textrm{\scriptsize 38}$,    
T.P.~Calvet$^\textrm{\scriptsize 154}$,    
M.~Calvetti$^\textrm{\scriptsize 71a,71b}$,    
R.~Camacho~Toro$^\textrm{\scriptsize 37}$,    
S.~Camarda$^\textrm{\scriptsize 36}$,    
P.~Camarri$^\textrm{\scriptsize 73a,73b}$,    
D.~Cameron$^\textrm{\scriptsize 133}$,    
R.~Caminal~Armadans$^\textrm{\scriptsize 102}$,    
C.~Camincher$^\textrm{\scriptsize 57}$,    
S.~Campana$^\textrm{\scriptsize 36}$,    
M.~Campanelli$^\textrm{\scriptsize 94}$,    
A.~Camplani$^\textrm{\scriptsize 68a,68b}$,    
A.~Campoverde$^\textrm{\scriptsize 150}$,    
V.~Canale$^\textrm{\scriptsize 69a,69b}$,    
M.~Cano~Bret$^\textrm{\scriptsize 59c}$,    
J.~Cantero$^\textrm{\scriptsize 129}$,    
T.~Cao$^\textrm{\scriptsize 161}$,    
Y.~Cao$^\textrm{\scriptsize 173}$,    
M.D.M.~Capeans~Garrido$^\textrm{\scriptsize 36}$,    
I.~Caprini$^\textrm{\scriptsize 27b}$,    
M.~Caprini$^\textrm{\scriptsize 27b}$,    
M.~Capua$^\textrm{\scriptsize 41b,41a}$,    
R.M.~Carbone$^\textrm{\scriptsize 39}$,    
R.~Cardarelli$^\textrm{\scriptsize 73a}$,    
F.~Cardillo$^\textrm{\scriptsize 51}$,    
I.~Carli$^\textrm{\scriptsize 142}$,    
T.~Carli$^\textrm{\scriptsize 36}$,    
G.~Carlino$^\textrm{\scriptsize 69a}$,    
B.T.~Carlson$^\textrm{\scriptsize 138}$,    
L.~Carminati$^\textrm{\scriptsize 68a,68b}$,    
R.M.D.~Carney$^\textrm{\scriptsize 44a,44b}$,    
S.~Caron$^\textrm{\scriptsize 118}$,    
E.~Carquin$^\textrm{\scriptsize 146c}$,    
S.~Carr\'a$^\textrm{\scriptsize 68a,68b}$,    
G.D.~Carrillo-Montoya$^\textrm{\scriptsize 36}$,    
D.~Casadei$^\textrm{\scriptsize 33c}$,    
M.P.~Casado$^\textrm{\scriptsize 14,f}$,    
A.F.~Casha$^\textrm{\scriptsize 167}$,    
M.~Casolino$^\textrm{\scriptsize 14}$,    
D.W.~Casper$^\textrm{\scriptsize 171}$,    
R.~Castelijn$^\textrm{\scriptsize 119}$,    
V.~Castillo~Gimenez$^\textrm{\scriptsize 174}$,    
N.F.~Castro$^\textrm{\scriptsize 139a,139e}$,    
A.~Catinaccio$^\textrm{\scriptsize 36}$,    
J.R.~Catmore$^\textrm{\scriptsize 133}$,    
A.~Cattai$^\textrm{\scriptsize 36}$,    
J.~Caudron$^\textrm{\scriptsize 24}$,    
V.~Cavaliere$^\textrm{\scriptsize 29}$,    
E.~Cavallaro$^\textrm{\scriptsize 14}$,    
D.~Cavalli$^\textrm{\scriptsize 68a}$,    
M.~Cavalli-Sforza$^\textrm{\scriptsize 14}$,    
V.~Cavasinni$^\textrm{\scriptsize 71a,71b}$,    
E.~Celebi$^\textrm{\scriptsize 12b}$,    
F.~Ceradini$^\textrm{\scriptsize 74a,74b}$,    
L.~Cerda~Alberich$^\textrm{\scriptsize 174}$,    
A.S.~Cerqueira$^\textrm{\scriptsize 80a}$,    
A.~Cerri$^\textrm{\scriptsize 155}$,    
L.~Cerrito$^\textrm{\scriptsize 73a,73b}$,    
F.~Cerutti$^\textrm{\scriptsize 18}$,    
A.~Cervelli$^\textrm{\scriptsize 23b,23a}$,    
S.A.~Cetin$^\textrm{\scriptsize 12b}$,    
A.~Chafaq$^\textrm{\scriptsize 35a}$,    
D.~Chakraborty$^\textrm{\scriptsize 120}$,    
S.K.~Chan$^\textrm{\scriptsize 58}$,    
W.S.~Chan$^\textrm{\scriptsize 119}$,    
Y.L.~Chan$^\textrm{\scriptsize 62a}$,    
P.~Chang$^\textrm{\scriptsize 173}$,    
J.D.~Chapman$^\textrm{\scriptsize 32}$,    
D.G.~Charlton$^\textrm{\scriptsize 21}$,    
C.C.~Chau$^\textrm{\scriptsize 34}$,    
C.A.~Chavez~Barajas$^\textrm{\scriptsize 155}$,    
S.~Che$^\textrm{\scriptsize 126}$,    
A.~Chegwidden$^\textrm{\scriptsize 106}$,    
S.~Chekanov$^\textrm{\scriptsize 6}$,    
S.V.~Chekulaev$^\textrm{\scriptsize 168a}$,    
G.A.~Chelkov$^\textrm{\scriptsize 79,aw}$,    
M.A.~Chelstowska$^\textrm{\scriptsize 36}$,    
C.~Chen$^\textrm{\scriptsize 59a}$,    
C.H.~Chen$^\textrm{\scriptsize 78}$,    
H.~Chen$^\textrm{\scriptsize 29}$,    
J.~Chen$^\textrm{\scriptsize 59a}$,    
J.~Chen$^\textrm{\scriptsize 39}$,    
S.~Chen$^\textrm{\scriptsize 136}$,    
S.J.~Chen$^\textrm{\scriptsize 15c}$,    
X.~Chen$^\textrm{\scriptsize 15b,av}$,    
Y.~Chen$^\textrm{\scriptsize 82}$,    
Y-H.~Chen$^\textrm{\scriptsize 45}$,    
H.C.~Cheng$^\textrm{\scriptsize 105}$,    
H.J.~Cheng$^\textrm{\scriptsize 15a}$,    
A.~Cheplakov$^\textrm{\scriptsize 79}$,    
E.~Cheremushkina$^\textrm{\scriptsize 122}$,    
R.~Cherkaoui~El~Moursli$^\textrm{\scriptsize 35e}$,    
E.~Cheu$^\textrm{\scriptsize 7}$,    
K.~Cheung$^\textrm{\scriptsize 63}$,    
L.~Chevalier$^\textrm{\scriptsize 144}$,    
V.~Chiarella$^\textrm{\scriptsize 50}$,    
G.~Chiarelli$^\textrm{\scriptsize 71a}$,    
G.~Chiodini$^\textrm{\scriptsize 67a}$,    
A.S.~Chisholm$^\textrm{\scriptsize 36}$,    
A.~Chitan$^\textrm{\scriptsize 27b}$,    
I.~Chiu$^\textrm{\scriptsize 163}$,    
Y.H.~Chiu$^\textrm{\scriptsize 176}$,    
M.V.~Chizhov$^\textrm{\scriptsize 79}$,    
K.~Choi$^\textrm{\scriptsize 65}$,    
A.R.~Chomont$^\textrm{\scriptsize 64}$,    
S.~Chouridou$^\textrm{\scriptsize 162}$,    
Y.S.~Chow$^\textrm{\scriptsize 119}$,    
V.~Christodoulou$^\textrm{\scriptsize 94}$,    
M.C.~Chu$^\textrm{\scriptsize 62a}$,    
J.~Chudoba$^\textrm{\scriptsize 140}$,    
A.J.~Chuinard$^\textrm{\scriptsize 103}$,    
J.J.~Chwastowski$^\textrm{\scriptsize 84}$,    
L.~Chytka$^\textrm{\scriptsize 130}$,    
D.~Cinca$^\textrm{\scriptsize 46}$,    
V.~Cindro$^\textrm{\scriptsize 91}$,    
I.A.~Cioar\u{a}$^\textrm{\scriptsize 24}$,    
A.~Ciocio$^\textrm{\scriptsize 18}$,    
F.~Cirotto$^\textrm{\scriptsize 69a,69b}$,    
Z.H.~Citron$^\textrm{\scriptsize 180,l}$,    
M.~Citterio$^\textrm{\scriptsize 68a}$,    
A.~Clark$^\textrm{\scriptsize 53}$,    
M.R.~Clark$^\textrm{\scriptsize 39}$,    
P.J.~Clark$^\textrm{\scriptsize 49}$,    
R.N.~Clarke$^\textrm{\scriptsize 18}$,    
C.~Clement$^\textrm{\scriptsize 44a,44b}$,    
Y.~Coadou$^\textrm{\scriptsize 101}$,    
M.~Cobal$^\textrm{\scriptsize 66a,66c}$,    
A.~Coccaro$^\textrm{\scriptsize 54b}$,    
J.~Cochran$^\textrm{\scriptsize 78}$,    
A.E.C.~Coimbra$^\textrm{\scriptsize 180}$,    
L.~Colasurdo$^\textrm{\scriptsize 118}$,    
B.~Cole$^\textrm{\scriptsize 39}$,    
A.P.~Colijn$^\textrm{\scriptsize 119}$,    
J.~Collot$^\textrm{\scriptsize 57}$,    
P.~Conde~Mui\~no$^\textrm{\scriptsize 139a}$,    
E.~Coniavitis$^\textrm{\scriptsize 51}$,    
S.H.~Connell$^\textrm{\scriptsize 33c}$,    
I.A.~Connelly$^\textrm{\scriptsize 100}$,    
S.~Constantinescu$^\textrm{\scriptsize 27b}$,    
F.~Conventi$^\textrm{\scriptsize 69a,ay}$,    
A.M.~Cooper-Sarkar$^\textrm{\scriptsize 134}$,    
F.~Cormier$^\textrm{\scriptsize 175}$,    
K.J.R.~Cormier$^\textrm{\scriptsize 167}$,    
M.~Corradi$^\textrm{\scriptsize 72a,72b}$,    
E.E.~Corrigan$^\textrm{\scriptsize 96}$,    
F.~Corriveau$^\textrm{\scriptsize 103,ag}$,    
A.~Cortes-Gonzalez$^\textrm{\scriptsize 36}$,    
M.J.~Costa$^\textrm{\scriptsize 174}$,    
D.~Costanzo$^\textrm{\scriptsize 148}$,    
G.~Cottin$^\textrm{\scriptsize 32}$,    
G.~Cowan$^\textrm{\scriptsize 93}$,    
B.E.~Cox$^\textrm{\scriptsize 100}$,    
J.~Crane$^\textrm{\scriptsize 100}$,    
K.~Cranmer$^\textrm{\scriptsize 124}$,    
S.J.~Crawley$^\textrm{\scriptsize 56}$,    
R.A.~Creager$^\textrm{\scriptsize 136}$,    
G.~Cree$^\textrm{\scriptsize 34}$,    
S.~Cr\'ep\'e-Renaudin$^\textrm{\scriptsize 57}$,    
F.~Crescioli$^\textrm{\scriptsize 135}$,    
M.~Cristinziani$^\textrm{\scriptsize 24}$,    
V.~Croft$^\textrm{\scriptsize 124}$,    
G.~Crosetti$^\textrm{\scriptsize 41b,41a}$,    
A.~Cueto$^\textrm{\scriptsize 98}$,    
T.~Cuhadar~Donszelmann$^\textrm{\scriptsize 148}$,    
A.R.~Cukierman$^\textrm{\scriptsize 152}$,    
M.~Curatolo$^\textrm{\scriptsize 50}$,    
J.~C\'uth$^\textrm{\scriptsize 99}$,    
S.~Czekierda$^\textrm{\scriptsize 84}$,    
P.~Czodrowski$^\textrm{\scriptsize 36}$,    
M.J.~Da~Cunha~Sargedas~De~Sousa$^\textrm{\scriptsize 59b,139b}$,    
C.~Da~Via$^\textrm{\scriptsize 100}$,    
W.~Dabrowski$^\textrm{\scriptsize 83a}$,    
T.~Dado$^\textrm{\scriptsize 28a,aa}$,    
S.~Dahbi$^\textrm{\scriptsize 35e}$,    
T.~Dai$^\textrm{\scriptsize 105}$,    
O.~Dale$^\textrm{\scriptsize 17}$,    
F.~Dallaire$^\textrm{\scriptsize 109}$,    
C.~Dallapiccola$^\textrm{\scriptsize 102}$,    
M.~Dam$^\textrm{\scriptsize 40}$,    
G.~D'amen$^\textrm{\scriptsize 23b,23a}$,    
J.R.~Dandoy$^\textrm{\scriptsize 136}$,    
M.F.~Daneri$^\textrm{\scriptsize 30}$,    
N.P.~Dang$^\textrm{\scriptsize 181,j}$,    
N.S.~Dann$^\textrm{\scriptsize 100}$,    
M.~Danninger$^\textrm{\scriptsize 175}$,    
V.~Dao$^\textrm{\scriptsize 36}$,    
G.~Darbo$^\textrm{\scriptsize 54b}$,    
O.~Dartsi$^\textrm{\scriptsize 5}$,    
A.~Dattagupta$^\textrm{\scriptsize 131}$,    
T.~Daubney$^\textrm{\scriptsize 45}$,    
S.~D'Auria$^\textrm{\scriptsize 56}$,    
W.~Davey$^\textrm{\scriptsize 24}$,    
C.~David$^\textrm{\scriptsize 45}$,    
T.~Davidek$^\textrm{\scriptsize 142}$,    
D.R.~Davis$^\textrm{\scriptsize 48}$,    
E.~Dawe$^\textrm{\scriptsize 104}$,    
I.~Dawson$^\textrm{\scriptsize 148}$,    
K.~De$^\textrm{\scriptsize 8}$,    
R.~De~Asmundis$^\textrm{\scriptsize 69a}$,    
A.~De~Benedetti$^\textrm{\scriptsize 128}$,    
S.~De~Castro$^\textrm{\scriptsize 23b,23a}$,    
S.~De~Cecco$^\textrm{\scriptsize 135}$,    
N.~De~Groot$^\textrm{\scriptsize 118}$,    
P.~de~Jong$^\textrm{\scriptsize 119}$,    
H.~De~la~Torre$^\textrm{\scriptsize 106}$,    
F.~De~Lorenzi$^\textrm{\scriptsize 78}$,    
A.~De~Maria$^\textrm{\scriptsize 52,u}$,    
D.~De~Pedis$^\textrm{\scriptsize 72a}$,    
A.~De~Salvo$^\textrm{\scriptsize 72a}$,    
U.~De~Sanctis$^\textrm{\scriptsize 73a,73b}$,    
A.~De~Santo$^\textrm{\scriptsize 155}$,    
K.~De~Vasconcelos~Corga$^\textrm{\scriptsize 101}$,    
J.B.~De~Vivie~De~Regie$^\textrm{\scriptsize 64}$,    
C.~Debenedetti$^\textrm{\scriptsize 145}$,    
D.V.~Dedovich$^\textrm{\scriptsize 79}$,    
N.~Dehghanian$^\textrm{\scriptsize 3}$,    
A.M.~Deiana$^\textrm{\scriptsize 105}$,    
M.~Del~Gaudio$^\textrm{\scriptsize 41b,41a}$,    
J.~Del~Peso$^\textrm{\scriptsize 98}$,    
D.~Delgove$^\textrm{\scriptsize 64}$,    
F.~Deliot$^\textrm{\scriptsize 144}$,    
C.M.~Delitzsch$^\textrm{\scriptsize 7}$,    
M.~Della~Pietra$^\textrm{\scriptsize 69a,69b}$,    
D.~Della~Volpe$^\textrm{\scriptsize 53}$,    
A.~Dell'Acqua$^\textrm{\scriptsize 36}$,    
L.~Dell'Asta$^\textrm{\scriptsize 25}$,    
M.~Delmastro$^\textrm{\scriptsize 5}$,    
C.~Delporte$^\textrm{\scriptsize 64}$,    
P.A.~Delsart$^\textrm{\scriptsize 57}$,    
D.A.~DeMarco$^\textrm{\scriptsize 167}$,    
S.~Demers$^\textrm{\scriptsize 183}$,    
M.~Demichev$^\textrm{\scriptsize 79}$,    
S.P.~Denisov$^\textrm{\scriptsize 122}$,    
D.~Denysiuk$^\textrm{\scriptsize 119}$,    
L.~D'Eramo$^\textrm{\scriptsize 135}$,    
D.~Derendarz$^\textrm{\scriptsize 84}$,    
J.E.~Derkaoui$^\textrm{\scriptsize 35d}$,    
F.~Derue$^\textrm{\scriptsize 135}$,    
P.~Dervan$^\textrm{\scriptsize 90}$,    
K.~Desch$^\textrm{\scriptsize 24}$,    
C.~Deterre$^\textrm{\scriptsize 45}$,    
K.~Dette$^\textrm{\scriptsize 167}$,    
M.R.~Devesa$^\textrm{\scriptsize 30}$,    
P.O.~Deviveiros$^\textrm{\scriptsize 36}$,    
A.~Dewhurst$^\textrm{\scriptsize 143}$,    
S.~Dhaliwal$^\textrm{\scriptsize 26}$,    
F.A.~Di~Bello$^\textrm{\scriptsize 53}$,    
A.~Di~Ciaccio$^\textrm{\scriptsize 73a,73b}$,    
L.~Di~Ciaccio$^\textrm{\scriptsize 5}$,    
W.K.~Di~Clemente$^\textrm{\scriptsize 136}$,    
C.~Di~Donato$^\textrm{\scriptsize 69a,69b}$,    
A.~Di~Girolamo$^\textrm{\scriptsize 36}$,    
B.~Di~Micco$^\textrm{\scriptsize 74a,74b}$,    
R.~Di~Nardo$^\textrm{\scriptsize 36}$,    
K.F.~Di~Petrillo$^\textrm{\scriptsize 58}$,    
A.~Di~Simone$^\textrm{\scriptsize 51}$,    
R.~Di~Sipio$^\textrm{\scriptsize 167}$,    
D.~Di~Valentino$^\textrm{\scriptsize 34}$,    
C.~Diaconu$^\textrm{\scriptsize 101}$,    
M.~Diamond$^\textrm{\scriptsize 167}$,    
F.A.~Dias$^\textrm{\scriptsize 40}$,    
T.~Dias~Do~Vale$^\textrm{\scriptsize 139a}$,    
M.A.~Diaz$^\textrm{\scriptsize 146a}$,    
J.~Dickinson$^\textrm{\scriptsize 18}$,    
E.B.~Diehl$^\textrm{\scriptsize 105}$,    
J.~Dietrich$^\textrm{\scriptsize 19}$,    
S.~D\'iez~Cornell$^\textrm{\scriptsize 45}$,    
A.~Dimitrievska$^\textrm{\scriptsize 18}$,    
J.~Dingfelder$^\textrm{\scriptsize 24}$,    
F.~Dittus$^\textrm{\scriptsize 36}$,    
F.~Djama$^\textrm{\scriptsize 101}$,    
T.~Djobava$^\textrm{\scriptsize 159b}$,    
J.I.~Djuvsland$^\textrm{\scriptsize 60a}$,    
M.A.B.~Do~Vale$^\textrm{\scriptsize 80c}$,    
M.~Dobre$^\textrm{\scriptsize 27b}$,    
D.~Dodsworth$^\textrm{\scriptsize 26}$,    
C.~Doglioni$^\textrm{\scriptsize 96}$,    
J.~Dolejsi$^\textrm{\scriptsize 142}$,    
Z.~Dolezal$^\textrm{\scriptsize 142}$,    
M.~Donadelli$^\textrm{\scriptsize 80d}$,    
J.~Donini$^\textrm{\scriptsize 38}$,    
A.~D'onofrio$^\textrm{\scriptsize 92}$,    
M.~D'Onofrio$^\textrm{\scriptsize 90}$,    
J.~Dopke$^\textrm{\scriptsize 143}$,    
A.~Doria$^\textrm{\scriptsize 69a}$,    
M.T.~Dova$^\textrm{\scriptsize 88}$,    
A.T.~Doyle$^\textrm{\scriptsize 56}$,    
E.~Drechsler$^\textrm{\scriptsize 52}$,    
E.~Dreyer$^\textrm{\scriptsize 151}$,    
T.~Dreyer$^\textrm{\scriptsize 52}$,    
M.~Dris$^\textrm{\scriptsize 10}$,    
Y.~Du$^\textrm{\scriptsize 59b}$,    
J.~Duarte-Campderros$^\textrm{\scriptsize 161}$,    
F.~Dubinin$^\textrm{\scriptsize 110}$,    
A.~Dubreuil$^\textrm{\scriptsize 53}$,    
E.~Duchovni$^\textrm{\scriptsize 180}$,    
G.~Duckeck$^\textrm{\scriptsize 113}$,    
A.~Ducourthial$^\textrm{\scriptsize 135}$,    
O.A.~Ducu$^\textrm{\scriptsize 109,z}$,    
D.~Duda$^\textrm{\scriptsize 119}$,    
A.~Dudarev$^\textrm{\scriptsize 36}$,    
A.C.~Dudder$^\textrm{\scriptsize 99}$,    
E.M.~Duffield$^\textrm{\scriptsize 18}$,    
L.~Duflot$^\textrm{\scriptsize 64}$,    
M.~D\"uhrssen$^\textrm{\scriptsize 36}$,    
C.~D{\"u}lsen$^\textrm{\scriptsize 182}$,    
M.~Dumancic$^\textrm{\scriptsize 180}$,    
A.E.~Dumitriu$^\textrm{\scriptsize 27b,d}$,    
A.K.~Duncan$^\textrm{\scriptsize 56}$,    
M.~Dunford$^\textrm{\scriptsize 60a}$,    
A.~Duperrin$^\textrm{\scriptsize 101}$,    
H.~Duran~Yildiz$^\textrm{\scriptsize 4a}$,    
M.~D\"uren$^\textrm{\scriptsize 55}$,    
A.~Durglishvili$^\textrm{\scriptsize 159b}$,    
D.~Duschinger$^\textrm{\scriptsize 47}$,    
B.~Dutta$^\textrm{\scriptsize 45}$,    
D.~Duvnjak$^\textrm{\scriptsize 1}$,    
M.~Dyndal$^\textrm{\scriptsize 45}$,    
B.S.~Dziedzic$^\textrm{\scriptsize 84}$,    
C.~Eckardt$^\textrm{\scriptsize 45}$,    
K.M.~Ecker$^\textrm{\scriptsize 114}$,    
R.C.~Edgar$^\textrm{\scriptsize 105}$,    
T.~Eifert$^\textrm{\scriptsize 36}$,    
G.~Eigen$^\textrm{\scriptsize 17}$,    
K.~Einsweiler$^\textrm{\scriptsize 18}$,    
T.~Ekelof$^\textrm{\scriptsize 172}$,    
M.~El~Kacimi$^\textrm{\scriptsize 35c}$,    
R.~El~Kosseifi$^\textrm{\scriptsize 101}$,    
V.~Ellajosyula$^\textrm{\scriptsize 101}$,    
M.~Ellert$^\textrm{\scriptsize 172}$,    
F.~Ellinghaus$^\textrm{\scriptsize 182}$,    
A.A.~Elliot$^\textrm{\scriptsize 176}$,    
N.~Ellis$^\textrm{\scriptsize 36}$,    
J.~Elmsheuser$^\textrm{\scriptsize 29}$,    
M.~Elsing$^\textrm{\scriptsize 36}$,    
D.~Emeliyanov$^\textrm{\scriptsize 143}$,    
Y.~Enari$^\textrm{\scriptsize 163}$,    
J.S.~Ennis$^\textrm{\scriptsize 178}$,    
M.B.~Epland$^\textrm{\scriptsize 48}$,    
J.~Erdmann$^\textrm{\scriptsize 46}$,    
A.~Ereditato$^\textrm{\scriptsize 20}$,    
S.~Errede$^\textrm{\scriptsize 173}$,    
M.~Escalier$^\textrm{\scriptsize 64}$,    
C.~Escobar$^\textrm{\scriptsize 174}$,    
B.~Esposito$^\textrm{\scriptsize 50}$,    
O.~Estrada~Pastor$^\textrm{\scriptsize 174}$,    
A.I.~Etienvre$^\textrm{\scriptsize 144}$,    
E.~Etzion$^\textrm{\scriptsize 161}$,    
H.~Evans$^\textrm{\scriptsize 65}$,    
A.~Ezhilov$^\textrm{\scriptsize 137}$,    
M.~Ezzi$^\textrm{\scriptsize 35e}$,    
F.~Fabbri$^\textrm{\scriptsize 23b,23a}$,    
L.~Fabbri$^\textrm{\scriptsize 23b,23a}$,    
V.~Fabiani$^\textrm{\scriptsize 118}$,    
G.~Facini$^\textrm{\scriptsize 94}$,    
R.M.~Faisca~Rodrigues~Pereira$^\textrm{\scriptsize 139a}$,    
R.M.~Fakhrutdinov$^\textrm{\scriptsize 122}$,    
S.~Falciano$^\textrm{\scriptsize 72a}$,    
P.J.~Falke$^\textrm{\scriptsize 5}$,    
S.~Falke$^\textrm{\scriptsize 5}$,    
J.~Faltova$^\textrm{\scriptsize 142}$,    
Y.~Fang$^\textrm{\scriptsize 15a}$,    
M.~Fanti$^\textrm{\scriptsize 68a,68b}$,    
A.~Farbin$^\textrm{\scriptsize 8}$,    
A.~Farilla$^\textrm{\scriptsize 74a}$,    
E.M.~Farina$^\textrm{\scriptsize 70a,70b}$,    
T.~Farooque$^\textrm{\scriptsize 106}$,    
S.~Farrell$^\textrm{\scriptsize 18}$,    
S.M.~Farrington$^\textrm{\scriptsize 178}$,    
P.~Farthouat$^\textrm{\scriptsize 36}$,    
F.~Fassi$^\textrm{\scriptsize 35e}$,    
P.~Fassnacht$^\textrm{\scriptsize 36}$,    
D.~Fassouliotis$^\textrm{\scriptsize 9}$,    
M.~Faucci~Giannelli$^\textrm{\scriptsize 49}$,    
A.~Favareto$^\textrm{\scriptsize 54b,54a}$,    
W.J.~Fawcett$^\textrm{\scriptsize 53}$,    
L.~Fayard$^\textrm{\scriptsize 64}$,    
O.L.~Fedin$^\textrm{\scriptsize 137,r}$,    
W.~Fedorko$^\textrm{\scriptsize 175}$,    
M.~Feickert$^\textrm{\scriptsize 42}$,    
S.~Feigl$^\textrm{\scriptsize 133}$,    
L.~Feligioni$^\textrm{\scriptsize 101}$,    
C.~Feng$^\textrm{\scriptsize 59b}$,    
E.J.~Feng$^\textrm{\scriptsize 36}$,    
M.~Feng$^\textrm{\scriptsize 48}$,    
M.J.~Fenton$^\textrm{\scriptsize 56}$,    
A.B.~Fenyuk$^\textrm{\scriptsize 122}$,    
L.~Feremenga$^\textrm{\scriptsize 8}$,    
J.~Ferrando$^\textrm{\scriptsize 45}$,    
A.~Ferrari$^\textrm{\scriptsize 172}$,    
P.~Ferrari$^\textrm{\scriptsize 119}$,    
R.~Ferrari$^\textrm{\scriptsize 70a}$,    
D.E.~Ferreira~de~Lima$^\textrm{\scriptsize 60b}$,    
A.~Ferrer$^\textrm{\scriptsize 174}$,    
D.~Ferrere$^\textrm{\scriptsize 53}$,    
C.~Ferretti$^\textrm{\scriptsize 105}$,    
F.~Fiedler$^\textrm{\scriptsize 99}$,    
A.~Filip\v{c}i\v{c}$^\textrm{\scriptsize 91}$,    
F.~Filthaut$^\textrm{\scriptsize 118}$,    
M.~Fincke-Keeler$^\textrm{\scriptsize 176}$,    
K.D.~Finelli$^\textrm{\scriptsize 25}$,    
M.C.N.~Fiolhais$^\textrm{\scriptsize 139a,139c,a}$,    
L.~Fiorini$^\textrm{\scriptsize 174}$,    
C.~Fischer$^\textrm{\scriptsize 14}$,    
J.~Fischer$^\textrm{\scriptsize 182}$,    
W.C.~Fisher$^\textrm{\scriptsize 106}$,    
N.~Flaschel$^\textrm{\scriptsize 45}$,    
I.~Fleck$^\textrm{\scriptsize 150}$,    
P.~Fleischmann$^\textrm{\scriptsize 105}$,    
R.R.M.~Fletcher$^\textrm{\scriptsize 136}$,    
T.~Flick$^\textrm{\scriptsize 182}$,    
B.M.~Flierl$^\textrm{\scriptsize 113}$,    
L.~Flores$^\textrm{\scriptsize 136}$,    
L.R.~Flores~Castillo$^\textrm{\scriptsize 62a}$,    
N.~Fomin$^\textrm{\scriptsize 17}$,    
G.T.~Forcolin$^\textrm{\scriptsize 100}$,    
A.~Formica$^\textrm{\scriptsize 144}$,    
F.A.~F\"orster$^\textrm{\scriptsize 14}$,    
A.C.~Forti$^\textrm{\scriptsize 100}$,    
A.G.~Foster$^\textrm{\scriptsize 21}$,    
D.~Fournier$^\textrm{\scriptsize 64}$,    
H.~Fox$^\textrm{\scriptsize 89}$,    
S.~Fracchia$^\textrm{\scriptsize 148}$,    
P.~Francavilla$^\textrm{\scriptsize 71a,71b}$,    
M.~Franchini$^\textrm{\scriptsize 23b,23a}$,    
S.~Franchino$^\textrm{\scriptsize 60a}$,    
D.~Francis$^\textrm{\scriptsize 36}$,    
L.~Franconi$^\textrm{\scriptsize 133}$,    
M.~Franklin$^\textrm{\scriptsize 58}$,    
M.~Frate$^\textrm{\scriptsize 171}$,    
M.~Fraternali$^\textrm{\scriptsize 70a,70b}$,    
D.~Freeborn$^\textrm{\scriptsize 94}$,    
S.M.~Fressard-Batraneanu$^\textrm{\scriptsize 36}$,    
B.~Freund$^\textrm{\scriptsize 109}$,    
W.S.~Freund$^\textrm{\scriptsize 80b}$,    
D.~Froidevaux$^\textrm{\scriptsize 36}$,    
J.A.~Frost$^\textrm{\scriptsize 134}$,    
C.~Fukunaga$^\textrm{\scriptsize 164}$,    
T.~Fusayasu$^\textrm{\scriptsize 115}$,    
J.~Fuster$^\textrm{\scriptsize 174}$,    
O.~Gabizon$^\textrm{\scriptsize 160}$,    
A.~Gabrielli$^\textrm{\scriptsize 23b,23a}$,    
A.~Gabrielli$^\textrm{\scriptsize 18}$,    
G.P.~Gach$^\textrm{\scriptsize 83a}$,    
S.~Gadatsch$^\textrm{\scriptsize 53}$,    
S.~Gadomski$^\textrm{\scriptsize 53}$,    
P.~Gadow$^\textrm{\scriptsize 114}$,    
G.~Gagliardi$^\textrm{\scriptsize 54b,54a}$,    
L.G.~Gagnon$^\textrm{\scriptsize 109}$,    
C.~Galea$^\textrm{\scriptsize 27b}$,    
B.~Galhardo$^\textrm{\scriptsize 139a,139c}$,    
E.J.~Gallas$^\textrm{\scriptsize 134}$,    
B.J.~Gallop$^\textrm{\scriptsize 143}$,    
P.~Gallus$^\textrm{\scriptsize 141}$,    
G.~Galster$^\textrm{\scriptsize 40}$,    
R.~Gamboa~Goni$^\textrm{\scriptsize 92}$,    
K.K.~Gan$^\textrm{\scriptsize 126}$,    
S.~Ganguly$^\textrm{\scriptsize 180}$,    
Y.~Gao$^\textrm{\scriptsize 90}$,    
Y.S.~Gao$^\textrm{\scriptsize 31,n}$,    
C.~Garc\'ia$^\textrm{\scriptsize 174}$,    
J.E.~Garc\'ia~Navarro$^\textrm{\scriptsize 174}$,    
J.A.~Garc\'ia~Pascual$^\textrm{\scriptsize 15a}$,    
M.~Garcia-Sciveres$^\textrm{\scriptsize 18}$,    
R.W.~Gardner$^\textrm{\scriptsize 37}$,    
N.~Garelli$^\textrm{\scriptsize 152}$,    
V.~Garonne$^\textrm{\scriptsize 133}$,    
K.~Gasnikova$^\textrm{\scriptsize 45}$,    
A.~Gaudiello$^\textrm{\scriptsize 54b,54a}$,    
G.~Gaudio$^\textrm{\scriptsize 70a}$,    
I.L.~Gavrilenko$^\textrm{\scriptsize 110}$,    
A.~Gavrilyuk$^\textrm{\scriptsize 123}$,    
C.~Gay$^\textrm{\scriptsize 175}$,    
G.~Gaycken$^\textrm{\scriptsize 24}$,    
E.N.~Gazis$^\textrm{\scriptsize 10}$,    
C.N.P.~Gee$^\textrm{\scriptsize 143}$,    
J.~Geisen$^\textrm{\scriptsize 52}$,    
M.~Geisen$^\textrm{\scriptsize 99}$,    
M.P.~Geisler$^\textrm{\scriptsize 60a}$,    
K.~Gellerstedt$^\textrm{\scriptsize 44a,44b}$,    
C.~Gemme$^\textrm{\scriptsize 54b}$,    
M.H.~Genest$^\textrm{\scriptsize 57}$,    
C.~Geng$^\textrm{\scriptsize 105}$,    
S.~Gentile$^\textrm{\scriptsize 72a,72b}$,    
C.~Gentsos$^\textrm{\scriptsize 162}$,    
S.~George$^\textrm{\scriptsize 93}$,    
D.~Gerbaudo$^\textrm{\scriptsize 14}$,    
G.~Gessner$^\textrm{\scriptsize 46}$,    
S.~Ghasemi$^\textrm{\scriptsize 150}$,    
B.~Giacobbe$^\textrm{\scriptsize 23b}$,    
S.~Giagu$^\textrm{\scriptsize 72a,72b}$,    
N.~Giangiacomi$^\textrm{\scriptsize 23b,23a}$,    
P.~Giannetti$^\textrm{\scriptsize 71a}$,    
S.M.~Gibson$^\textrm{\scriptsize 93}$,    
M.~Gignac$^\textrm{\scriptsize 145}$,    
D.~Gillberg$^\textrm{\scriptsize 34}$,    
G.~Gilles$^\textrm{\scriptsize 182}$,    
D.M.~Gingrich$^\textrm{\scriptsize 3,ax}$,    
M.P.~Giordani$^\textrm{\scriptsize 66a,66c}$,    
F.M.~Giorgi$^\textrm{\scriptsize 23b}$,    
P.F.~Giraud$^\textrm{\scriptsize 144}$,    
P.~Giromini$^\textrm{\scriptsize 58}$,    
G.~Giugliarelli$^\textrm{\scriptsize 66a,66c}$,    
D.~Giugni$^\textrm{\scriptsize 68a}$,    
F.~Giuli$^\textrm{\scriptsize 134}$,    
M.~Giulini$^\textrm{\scriptsize 60b}$,    
S.~Gkaitatzis$^\textrm{\scriptsize 162}$,    
I.~Gkialas$^\textrm{\scriptsize 9,i}$,    
E.L.~Gkougkousis$^\textrm{\scriptsize 14}$,    
P.~Gkountoumis$^\textrm{\scriptsize 10}$,    
L.K.~Gladilin$^\textrm{\scriptsize 112}$,    
C.~Glasman$^\textrm{\scriptsize 98}$,    
J.~Glatzer$^\textrm{\scriptsize 14}$,    
P.C.F.~Glaysher$^\textrm{\scriptsize 45}$,    
A.~Glazov$^\textrm{\scriptsize 45}$,    
M.~Goblirsch-Kolb$^\textrm{\scriptsize 26}$,    
J.~Godlewski$^\textrm{\scriptsize 84}$,    
S.~Goldfarb$^\textrm{\scriptsize 104}$,    
T.~Golling$^\textrm{\scriptsize 53}$,    
D.~Golubkov$^\textrm{\scriptsize 122}$,    
A.~Gomes$^\textrm{\scriptsize 139a,139b}$,    
R.~Goncalves~Gama$^\textrm{\scriptsize 80a}$,    
R.~Gon\c{c}alo$^\textrm{\scriptsize 139a}$,    
G.~Gonella$^\textrm{\scriptsize 51}$,    
L.~Gonella$^\textrm{\scriptsize 21}$,    
A.~Gongadze$^\textrm{\scriptsize 79}$,    
F.~Gonnella$^\textrm{\scriptsize 21}$,    
J.L.~Gonski$^\textrm{\scriptsize 58}$,    
S.~Gonz\'alez~de~la~Hoz$^\textrm{\scriptsize 174}$,    
S.~Gonzalez-Sevilla$^\textrm{\scriptsize 53}$,    
L.~Goossens$^\textrm{\scriptsize 36}$,    
P.A.~Gorbounov$^\textrm{\scriptsize 123}$,    
H.A.~Gordon$^\textrm{\scriptsize 29}$,    
B.~Gorini$^\textrm{\scriptsize 36}$,    
E.~Gorini$^\textrm{\scriptsize 67a,67b}$,    
A.~Gori\v{s}ek$^\textrm{\scriptsize 91}$,    
A.T.~Goshaw$^\textrm{\scriptsize 48}$,    
C.~G\"ossling$^\textrm{\scriptsize 46}$,    
M.I.~Gostkin$^\textrm{\scriptsize 79}$,    
C.A.~Gottardo$^\textrm{\scriptsize 24}$,    
C.R.~Goudet$^\textrm{\scriptsize 64}$,    
D.~Goujdami$^\textrm{\scriptsize 35c}$,    
A.G.~Goussiou$^\textrm{\scriptsize 147}$,    
N.~Govender$^\textrm{\scriptsize 33c,b}$,    
C.~Goy$^\textrm{\scriptsize 5}$,    
E.~Gozani$^\textrm{\scriptsize 160}$,    
I.~Grabowska-Bold$^\textrm{\scriptsize 83a}$,    
P.O.J.~Gradin$^\textrm{\scriptsize 172}$,    
E.C.~Graham$^\textrm{\scriptsize 90}$,    
J.~Gramling$^\textrm{\scriptsize 171}$,    
E.~Gramstad$^\textrm{\scriptsize 133}$,    
S.~Grancagnolo$^\textrm{\scriptsize 19}$,    
V.~Gratchev$^\textrm{\scriptsize 137}$,    
P.M.~Gravila$^\textrm{\scriptsize 27f}$,    
C.~Gray$^\textrm{\scriptsize 56}$,    
H.M.~Gray$^\textrm{\scriptsize 18}$,    
Z.D.~Greenwood$^\textrm{\scriptsize 95}$,    
C.~Grefe$^\textrm{\scriptsize 24}$,    
K.~Gregersen$^\textrm{\scriptsize 94}$,    
I.M.~Gregor$^\textrm{\scriptsize 45}$,    
P.~Grenier$^\textrm{\scriptsize 152}$,    
K.~Grevtsov$^\textrm{\scriptsize 45}$,    
J.~Griffiths$^\textrm{\scriptsize 8}$,    
A.A.~Grillo$^\textrm{\scriptsize 145}$,    
K.~Grimm$^\textrm{\scriptsize 31,m}$,    
S.~Grinstein$^\textrm{\scriptsize 14,ac}$,    
Ph.~Gris$^\textrm{\scriptsize 38}$,    
J.-F.~Grivaz$^\textrm{\scriptsize 64}$,    
S.~Groh$^\textrm{\scriptsize 99}$,    
E.~Gross$^\textrm{\scriptsize 180}$,    
J.~Grosse-Knetter$^\textrm{\scriptsize 52}$,    
G.C.~Grossi$^\textrm{\scriptsize 95}$,    
Z.J.~Grout$^\textrm{\scriptsize 94}$,    
A.~Grummer$^\textrm{\scriptsize 117}$,    
L.~Guan$^\textrm{\scriptsize 105}$,    
W.~Guan$^\textrm{\scriptsize 181}$,    
J.~Guenther$^\textrm{\scriptsize 36}$,    
A.~Guerguichon$^\textrm{\scriptsize 64}$,    
F.~Guescini$^\textrm{\scriptsize 168a}$,    
D.~Guest$^\textrm{\scriptsize 171}$,    
O.~Gueta$^\textrm{\scriptsize 161}$,    
R.~Gugel$^\textrm{\scriptsize 51}$,    
B.~Gui$^\textrm{\scriptsize 126}$,    
T.~Guillemin$^\textrm{\scriptsize 5}$,    
S.~Guindon$^\textrm{\scriptsize 36}$,    
U.~Gul$^\textrm{\scriptsize 56}$,    
C.~Gumpert$^\textrm{\scriptsize 36}$,    
J.~Guo$^\textrm{\scriptsize 59c}$,    
W.~Guo$^\textrm{\scriptsize 105}$,    
Y.~Guo$^\textrm{\scriptsize 59a,t}$,    
Z.~Guo$^\textrm{\scriptsize 101}$,    
R.~Gupta$^\textrm{\scriptsize 42}$,    
S.~Gupta$^\textrm{\scriptsize 134}$,    
S.~Gurbuz$^\textrm{\scriptsize 12c}$,    
G.~Gustavino$^\textrm{\scriptsize 128}$,    
B.J.~Gutelman$^\textrm{\scriptsize 160}$,    
P.~Gutierrez$^\textrm{\scriptsize 128}$,    
N.G.~Gutierrez~Ortiz$^\textrm{\scriptsize 94}$,    
C.~Gutschow$^\textrm{\scriptsize 94}$,    
C.~Guyot$^\textrm{\scriptsize 144}$,    
M.P.~Guzik$^\textrm{\scriptsize 83a}$,    
C.~Gwenlan$^\textrm{\scriptsize 134}$,    
C.B.~Gwilliam$^\textrm{\scriptsize 90}$,    
A.~Haas$^\textrm{\scriptsize 124}$,    
C.~Haber$^\textrm{\scriptsize 18}$,    
H.K.~Hadavand$^\textrm{\scriptsize 8}$,    
N.~Haddad$^\textrm{\scriptsize 35e}$,    
A.~Hadef$^\textrm{\scriptsize 101}$,    
S.~Hageb\"ock$^\textrm{\scriptsize 24}$,    
M.~Hagihara$^\textrm{\scriptsize 169}$,    
H.~Hakobyan$^\textrm{\scriptsize 184,*}$,    
M.~Haleem$^\textrm{\scriptsize 177}$,    
J.~Haley$^\textrm{\scriptsize 129}$,    
G.~Halladjian$^\textrm{\scriptsize 106}$,    
G.D.~Hallewell$^\textrm{\scriptsize 101}$,    
K.~Hamacher$^\textrm{\scriptsize 182}$,    
P.~Hamal$^\textrm{\scriptsize 130}$,    
K.~Hamano$^\textrm{\scriptsize 176}$,    
A.~Hamilton$^\textrm{\scriptsize 33a}$,    
G.N.~Hamity$^\textrm{\scriptsize 148}$,    
K.~Han$^\textrm{\scriptsize 59a,ab}$,    
L.~Han$^\textrm{\scriptsize 59a}$,    
S.~Han$^\textrm{\scriptsize 15a}$,    
K.~Hanagaki$^\textrm{\scriptsize 81,x}$,    
M.~Hance$^\textrm{\scriptsize 145}$,    
D.M.~Handl$^\textrm{\scriptsize 113}$,    
B.~Haney$^\textrm{\scriptsize 136}$,    
R.~Hankache$^\textrm{\scriptsize 135}$,    
P.~Hanke$^\textrm{\scriptsize 60a}$,    
E.~Hansen$^\textrm{\scriptsize 96}$,    
J.B.~Hansen$^\textrm{\scriptsize 40}$,    
J.D.~Hansen$^\textrm{\scriptsize 40}$,    
M.C.~Hansen$^\textrm{\scriptsize 24}$,    
P.H.~Hansen$^\textrm{\scriptsize 40}$,    
E.C.~Hanson$^\textrm{\scriptsize 100}$,    
K.~Hara$^\textrm{\scriptsize 169}$,    
A.S.~Hard$^\textrm{\scriptsize 181}$,    
T.~Harenberg$^\textrm{\scriptsize 182}$,    
S.~Harkusha$^\textrm{\scriptsize 107}$,    
P.F.~Harrison$^\textrm{\scriptsize 178}$,    
N.M.~Hartmann$^\textrm{\scriptsize 113}$,    
Y.~Hasegawa$^\textrm{\scriptsize 149}$,    
A.~Hasib$^\textrm{\scriptsize 49}$,    
S.~Hassani$^\textrm{\scriptsize 144}$,    
S.~Haug$^\textrm{\scriptsize 20}$,    
R.~Hauser$^\textrm{\scriptsize 106}$,    
L.~Hauswald$^\textrm{\scriptsize 47}$,    
L.B.~Havener$^\textrm{\scriptsize 39}$,    
M.~Havranek$^\textrm{\scriptsize 141}$,    
C.M.~Hawkes$^\textrm{\scriptsize 21}$,    
R.J.~Hawkings$^\textrm{\scriptsize 36}$,    
D.~Hayden$^\textrm{\scriptsize 106}$,    
C.~Hayes$^\textrm{\scriptsize 154}$,    
C.P.~Hays$^\textrm{\scriptsize 134}$,    
J.M.~Hays$^\textrm{\scriptsize 92}$,    
H.S.~Hayward$^\textrm{\scriptsize 90}$,    
S.J.~Haywood$^\textrm{\scriptsize 143}$,    
M.P.~Heath$^\textrm{\scriptsize 49}$,    
V.~Hedberg$^\textrm{\scriptsize 96}$,    
L.~Heelan$^\textrm{\scriptsize 8}$,    
S.~Heer$^\textrm{\scriptsize 24}$,    
K.K.~Heidegger$^\textrm{\scriptsize 51}$,    
J.~Heilman$^\textrm{\scriptsize 34}$,    
S.~Heim$^\textrm{\scriptsize 45}$,    
T.~Heim$^\textrm{\scriptsize 18}$,    
B.~Heinemann$^\textrm{\scriptsize 45,as}$,    
J.J.~Heinrich$^\textrm{\scriptsize 113}$,    
L.~Heinrich$^\textrm{\scriptsize 124}$,    
C.~Heinz$^\textrm{\scriptsize 55}$,    
J.~Hejbal$^\textrm{\scriptsize 140}$,    
L.~Helary$^\textrm{\scriptsize 36}$,    
A.~Held$^\textrm{\scriptsize 175}$,    
S.~Hellesund$^\textrm{\scriptsize 133}$,    
S.~Hellman$^\textrm{\scriptsize 44a,44b}$,    
C.~Helsens$^\textrm{\scriptsize 36}$,    
R.C.W.~Henderson$^\textrm{\scriptsize 89}$,    
Y.~Heng$^\textrm{\scriptsize 181}$,    
S.~Henkelmann$^\textrm{\scriptsize 175}$,    
A.M.~Henriques~Correia$^\textrm{\scriptsize 36}$,    
G.H.~Herbert$^\textrm{\scriptsize 19}$,    
H.~Herde$^\textrm{\scriptsize 26}$,    
V.~Herget$^\textrm{\scriptsize 177}$,    
Y.~Hern\'andez~Jim\'enez$^\textrm{\scriptsize 33e}$,    
H.~Herr$^\textrm{\scriptsize 99}$,    
G.~Herten$^\textrm{\scriptsize 51}$,    
R.~Hertenberger$^\textrm{\scriptsize 113}$,    
L.~Hervas$^\textrm{\scriptsize 36}$,    
T.C.~Herwig$^\textrm{\scriptsize 136}$,    
G.G.~Hesketh$^\textrm{\scriptsize 94}$,    
N.P.~Hessey$^\textrm{\scriptsize 168a}$,    
J.W.~Hetherly$^\textrm{\scriptsize 42}$,    
S.~Higashino$^\textrm{\scriptsize 81}$,    
E.~Hig\'on-Rodriguez$^\textrm{\scriptsize 174}$,    
K.~Hildebrand$^\textrm{\scriptsize 37}$,    
E.~Hill$^\textrm{\scriptsize 176}$,    
J.C.~Hill$^\textrm{\scriptsize 32}$,    
K.H.~Hiller$^\textrm{\scriptsize 45}$,    
S.J.~Hillier$^\textrm{\scriptsize 21}$,    
M.~Hils$^\textrm{\scriptsize 47}$,    
I.~Hinchliffe$^\textrm{\scriptsize 18}$,    
M.~Hirose$^\textrm{\scriptsize 132}$,    
D.~Hirschbuehl$^\textrm{\scriptsize 182}$,    
B.~Hiti$^\textrm{\scriptsize 91}$,    
O.~Hladik$^\textrm{\scriptsize 140}$,    
D.R.~Hlaluku$^\textrm{\scriptsize 33e}$,    
X.~Hoad$^\textrm{\scriptsize 49}$,    
J.~Hobbs$^\textrm{\scriptsize 154}$,    
N.~Hod$^\textrm{\scriptsize 168a}$,    
M.C.~Hodgkinson$^\textrm{\scriptsize 148}$,    
A.~Hoecker$^\textrm{\scriptsize 36}$,    
M.R.~Hoeferkamp$^\textrm{\scriptsize 117}$,    
F.~Hoenig$^\textrm{\scriptsize 113}$,    
D.~Hohn$^\textrm{\scriptsize 24}$,    
D.~Hohov$^\textrm{\scriptsize 64}$,    
T.R.~Holmes$^\textrm{\scriptsize 37}$,    
M.~Holzbock$^\textrm{\scriptsize 113}$,    
M.~Homann$^\textrm{\scriptsize 46}$,    
S.~Honda$^\textrm{\scriptsize 169}$,    
T.~Honda$^\textrm{\scriptsize 81}$,    
T.M.~Hong$^\textrm{\scriptsize 138}$,    
A.~H\"{o}nle$^\textrm{\scriptsize 114}$,    
B.H.~Hooberman$^\textrm{\scriptsize 173}$,    
W.H.~Hopkins$^\textrm{\scriptsize 131}$,    
Y.~Horii$^\textrm{\scriptsize 116}$,    
P.~Horn$^\textrm{\scriptsize 47}$,    
A.J.~Horton$^\textrm{\scriptsize 151}$,    
L.A.~Horyn$^\textrm{\scriptsize 37}$,    
J-Y.~Hostachy$^\textrm{\scriptsize 57}$,    
A.~Hostiuc$^\textrm{\scriptsize 147}$,    
S.~Hou$^\textrm{\scriptsize 157}$,    
A.~Hoummada$^\textrm{\scriptsize 35a}$,    
J.~Howarth$^\textrm{\scriptsize 100}$,    
J.~Hoya$^\textrm{\scriptsize 88}$,    
M.~Hrabovsky$^\textrm{\scriptsize 130}$,    
J.~Hrdinka$^\textrm{\scriptsize 36}$,    
I.~Hristova$^\textrm{\scriptsize 19}$,    
J.~Hrivnac$^\textrm{\scriptsize 64}$,    
A.~Hrynevich$^\textrm{\scriptsize 108}$,    
T.~Hryn'ova$^\textrm{\scriptsize 5}$,    
P.J.~Hsu$^\textrm{\scriptsize 63}$,    
S.-C.~Hsu$^\textrm{\scriptsize 147}$,    
Q.~Hu$^\textrm{\scriptsize 29}$,    
S.~Hu$^\textrm{\scriptsize 59c}$,    
Y.~Huang$^\textrm{\scriptsize 15a}$,    
Z.~Hubacek$^\textrm{\scriptsize 141}$,    
F.~Hubaut$^\textrm{\scriptsize 101}$,    
M.~Huebner$^\textrm{\scriptsize 24}$,    
F.~Huegging$^\textrm{\scriptsize 24}$,    
T.B.~Huffman$^\textrm{\scriptsize 134}$,    
E.W.~Hughes$^\textrm{\scriptsize 39}$,    
M.~Huhtinen$^\textrm{\scriptsize 36}$,    
R.F.H.~Hunter$^\textrm{\scriptsize 34}$,    
P.~Huo$^\textrm{\scriptsize 154}$,    
A.M.~Hupe$^\textrm{\scriptsize 34}$,    
N.~Huseynov$^\textrm{\scriptsize 79,ai}$,    
J.~Huston$^\textrm{\scriptsize 106}$,    
J.~Huth$^\textrm{\scriptsize 58}$,    
R.~Hyneman$^\textrm{\scriptsize 105}$,    
G.~Iacobucci$^\textrm{\scriptsize 53}$,    
G.~Iakovidis$^\textrm{\scriptsize 29}$,    
I.~Ibragimov$^\textrm{\scriptsize 150}$,    
L.~Iconomidou-Fayard$^\textrm{\scriptsize 64}$,    
Z.~Idrissi$^\textrm{\scriptsize 35e}$,    
P.~Iengo$^\textrm{\scriptsize 36}$,    
R.~Ignazzi$^\textrm{\scriptsize 40}$,    
O.~Igonkina$^\textrm{\scriptsize 119,ae,*}$,    
R.~Iguchi$^\textrm{\scriptsize 163}$,    
T.~Iizawa$^\textrm{\scriptsize 179}$,    
Y.~Ikegami$^\textrm{\scriptsize 81}$,    
M.~Ikeno$^\textrm{\scriptsize 81}$,    
D.~Iliadis$^\textrm{\scriptsize 162}$,    
N.~Ilic$^\textrm{\scriptsize 152}$,    
F.~Iltzsche$^\textrm{\scriptsize 47}$,    
G.~Introzzi$^\textrm{\scriptsize 70a,70b}$,    
M.~Iodice$^\textrm{\scriptsize 74a}$,    
K.~Iordanidou$^\textrm{\scriptsize 39}$,    
V.~Ippolito$^\textrm{\scriptsize 72a,72b}$,    
M.F.~Isacson$^\textrm{\scriptsize 172}$,    
N.~Ishijima$^\textrm{\scriptsize 132}$,    
M.~Ishino$^\textrm{\scriptsize 163}$,    
M.~Ishitsuka$^\textrm{\scriptsize 165}$,    
C.~Issever$^\textrm{\scriptsize 134}$,    
S.~Istin$^\textrm{\scriptsize 12c,ap}$,    
F.~Ito$^\textrm{\scriptsize 169}$,    
J.M.~Iturbe~Ponce$^\textrm{\scriptsize 62a}$,    
R.~Iuppa$^\textrm{\scriptsize 75a,75b}$,    
A.~Ivina$^\textrm{\scriptsize 180}$,    
H.~Iwasaki$^\textrm{\scriptsize 81}$,    
J.M.~Izen$^\textrm{\scriptsize 43}$,    
V.~Izzo$^\textrm{\scriptsize 69a}$,    
S.~Jabbar$^\textrm{\scriptsize 3}$,    
P.~Jacka$^\textrm{\scriptsize 140}$,    
P.~Jackson$^\textrm{\scriptsize 1}$,    
R.M.~Jacobs$^\textrm{\scriptsize 24}$,    
V.~Jain$^\textrm{\scriptsize 2}$,    
G.~J\"akel$^\textrm{\scriptsize 182}$,    
K.B.~Jakobi$^\textrm{\scriptsize 99}$,    
K.~Jakobs$^\textrm{\scriptsize 51}$,    
S.~Jakobsen$^\textrm{\scriptsize 76}$,    
T.~Jakoubek$^\textrm{\scriptsize 140}$,    
D.O.~Jamin$^\textrm{\scriptsize 129}$,    
D.K.~Jana$^\textrm{\scriptsize 95}$,    
R.~Jansky$^\textrm{\scriptsize 53}$,    
J.~Janssen$^\textrm{\scriptsize 24}$,    
M.~Janus$^\textrm{\scriptsize 52}$,    
P.A.~Janus$^\textrm{\scriptsize 83a}$,    
G.~Jarlskog$^\textrm{\scriptsize 96}$,    
N.~Javadov$^\textrm{\scriptsize 79,ai}$,    
T.~Jav\r{u}rek$^\textrm{\scriptsize 51}$,    
M.~Javurkova$^\textrm{\scriptsize 51}$,    
F.~Jeanneau$^\textrm{\scriptsize 144}$,    
L.~Jeanty$^\textrm{\scriptsize 18}$,    
J.~Jejelava$^\textrm{\scriptsize 159a,aj}$,    
A.~Jelinskas$^\textrm{\scriptsize 178}$,    
P.~Jenni$^\textrm{\scriptsize 51,c}$,    
J.~Jeong$^\textrm{\scriptsize 45}$,    
C.~Jeske$^\textrm{\scriptsize 178}$,    
S.~J\'ez\'equel$^\textrm{\scriptsize 5}$,    
H.~Ji$^\textrm{\scriptsize 181}$,    
J.~Jia$^\textrm{\scriptsize 154}$,    
H.~Jiang$^\textrm{\scriptsize 78}$,    
Y.~Jiang$^\textrm{\scriptsize 59a}$,    
Z.~Jiang$^\textrm{\scriptsize 152}$,    
S.~Jiggins$^\textrm{\scriptsize 51}$,    
F.A.~Jimenez~Morales$^\textrm{\scriptsize 38}$,    
J.~Jimenez~Pena$^\textrm{\scriptsize 174}$,    
S.~Jin$^\textrm{\scriptsize 15c}$,    
A.~Jinaru$^\textrm{\scriptsize 27b}$,    
O.~Jinnouchi$^\textrm{\scriptsize 165}$,    
H.~Jivan$^\textrm{\scriptsize 33e}$,    
P.~Johansson$^\textrm{\scriptsize 148}$,    
K.A.~Johns$^\textrm{\scriptsize 7}$,    
C.A.~Johnson$^\textrm{\scriptsize 65}$,    
W.J.~Johnson$^\textrm{\scriptsize 147}$,    
K.~Jon-And$^\textrm{\scriptsize 44a,44b}$,    
R.W.L.~Jones$^\textrm{\scriptsize 89}$,    
S.D.~Jones$^\textrm{\scriptsize 155}$,    
S.~Jones$^\textrm{\scriptsize 7}$,    
T.J.~Jones$^\textrm{\scriptsize 90}$,    
J.~Jongmanns$^\textrm{\scriptsize 60a}$,    
P.M.~Jorge$^\textrm{\scriptsize 139a,139b}$,    
J.~Jovicevic$^\textrm{\scriptsize 168a}$,    
X.~Ju$^\textrm{\scriptsize 181}$,    
J.J.~Junggeburth$^\textrm{\scriptsize 114}$,    
A.~Juste~Rozas$^\textrm{\scriptsize 14,ac}$,    
A.~Kaczmarska$^\textrm{\scriptsize 84}$,    
M.~Kado$^\textrm{\scriptsize 64}$,    
H.~Kagan$^\textrm{\scriptsize 126}$,    
M.~Kagan$^\textrm{\scriptsize 152}$,    
T.~Kaji$^\textrm{\scriptsize 179}$,    
E.~Kajomovitz$^\textrm{\scriptsize 160}$,    
C.W.~Kalderon$^\textrm{\scriptsize 96}$,    
A.~Kaluza$^\textrm{\scriptsize 99}$,    
S.~Kama$^\textrm{\scriptsize 42}$,    
A.~Kamenshchikov$^\textrm{\scriptsize 122}$,    
L.~Kanjir$^\textrm{\scriptsize 91}$,    
Y.~Kano$^\textrm{\scriptsize 163}$,    
V.A.~Kantserov$^\textrm{\scriptsize 111}$,    
J.~Kanzaki$^\textrm{\scriptsize 81}$,    
B.~Kaplan$^\textrm{\scriptsize 124}$,    
L.S.~Kaplan$^\textrm{\scriptsize 181}$,    
D.~Kar$^\textrm{\scriptsize 33e}$,    
M.J.~Kareem$^\textrm{\scriptsize 168b}$,    
E.~Karentzos$^\textrm{\scriptsize 10}$,    
S.N.~Karpov$^\textrm{\scriptsize 79}$,    
Z.M.~Karpova$^\textrm{\scriptsize 79}$,    
V.~Kartvelishvili$^\textrm{\scriptsize 89}$,    
A.N.~Karyukhin$^\textrm{\scriptsize 122}$,    
K.~Kasahara$^\textrm{\scriptsize 169}$,    
L.~Kashif$^\textrm{\scriptsize 181}$,    
R.D.~Kass$^\textrm{\scriptsize 126}$,    
A.~Kastanas$^\textrm{\scriptsize 153}$,    
Y.~Kataoka$^\textrm{\scriptsize 163}$,    
C.~Kato$^\textrm{\scriptsize 163}$,    
A.~Katre$^\textrm{\scriptsize 53}$,    
J.~Katzy$^\textrm{\scriptsize 45}$,    
K.~Kawade$^\textrm{\scriptsize 82}$,    
K.~Kawagoe$^\textrm{\scriptsize 87}$,    
T.~Kawamoto$^\textrm{\scriptsize 163}$,    
G.~Kawamura$^\textrm{\scriptsize 52}$,    
E.F.~Kay$^\textrm{\scriptsize 90}$,    
V.F.~Kazanin$^\textrm{\scriptsize 121b,121a}$,    
R.~Keeler$^\textrm{\scriptsize 176}$,    
R.~Kehoe$^\textrm{\scriptsize 42}$,    
J.S.~Keller$^\textrm{\scriptsize 34}$,    
E.~Kellermann$^\textrm{\scriptsize 96}$,    
J.J.~Kempster$^\textrm{\scriptsize 21}$,    
J.~Kendrick$^\textrm{\scriptsize 21}$,    
O.~Kepka$^\textrm{\scriptsize 140}$,    
S.~Kersten$^\textrm{\scriptsize 182}$,    
B.P.~Ker\v{s}evan$^\textrm{\scriptsize 91}$,    
R.A.~Keyes$^\textrm{\scriptsize 103}$,    
M.~Khader$^\textrm{\scriptsize 173}$,    
F.~Khalil-Zada$^\textrm{\scriptsize 13}$,    
A.~Khanov$^\textrm{\scriptsize 129}$,    
A.G.~Kharlamov$^\textrm{\scriptsize 121b,121a}$,    
T.~Kharlamova$^\textrm{\scriptsize 121b,121a}$,    
A.~Khodinov$^\textrm{\scriptsize 166}$,    
T.J.~Khoo$^\textrm{\scriptsize 53}$,    
V.~Khovanskiy$^\textrm{\scriptsize 123,*}$,    
E.~Khramov$^\textrm{\scriptsize 79}$,    
J.~Khubua$^\textrm{\scriptsize 159b}$,    
S.~Kido$^\textrm{\scriptsize 82}$,    
M.~Kiehn$^\textrm{\scriptsize 53}$,    
C.R.~Kilby$^\textrm{\scriptsize 93}$,    
H.Y.~Kim$^\textrm{\scriptsize 8}$,    
S.H.~Kim$^\textrm{\scriptsize 169}$,    
Y.K.~Kim$^\textrm{\scriptsize 37}$,    
N.~Kimura$^\textrm{\scriptsize 66a,66c}$,    
O.M.~Kind$^\textrm{\scriptsize 19}$,    
B.T.~King$^\textrm{\scriptsize 90,*}$,    
D.~Kirchmeier$^\textrm{\scriptsize 47}$,    
J.~Kirk$^\textrm{\scriptsize 143}$,    
A.E.~Kiryunin$^\textrm{\scriptsize 114}$,    
T.~Kishimoto$^\textrm{\scriptsize 163}$,    
D.~Kisielewska$^\textrm{\scriptsize 83a}$,    
V.~Kitali$^\textrm{\scriptsize 45}$,    
O.~Kivernyk$^\textrm{\scriptsize 5}$,    
E.~Kladiva$^\textrm{\scriptsize 28b,*}$,    
T.~Klapdor-Kleingrothaus$^\textrm{\scriptsize 51}$,    
M.H.~Klein$^\textrm{\scriptsize 105}$,    
M.~Klein$^\textrm{\scriptsize 90}$,    
U.~Klein$^\textrm{\scriptsize 90}$,    
K.~Kleinknecht$^\textrm{\scriptsize 99}$,    
P.~Klimek$^\textrm{\scriptsize 120}$,    
A.~Klimentov$^\textrm{\scriptsize 29}$,    
R.~Klingenberg$^\textrm{\scriptsize 46,*}$,    
T.~Klingl$^\textrm{\scriptsize 24}$,    
T.~Klioutchnikova$^\textrm{\scriptsize 36}$,    
F.F.~Klitzner$^\textrm{\scriptsize 113}$,    
P.~Kluit$^\textrm{\scriptsize 119}$,    
S.~Kluth$^\textrm{\scriptsize 114}$,    
E.~Kneringer$^\textrm{\scriptsize 76}$,    
E.B.F.G.~Knoops$^\textrm{\scriptsize 101}$,    
A.~Knue$^\textrm{\scriptsize 51}$,    
A.~Kobayashi$^\textrm{\scriptsize 163}$,    
D.~Kobayashi$^\textrm{\scriptsize 87}$,    
T.~Kobayashi$^\textrm{\scriptsize 163}$,    
M.~Kobel$^\textrm{\scriptsize 47}$,    
M.~Kocian$^\textrm{\scriptsize 152}$,    
P.~Kodys$^\textrm{\scriptsize 142}$,    
T.~Koffas$^\textrm{\scriptsize 34}$,    
E.~Koffeman$^\textrm{\scriptsize 119}$,    
L.A.~Kogan$^\textrm{\scriptsize 134}$,    
N.M.~K\"ohler$^\textrm{\scriptsize 114}$,    
T.~Koi$^\textrm{\scriptsize 152}$,    
M.~Kolb$^\textrm{\scriptsize 60b}$,    
I.~Koletsou$^\textrm{\scriptsize 5}$,    
T.~Kondo$^\textrm{\scriptsize 81}$,    
N.~Kondrashova$^\textrm{\scriptsize 59c}$,    
K.~K\"oneke$^\textrm{\scriptsize 51}$,    
A.C.~K\"onig$^\textrm{\scriptsize 118}$,    
T.~Kono$^\textrm{\scriptsize 125,aq}$,    
R.~Konoplich$^\textrm{\scriptsize 124,am}$,    
N.~Konstantinidis$^\textrm{\scriptsize 94}$,    
B.~Konya$^\textrm{\scriptsize 96}$,    
R.~Kopeliansky$^\textrm{\scriptsize 65}$,    
S.~Koperny$^\textrm{\scriptsize 83a}$,    
K.~Korcyl$^\textrm{\scriptsize 84}$,    
K.~Kordas$^\textrm{\scriptsize 162}$,    
A.~Korn$^\textrm{\scriptsize 94}$,    
I.~Korolkov$^\textrm{\scriptsize 14}$,    
E.V.~Korolkova$^\textrm{\scriptsize 148}$,    
O.~Kortner$^\textrm{\scriptsize 114}$,    
S.~Kortner$^\textrm{\scriptsize 114}$,    
T.~Kosek$^\textrm{\scriptsize 142}$,    
V.V.~Kostyukhin$^\textrm{\scriptsize 24}$,    
A.~Kotwal$^\textrm{\scriptsize 48}$,    
A.~Koulouris$^\textrm{\scriptsize 10}$,    
A.~Kourkoumeli-Charalampidi$^\textrm{\scriptsize 70a,70b}$,    
C.~Kourkoumelis$^\textrm{\scriptsize 9}$,    
E.~Kourlitis$^\textrm{\scriptsize 148}$,    
V.~Kouskoura$^\textrm{\scriptsize 29}$,    
A.B.~Kowalewska$^\textrm{\scriptsize 84}$,    
R.~Kowalewski$^\textrm{\scriptsize 176}$,    
T.Z.~Kowalski$^\textrm{\scriptsize 83a}$,    
C.~Kozakai$^\textrm{\scriptsize 163}$,    
W.~Kozanecki$^\textrm{\scriptsize 144}$,    
A.S.~Kozhin$^\textrm{\scriptsize 122}$,    
V.A.~Kramarenko$^\textrm{\scriptsize 112}$,    
G.~Kramberger$^\textrm{\scriptsize 91}$,    
D.~Krasnopevtsev$^\textrm{\scriptsize 111}$,    
M.W.~Krasny$^\textrm{\scriptsize 135}$,    
A.~Krasznahorkay$^\textrm{\scriptsize 36}$,    
D.~Krauss$^\textrm{\scriptsize 114}$,    
J.A.~Kremer$^\textrm{\scriptsize 83a}$,    
J.~Kretzschmar$^\textrm{\scriptsize 90}$,    
K.~Kreutzfeldt$^\textrm{\scriptsize 55}$,    
P.~Krieger$^\textrm{\scriptsize 167}$,    
K.~Krizka$^\textrm{\scriptsize 18}$,    
K.~Kroeninger$^\textrm{\scriptsize 46}$,    
H.~Kroha$^\textrm{\scriptsize 114}$,    
J.~Kroll$^\textrm{\scriptsize 140}$,    
J.~Kroll$^\textrm{\scriptsize 136}$,    
J.~Kroseberg$^\textrm{\scriptsize 24}$,    
J.~Krstic$^\textrm{\scriptsize 16}$,    
U.~Kruchonak$^\textrm{\scriptsize 79}$,    
H.~Kr\"uger$^\textrm{\scriptsize 24}$,    
N.~Krumnack$^\textrm{\scriptsize 78}$,    
M.C.~Kruse$^\textrm{\scriptsize 48}$,    
T.~Kubota$^\textrm{\scriptsize 104}$,    
S.~Kuday$^\textrm{\scriptsize 4b}$,    
J.T.~Kuechler$^\textrm{\scriptsize 182}$,    
S.~Kuehn$^\textrm{\scriptsize 36}$,    
A.~Kugel$^\textrm{\scriptsize 60a}$,    
F.~Kuger$^\textrm{\scriptsize 177}$,    
T.~Kuhl$^\textrm{\scriptsize 45}$,    
V.~Kukhtin$^\textrm{\scriptsize 79}$,    
R.~Kukla$^\textrm{\scriptsize 101}$,    
Y.~Kulchitsky$^\textrm{\scriptsize 107}$,    
S.~Kuleshov$^\textrm{\scriptsize 146c}$,    
Y.P.~Kulinich$^\textrm{\scriptsize 173}$,    
M.~Kuna$^\textrm{\scriptsize 57}$,    
T.~Kunigo$^\textrm{\scriptsize 85}$,    
A.~Kupco$^\textrm{\scriptsize 140}$,    
T.~Kupfer$^\textrm{\scriptsize 46}$,    
O.~Kuprash$^\textrm{\scriptsize 161}$,    
H.~Kurashige$^\textrm{\scriptsize 82}$,    
L.L.~Kurchaninov$^\textrm{\scriptsize 168a}$,    
Y.A.~Kurochkin$^\textrm{\scriptsize 107}$,    
M.G.~Kurth$^\textrm{\scriptsize 15a,15d}$,    
E.S.~Kuwertz$^\textrm{\scriptsize 176}$,    
M.~Kuze$^\textrm{\scriptsize 165}$,    
J.~Kvita$^\textrm{\scriptsize 130}$,    
T.~Kwan$^\textrm{\scriptsize 176}$,    
A.~La~Rosa$^\textrm{\scriptsize 114}$,    
J.L.~La~Rosa~Navarro$^\textrm{\scriptsize 80d}$,    
L.~La~Rotonda$^\textrm{\scriptsize 41b,41a}$,    
F.~La~Ruffa$^\textrm{\scriptsize 41b,41a}$,    
C.~Lacasta$^\textrm{\scriptsize 174}$,    
F.~Lacava$^\textrm{\scriptsize 72a,72b}$,    
J.~Lacey$^\textrm{\scriptsize 45}$,    
D.P.J.~Lack$^\textrm{\scriptsize 100}$,    
H.~Lacker$^\textrm{\scriptsize 19}$,    
D.~Lacour$^\textrm{\scriptsize 135}$,    
E.~Ladygin$^\textrm{\scriptsize 79}$,    
R.~Lafaye$^\textrm{\scriptsize 5}$,    
B.~Laforge$^\textrm{\scriptsize 135}$,    
S.~Lai$^\textrm{\scriptsize 52}$,    
S.~Lammers$^\textrm{\scriptsize 65}$,    
W.~Lampl$^\textrm{\scriptsize 7}$,    
E.~Lan\c{c}on$^\textrm{\scriptsize 29}$,    
U.~Landgraf$^\textrm{\scriptsize 51}$,    
M.P.J.~Landon$^\textrm{\scriptsize 92}$,    
M.C.~Lanfermann$^\textrm{\scriptsize 53}$,    
V.S.~Lang$^\textrm{\scriptsize 45}$,    
J.C.~Lange$^\textrm{\scriptsize 14}$,    
R.J.~Langenberg$^\textrm{\scriptsize 36}$,    
A.J.~Lankford$^\textrm{\scriptsize 171}$,    
F.~Lanni$^\textrm{\scriptsize 29}$,    
K.~Lantzsch$^\textrm{\scriptsize 24}$,    
A.~Lanza$^\textrm{\scriptsize 70a}$,    
A.~Lapertosa$^\textrm{\scriptsize 54b,54a}$,    
S.~Laplace$^\textrm{\scriptsize 135}$,    
J.F.~Laporte$^\textrm{\scriptsize 144}$,    
T.~Lari$^\textrm{\scriptsize 68a}$,    
F.~Lasagni~Manghi$^\textrm{\scriptsize 23b,23a}$,    
M.~Lassnig$^\textrm{\scriptsize 36}$,    
T.S.~Lau$^\textrm{\scriptsize 62a}$,    
A.~Laudrain$^\textrm{\scriptsize 64}$,    
A.T.~Law$^\textrm{\scriptsize 145}$,    
P.~Laycock$^\textrm{\scriptsize 90}$,    
M.~Lazzaroni$^\textrm{\scriptsize 68a,68b}$,    
B.~Le$^\textrm{\scriptsize 104}$,    
O.~Le~Dortz$^\textrm{\scriptsize 135}$,    
E.~Le~Guirriec$^\textrm{\scriptsize 101}$,    
E.P.~Le~Quilleuc$^\textrm{\scriptsize 144}$,    
M.~LeBlanc$^\textrm{\scriptsize 7}$,    
T.~LeCompte$^\textrm{\scriptsize 6}$,    
F.~Ledroit-Guillon$^\textrm{\scriptsize 57}$,    
C.A.~Lee$^\textrm{\scriptsize 29}$,    
G.R.~Lee$^\textrm{\scriptsize 146a}$,    
L.~Lee$^\textrm{\scriptsize 58}$,    
S.C.~Lee$^\textrm{\scriptsize 157}$,    
B.~Lefebvre$^\textrm{\scriptsize 103}$,    
G.~Lefebvre$^\textrm{\scriptsize 135}$,    
M.~Lefebvre$^\textrm{\scriptsize 176}$,    
F.~Legger$^\textrm{\scriptsize 113}$,    
C.~Leggett$^\textrm{\scriptsize 18}$,    
G.~Lehmann~Miotto$^\textrm{\scriptsize 36}$,    
W.A.~Leight$^\textrm{\scriptsize 45}$,    
A.~Leisos$^\textrm{\scriptsize 162,y}$,    
M.A.L.~Leite$^\textrm{\scriptsize 80d}$,    
R.~Leitner$^\textrm{\scriptsize 142}$,    
D.~Lellouch$^\textrm{\scriptsize 180,*}$,    
B.~Lemmer$^\textrm{\scriptsize 52}$,    
K.J.C.~Leney$^\textrm{\scriptsize 94}$,    
T.~Lenz$^\textrm{\scriptsize 24}$,    
B.~Lenzi$^\textrm{\scriptsize 36}$,    
R.~Leone$^\textrm{\scriptsize 7}$,    
S.~Leone$^\textrm{\scriptsize 71a}$,    
C.~Leonidopoulos$^\textrm{\scriptsize 49}$,    
G.~Lerner$^\textrm{\scriptsize 155}$,    
C.~Leroy$^\textrm{\scriptsize 109}$,    
R.~Les$^\textrm{\scriptsize 167}$,    
A.A.J.~Lesage$^\textrm{\scriptsize 144}$,    
C.G.~Lester$^\textrm{\scriptsize 32}$,    
M.~Levchenko$^\textrm{\scriptsize 137}$,    
J.~Lev\^eque$^\textrm{\scriptsize 5}$,    
D.~Levin$^\textrm{\scriptsize 105}$,    
L.J.~Levinson$^\textrm{\scriptsize 180}$,    
D.~Lewis$^\textrm{\scriptsize 92}$,    
B.~Li$^\textrm{\scriptsize 59a,t}$,    
C-Q.~Li$^\textrm{\scriptsize 59a,al}$,    
H.~Li$^\textrm{\scriptsize 59b}$,    
L.~Li$^\textrm{\scriptsize 59c}$,    
Q.~Li$^\textrm{\scriptsize 15a,15d}$,    
Q.Y.~Li$^\textrm{\scriptsize 59a}$,    
S.~Li$^\textrm{\scriptsize 59d,59c}$,    
X.~Li$^\textrm{\scriptsize 59c}$,    
Y.~Li$^\textrm{\scriptsize 150}$,    
Z.~Liang$^\textrm{\scriptsize 15a}$,    
B.~Liberti$^\textrm{\scriptsize 73a}$,    
A.~Liblong$^\textrm{\scriptsize 167}$,    
K.~Lie$^\textrm{\scriptsize 62c}$,    
S.~Liem$^\textrm{\scriptsize 119}$,    
A.~Limosani$^\textrm{\scriptsize 156}$,    
C.Y.~Lin$^\textrm{\scriptsize 32}$,    
K.~Lin$^\textrm{\scriptsize 106}$,    
S.C.~Lin$^\textrm{\scriptsize 158}$,    
T.H.~Lin$^\textrm{\scriptsize 99}$,    
R.A.~Linck$^\textrm{\scriptsize 65}$,    
B.E.~Lindquist$^\textrm{\scriptsize 154}$,    
A.L.~Lionti$^\textrm{\scriptsize 53}$,    
E.~Lipeles$^\textrm{\scriptsize 136}$,    
A.~Lipniacka$^\textrm{\scriptsize 17}$,    
M.~Lisovyi$^\textrm{\scriptsize 60b}$,    
T.M.~Liss$^\textrm{\scriptsize 173,au}$,    
A.~Lister$^\textrm{\scriptsize 175}$,    
A.M.~Litke$^\textrm{\scriptsize 145}$,    
J.D.~Little$^\textrm{\scriptsize 8}$,    
B.~Liu$^\textrm{\scriptsize 78}$,    
B.L.~Liu$^\textrm{\scriptsize 6}$,    
H.B.~Liu$^\textrm{\scriptsize 29}$,    
H.~Liu$^\textrm{\scriptsize 105}$,    
J.B.~Liu$^\textrm{\scriptsize 59a}$,    
J.K.K.~Liu$^\textrm{\scriptsize 134}$,    
K.~Liu$^\textrm{\scriptsize 135}$,    
M.~Liu$^\textrm{\scriptsize 59a}$,    
P.~Liu$^\textrm{\scriptsize 18}$,    
Y.L.~Liu$^\textrm{\scriptsize 59a}$,    
Y.W.~Liu$^\textrm{\scriptsize 59a}$,    
M.~Livan$^\textrm{\scriptsize 70a,70b}$,    
A.~Lleres$^\textrm{\scriptsize 57}$,    
J.~Llorente~Merino$^\textrm{\scriptsize 15a}$,    
S.L.~Lloyd$^\textrm{\scriptsize 92}$,    
C.Y.~Lo$^\textrm{\scriptsize 62b}$,    
F.~Lo~Sterzo$^\textrm{\scriptsize 42}$,    
E.M.~Lobodzinska$^\textrm{\scriptsize 45}$,    
P.~Loch$^\textrm{\scriptsize 7}$,    
F.K.~Loebinger$^\textrm{\scriptsize 100}$,    
K.M.~Loew$^\textrm{\scriptsize 26}$,    
T.~Lohse$^\textrm{\scriptsize 19}$,    
K.~Lohwasser$^\textrm{\scriptsize 148}$,    
M.~Lokajicek$^\textrm{\scriptsize 140}$,    
B.A.~Long$^\textrm{\scriptsize 25}$,    
J.D.~Long$^\textrm{\scriptsize 173}$,    
R.E.~Long$^\textrm{\scriptsize 89}$,    
L.~Longo$^\textrm{\scriptsize 67a,67b}$,    
K.A.~Looper$^\textrm{\scriptsize 126}$,    
J.A.~Lopez$^\textrm{\scriptsize 146c}$,    
D.~Lopez~Mateos$^\textrm{\scriptsize 58}$,    
I.~Lopez~Paz$^\textrm{\scriptsize 14}$,    
A.~Lopez~Solis$^\textrm{\scriptsize 135}$,    
J.~Lorenz$^\textrm{\scriptsize 113}$,    
N.~Lorenzo~Martinez$^\textrm{\scriptsize 5}$,    
M.~Losada$^\textrm{\scriptsize 22}$,    
P.J.~L{\"o}sel$^\textrm{\scriptsize 113}$,    
A.~L\"osle$^\textrm{\scriptsize 51}$,    
X.~Lou$^\textrm{\scriptsize 45}$,    
X.~Lou$^\textrm{\scriptsize 15a}$,    
A.~Lounis$^\textrm{\scriptsize 64}$,    
J.~Love$^\textrm{\scriptsize 6}$,    
P.A.~Love$^\textrm{\scriptsize 89}$,    
J.J.~Lozano~Bahilo$^\textrm{\scriptsize 174}$,    
H.~Lu$^\textrm{\scriptsize 62a}$,    
N.~Lu$^\textrm{\scriptsize 105}$,    
Y.J.~Lu$^\textrm{\scriptsize 63}$,    
H.J.~Lubatti$^\textrm{\scriptsize 147}$,    
C.~Luci$^\textrm{\scriptsize 72a,72b}$,    
A.~Lucotte$^\textrm{\scriptsize 57}$,    
C.~Luedtke$^\textrm{\scriptsize 51}$,    
F.~Luehring$^\textrm{\scriptsize 65}$,    
I.~Luise$^\textrm{\scriptsize 135}$,    
W.~Lukas$^\textrm{\scriptsize 76}$,    
L.~Luminari$^\textrm{\scriptsize 72a}$,    
B.~Lund-Jensen$^\textrm{\scriptsize 153}$,    
M.S.~Lutz$^\textrm{\scriptsize 102}$,    
P.M.~Luzi$^\textrm{\scriptsize 135}$,    
D.~Lynn$^\textrm{\scriptsize 29}$,    
R.~Lysak$^\textrm{\scriptsize 140}$,    
E.~Lytken$^\textrm{\scriptsize 96}$,    
F.~Lyu$^\textrm{\scriptsize 15a}$,    
V.~Lyubushkin$^\textrm{\scriptsize 79}$,    
H.~Ma$^\textrm{\scriptsize 29}$,    
L.L.~Ma$^\textrm{\scriptsize 59b}$,    
Y.~Ma$^\textrm{\scriptsize 59b}$,    
G.~Maccarrone$^\textrm{\scriptsize 50}$,    
A.~Macchiolo$^\textrm{\scriptsize 114}$,    
C.M.~Macdonald$^\textrm{\scriptsize 148}$,    
J.~Machado~Miguens$^\textrm{\scriptsize 136,139b}$,    
D.~Madaffari$^\textrm{\scriptsize 174}$,    
R.~Madar$^\textrm{\scriptsize 38}$,    
W.F.~Mader$^\textrm{\scriptsize 47}$,    
A.~Madsen$^\textrm{\scriptsize 45}$,    
N.~Madysa$^\textrm{\scriptsize 47}$,    
J.~Maeda$^\textrm{\scriptsize 82}$,    
S.~Maeland$^\textrm{\scriptsize 17}$,    
T.~Maeno$^\textrm{\scriptsize 29}$,    
A.S.~Maevskiy$^\textrm{\scriptsize 112}$,    
V.~Magerl$^\textrm{\scriptsize 51}$,    
C.~Maidantchik$^\textrm{\scriptsize 80b}$,    
T.~Maier$^\textrm{\scriptsize 113}$,    
A.~Maio$^\textrm{\scriptsize 139a,139b,139d}$,    
K.~Maj$^\textrm{\scriptsize 84}$,    
O.~Majersky$^\textrm{\scriptsize 28a}$,    
S.~Majewski$^\textrm{\scriptsize 131}$,    
Y.~Makida$^\textrm{\scriptsize 81}$,    
N.~Makovec$^\textrm{\scriptsize 64}$,    
B.~Malaescu$^\textrm{\scriptsize 135}$,    
Pa.~Malecki$^\textrm{\scriptsize 84}$,    
V.P.~Maleev$^\textrm{\scriptsize 137}$,    
F.~Malek$^\textrm{\scriptsize 57}$,    
U.~Mallik$^\textrm{\scriptsize 77}$,    
D.~Malon$^\textrm{\scriptsize 6}$,    
C.~Malone$^\textrm{\scriptsize 32}$,    
S.~Maltezos$^\textrm{\scriptsize 10}$,    
S.~Malyukov$^\textrm{\scriptsize 36}$,    
J.~Mamuzic$^\textrm{\scriptsize 174}$,    
G.~Mancini$^\textrm{\scriptsize 50}$,    
I.~Mandi\'{c}$^\textrm{\scriptsize 91}$,    
J.~Maneira$^\textrm{\scriptsize 139a}$,    
L.~Manhaes~de~Andrade~Filho$^\textrm{\scriptsize 80a}$,    
J.~Manjarres~Ramos$^\textrm{\scriptsize 47}$,    
K.H.~Mankinen$^\textrm{\scriptsize 96}$,    
A.~Mann$^\textrm{\scriptsize 113}$,    
A.~Manousos$^\textrm{\scriptsize 76}$,    
B.~Mansoulie$^\textrm{\scriptsize 144}$,    
J.D.~Mansour$^\textrm{\scriptsize 15a}$,    
R.~Mantifel$^\textrm{\scriptsize 103}$,    
M.~Mantoani$^\textrm{\scriptsize 52}$,    
S.~Manzoni$^\textrm{\scriptsize 68a,68b}$,    
G.~Marceca$^\textrm{\scriptsize 30}$,    
L.~March$^\textrm{\scriptsize 53}$,    
L.~Marchese$^\textrm{\scriptsize 134}$,    
G.~Marchiori$^\textrm{\scriptsize 135}$,    
M.~Marcisovsky$^\textrm{\scriptsize 140}$,    
C.A.~Marin~Tobon$^\textrm{\scriptsize 36}$,    
M.~Marjanovic$^\textrm{\scriptsize 38}$,    
D.E.~Marley$^\textrm{\scriptsize 105}$,    
F.~Marroquim$^\textrm{\scriptsize 80b}$,    
Z.~Marshall$^\textrm{\scriptsize 18}$,    
M.U.F.~Martensson$^\textrm{\scriptsize 172}$,    
S.~Marti-Garcia$^\textrm{\scriptsize 174}$,    
C.B.~Martin$^\textrm{\scriptsize 126}$,    
T.A.~Martin$^\textrm{\scriptsize 178}$,    
V.J.~Martin$^\textrm{\scriptsize 49}$,    
B.~Martin~dit~Latour$^\textrm{\scriptsize 17}$,    
M.~Martinez$^\textrm{\scriptsize 14,ac}$,    
V.I.~Martinez~Outschoorn$^\textrm{\scriptsize 102}$,    
S.~Martin-Haugh$^\textrm{\scriptsize 143}$,    
V.S.~Martoiu$^\textrm{\scriptsize 27b}$,    
A.C.~Martyniuk$^\textrm{\scriptsize 94}$,    
A.~Marzin$^\textrm{\scriptsize 36}$,    
L.~Masetti$^\textrm{\scriptsize 99}$,    
T.~Mashimo$^\textrm{\scriptsize 163}$,    
R.~Mashinistov$^\textrm{\scriptsize 110}$,    
J.~Masik$^\textrm{\scriptsize 100}$,    
A.L.~Maslennikov$^\textrm{\scriptsize 121b,121a}$,    
L.H.~Mason$^\textrm{\scriptsize 104}$,    
L.~Massa$^\textrm{\scriptsize 73a,73b}$,    
P.~Mastrandrea$^\textrm{\scriptsize 5}$,    
A.~Mastroberardino$^\textrm{\scriptsize 41b,41a}$,    
T.~Masubuchi$^\textrm{\scriptsize 163}$,    
P.~M\"attig$^\textrm{\scriptsize 182}$,    
J.~Maurer$^\textrm{\scriptsize 27b}$,    
B.~Ma\v{c}ek$^\textrm{\scriptsize 91}$,    
S.J.~Maxfield$^\textrm{\scriptsize 90}$,    
D.A.~Maximov$^\textrm{\scriptsize 121b,121a}$,    
R.~Mazini$^\textrm{\scriptsize 157}$,    
I.~Maznas$^\textrm{\scriptsize 162}$,    
S.M.~Mazza$^\textrm{\scriptsize 145}$,    
N.C.~Mc~Fadden$^\textrm{\scriptsize 117}$,    
G.~Mc~Goldrick$^\textrm{\scriptsize 167}$,    
S.P.~Mc~Kee$^\textrm{\scriptsize 105}$,    
T.G.~McCarthy$^\textrm{\scriptsize 114}$,    
L.I.~McClymont$^\textrm{\scriptsize 94}$,    
E.F.~McDonald$^\textrm{\scriptsize 104}$,    
J.A.~Mcfayden$^\textrm{\scriptsize 36}$,    
M.A.~McKay$^\textrm{\scriptsize 42}$,    
K.D.~McLean$^\textrm{\scriptsize 176}$,    
S.J.~McMahon$^\textrm{\scriptsize 143}$,    
P.C.~McNamara$^\textrm{\scriptsize 104}$,    
C.J.~McNicol$^\textrm{\scriptsize 178}$,    
R.A.~McPherson$^\textrm{\scriptsize 176,ag}$,    
J.E.~Mdhluli$^\textrm{\scriptsize 33e}$,    
Z.A.~Meadows$^\textrm{\scriptsize 102}$,    
S.~Meehan$^\textrm{\scriptsize 147}$,    
T.~Megy$^\textrm{\scriptsize 51}$,    
S.~Mehlhase$^\textrm{\scriptsize 113}$,    
A.~Mehta$^\textrm{\scriptsize 90}$,    
T.~Meideck$^\textrm{\scriptsize 57}$,    
B.~Meirose$^\textrm{\scriptsize 43}$,    
D.~Melini$^\textrm{\scriptsize 174,g}$,    
B.R.~Mellado~Garcia$^\textrm{\scriptsize 33e}$,    
J.D.~Mellenthin$^\textrm{\scriptsize 52}$,    
M.~Melo$^\textrm{\scriptsize 28a}$,    
F.~Meloni$^\textrm{\scriptsize 20}$,    
A.~Melzer$^\textrm{\scriptsize 24}$,    
S.B.~Menary$^\textrm{\scriptsize 100}$,    
L.~Meng$^\textrm{\scriptsize 90}$,    
X.T.~Meng$^\textrm{\scriptsize 105}$,    
A.~Mengarelli$^\textrm{\scriptsize 23b,23a}$,    
S.~Menke$^\textrm{\scriptsize 114}$,    
E.~Meoni$^\textrm{\scriptsize 41b,41a}$,    
S.~Mergelmeyer$^\textrm{\scriptsize 19}$,    
C.~Merlassino$^\textrm{\scriptsize 20}$,    
P.~Mermod$^\textrm{\scriptsize 53}$,    
L.~Merola$^\textrm{\scriptsize 69a,69b}$,    
C.~Meroni$^\textrm{\scriptsize 68a}$,    
F.S.~Merritt$^\textrm{\scriptsize 37}$,    
A.~Messina$^\textrm{\scriptsize 72a,72b}$,    
J.~Metcalfe$^\textrm{\scriptsize 6}$,    
A.S.~Mete$^\textrm{\scriptsize 171}$,    
C.~Meyer$^\textrm{\scriptsize 136}$,    
J.~Meyer$^\textrm{\scriptsize 160}$,    
J-P.~Meyer$^\textrm{\scriptsize 144}$,    
H.~Meyer~Zu~Theenhausen$^\textrm{\scriptsize 60a}$,    
F.~Miano$^\textrm{\scriptsize 155}$,    
R.P.~Middleton$^\textrm{\scriptsize 143}$,    
L.~Mijovi\'{c}$^\textrm{\scriptsize 49}$,    
G.~Mikenberg$^\textrm{\scriptsize 180}$,    
M.~Mikestikova$^\textrm{\scriptsize 140}$,    
M.~Miku\v{z}$^\textrm{\scriptsize 91}$,    
M.~Milesi$^\textrm{\scriptsize 104}$,    
A.~Milic$^\textrm{\scriptsize 167}$,    
D.A.~Millar$^\textrm{\scriptsize 92}$,    
D.W.~Miller$^\textrm{\scriptsize 37}$,    
A.~Milov$^\textrm{\scriptsize 180}$,    
D.A.~Milstead$^\textrm{\scriptsize 44a,44b}$,    
A.A.~Minaenko$^\textrm{\scriptsize 122}$,    
I.A.~Minashvili$^\textrm{\scriptsize 159b}$,    
A.I.~Mincer$^\textrm{\scriptsize 124}$,    
B.~Mindur$^\textrm{\scriptsize 83a}$,    
M.~Mineev$^\textrm{\scriptsize 79}$,    
Y.~Minegishi$^\textrm{\scriptsize 163}$,    
Y.~Ming$^\textrm{\scriptsize 181}$,    
L.M.~Mir$^\textrm{\scriptsize 14}$,    
A.~Mirto$^\textrm{\scriptsize 67a,67b}$,    
K.P.~Mistry$^\textrm{\scriptsize 136}$,    
T.~Mitani$^\textrm{\scriptsize 179}$,    
J.~Mitrevski$^\textrm{\scriptsize 113}$,    
V.A.~Mitsou$^\textrm{\scriptsize 174}$,    
A.~Miucci$^\textrm{\scriptsize 20}$,    
P.S.~Miyagawa$^\textrm{\scriptsize 148}$,    
A.~Mizukami$^\textrm{\scriptsize 81}$,    
J.U.~Mj\"ornmark$^\textrm{\scriptsize 96}$,    
T.~Mkrtchyan$^\textrm{\scriptsize 184}$,    
M.~Mlynarikova$^\textrm{\scriptsize 142}$,    
T.~Moa$^\textrm{\scriptsize 44a,44b}$,    
K.~Mochizuki$^\textrm{\scriptsize 109}$,    
P.~Mogg$^\textrm{\scriptsize 51}$,    
S.~Mohapatra$^\textrm{\scriptsize 39}$,    
S.~Molander$^\textrm{\scriptsize 44a,44b}$,    
R.~Moles-Valls$^\textrm{\scriptsize 24}$,    
M.C.~Mondragon$^\textrm{\scriptsize 106}$,    
K.~M\"onig$^\textrm{\scriptsize 45}$,    
J.~Monk$^\textrm{\scriptsize 40}$,    
E.~Monnier$^\textrm{\scriptsize 101}$,    
A.~Montalbano$^\textrm{\scriptsize 151}$,    
J.~Montejo~Berlingen$^\textrm{\scriptsize 36}$,    
F.~Monticelli$^\textrm{\scriptsize 88}$,    
S.~Monzani$^\textrm{\scriptsize 68a}$,    
R.W.~Moore$^\textrm{\scriptsize 3}$,    
N.~Morange$^\textrm{\scriptsize 64}$,    
D.~Moreno$^\textrm{\scriptsize 22}$,    
M.~Moreno~Ll\'acer$^\textrm{\scriptsize 36}$,    
P.~Morettini$^\textrm{\scriptsize 54b}$,    
M.~Morgenstern$^\textrm{\scriptsize 119}$,    
S.~Morgenstern$^\textrm{\scriptsize 36}$,    
D.~Mori$^\textrm{\scriptsize 151}$,    
T.~Mori$^\textrm{\scriptsize 163}$,    
M.~Morii$^\textrm{\scriptsize 58}$,    
M.~Morinaga$^\textrm{\scriptsize 179}$,    
V.~Morisbak$^\textrm{\scriptsize 133}$,    
A.K.~Morley$^\textrm{\scriptsize 36}$,    
G.~Mornacchi$^\textrm{\scriptsize 36}$,    
J.D.~Morris$^\textrm{\scriptsize 92}$,    
L.~Morvaj$^\textrm{\scriptsize 154}$,    
P.~Moschovakos$^\textrm{\scriptsize 10}$,    
M.~Mosidze$^\textrm{\scriptsize 159b}$,    
H.J.~Moss$^\textrm{\scriptsize 148}$,    
J.~Moss$^\textrm{\scriptsize 31,o}$,    
K.~Motohashi$^\textrm{\scriptsize 165}$,    
R.~Mount$^\textrm{\scriptsize 152}$,    
E.~Mountricha$^\textrm{\scriptsize 29}$,    
E.J.W.~Moyse$^\textrm{\scriptsize 102}$,    
S.~Muanza$^\textrm{\scriptsize 101}$,    
F.~Mueller$^\textrm{\scriptsize 114}$,    
J.~Mueller$^\textrm{\scriptsize 138}$,    
R.S.P.~Mueller$^\textrm{\scriptsize 113}$,    
D.~Muenstermann$^\textrm{\scriptsize 89}$,    
P.~Mullen$^\textrm{\scriptsize 56}$,    
G.A.~Mullier$^\textrm{\scriptsize 20}$,    
F.J.~Munoz~Sanchez$^\textrm{\scriptsize 100}$,    
P.~Murin$^\textrm{\scriptsize 28b}$,    
W.J.~Murray$^\textrm{\scriptsize 178,143}$,    
A.~Murrone$^\textrm{\scriptsize 68a,68b}$,    
M.~Mu\v{s}kinja$^\textrm{\scriptsize 91}$,    
C.~Mwewa$^\textrm{\scriptsize 33a}$,    
A.G.~Myagkov$^\textrm{\scriptsize 122,an}$,    
J.~Myers$^\textrm{\scriptsize 131}$,    
M.~Myska$^\textrm{\scriptsize 141}$,    
B.P.~Nachman$^\textrm{\scriptsize 18}$,    
O.~Nackenhorst$^\textrm{\scriptsize 46}$,    
K.~Nagai$^\textrm{\scriptsize 134}$,    
R.~Nagai$^\textrm{\scriptsize 125}$,    
K.~Nagano$^\textrm{\scriptsize 81}$,    
Y.~Nagasaka$^\textrm{\scriptsize 61}$,    
K.~Nagata$^\textrm{\scriptsize 169}$,    
M.~Nagel$^\textrm{\scriptsize 51}$,    
E.~Nagy$^\textrm{\scriptsize 101}$,    
A.M.~Nairz$^\textrm{\scriptsize 36}$,    
Y.~Nakahama$^\textrm{\scriptsize 116}$,    
K.~Nakamura$^\textrm{\scriptsize 81}$,    
T.~Nakamura$^\textrm{\scriptsize 163}$,    
I.~Nakano$^\textrm{\scriptsize 127}$,    
F.~Napolitano$^\textrm{\scriptsize 60a}$,    
R.F.~Naranjo~Garcia$^\textrm{\scriptsize 45}$,    
R.~Narayan$^\textrm{\scriptsize 11}$,    
D.I.~Narrias~Villar$^\textrm{\scriptsize 60a}$,    
I.~Naryshkin$^\textrm{\scriptsize 137}$,    
T.~Naumann$^\textrm{\scriptsize 45}$,    
G.~Navarro$^\textrm{\scriptsize 22}$,    
R.~Nayyar$^\textrm{\scriptsize 7}$,    
H.A.~Neal$^\textrm{\scriptsize 105,*}$,    
P.Y.~Nechaeva$^\textrm{\scriptsize 110}$,    
T.J.~Neep$^\textrm{\scriptsize 144}$,    
A.~Negri$^\textrm{\scriptsize 70a,70b}$,    
M.~Negrini$^\textrm{\scriptsize 23b}$,    
S.~Nektarijevic$^\textrm{\scriptsize 118}$,    
C.~Nellist$^\textrm{\scriptsize 52}$,    
M.E.~Nelson$^\textrm{\scriptsize 134}$,    
S.~Nemecek$^\textrm{\scriptsize 140}$,    
P.~Nemethy$^\textrm{\scriptsize 124}$,    
M.~Nessi$^\textrm{\scriptsize 36,e}$,    
M.S.~Neubauer$^\textrm{\scriptsize 173}$,    
M.~Neumann$^\textrm{\scriptsize 182}$,    
P.R.~Newman$^\textrm{\scriptsize 21}$,    
T.Y.~Ng$^\textrm{\scriptsize 62c}$,    
Y.S.~Ng$^\textrm{\scriptsize 19}$,    
H.D.N.~Nguyen$^\textrm{\scriptsize 101}$,    
T.~Nguyen~Manh$^\textrm{\scriptsize 109}$,    
E.~Nibigira$^\textrm{\scriptsize 38}$,    
R.B.~Nickerson$^\textrm{\scriptsize 134}$,    
R.~Nicolaidou$^\textrm{\scriptsize 144}$,    
J.~Nielsen$^\textrm{\scriptsize 145}$,    
N.~Nikiforou$^\textrm{\scriptsize 11}$,    
V.~Nikolaenko$^\textrm{\scriptsize 122,an}$,    
I.~Nikolic-Audit$^\textrm{\scriptsize 135}$,    
K.~Nikolopoulos$^\textrm{\scriptsize 21}$,    
P.~Nilsson$^\textrm{\scriptsize 29}$,    
Y.~Ninomiya$^\textrm{\scriptsize 81}$,    
A.~Nisati$^\textrm{\scriptsize 72a}$,    
N.~Nishu$^\textrm{\scriptsize 59c}$,    
R.~Nisius$^\textrm{\scriptsize 114}$,    
I.~Nitsche$^\textrm{\scriptsize 46}$,    
T.~Nitta$^\textrm{\scriptsize 179}$,    
T.~Nobe$^\textrm{\scriptsize 163}$,    
Y.~Noguchi$^\textrm{\scriptsize 85}$,    
M.~Nomachi$^\textrm{\scriptsize 132}$,    
I.~Nomidis$^\textrm{\scriptsize 34}$,    
M.A.~Nomura$^\textrm{\scriptsize 29}$,    
T.~Nooney$^\textrm{\scriptsize 92}$,    
M.~Nordberg$^\textrm{\scriptsize 36}$,    
N.~Norjoharuddeen$^\textrm{\scriptsize 134}$,    
T.~Novak$^\textrm{\scriptsize 91}$,    
O.~Novgorodova$^\textrm{\scriptsize 47}$,    
R.~Novotny$^\textrm{\scriptsize 141}$,    
M.~Nozaki$^\textrm{\scriptsize 81}$,    
L.~Nozka$^\textrm{\scriptsize 130}$,    
K.~Ntekas$^\textrm{\scriptsize 171}$,    
E.~Nurse$^\textrm{\scriptsize 94}$,    
F.~Nuti$^\textrm{\scriptsize 104}$,    
F.G.~Oakham$^\textrm{\scriptsize 34,ax}$,    
H.~Oberlack$^\textrm{\scriptsize 114}$,    
T.~Obermann$^\textrm{\scriptsize 24}$,    
J.~Ocariz$^\textrm{\scriptsize 135}$,    
A.~Ochi$^\textrm{\scriptsize 82}$,    
I.~Ochoa$^\textrm{\scriptsize 39}$,    
J.P.~Ochoa-Ricoux$^\textrm{\scriptsize 146a}$,    
K.~O'Connor$^\textrm{\scriptsize 26}$,    
S.~Oda$^\textrm{\scriptsize 87}$,    
S.~Odaka$^\textrm{\scriptsize 81}$,    
A.~Oh$^\textrm{\scriptsize 100}$,    
S.H.~Oh$^\textrm{\scriptsize 48}$,    
C.C.~Ohm$^\textrm{\scriptsize 153}$,    
H.~Ohman$^\textrm{\scriptsize 172}$,    
H.~Oide$^\textrm{\scriptsize 54b,54a}$,    
H.~Okawa$^\textrm{\scriptsize 169}$,    
Y.~Okazaki$^\textrm{\scriptsize 85}$,    
Y.~Okumura$^\textrm{\scriptsize 163}$,    
T.~Okuyama$^\textrm{\scriptsize 81}$,    
A.~Olariu$^\textrm{\scriptsize 27b}$,    
L.F.~Oleiro~Seabra$^\textrm{\scriptsize 139a}$,    
S.A.~Olivares~Pino$^\textrm{\scriptsize 146a}$,    
D.~Oliveira~Damazio$^\textrm{\scriptsize 29}$,    
J.L.~Oliver$^\textrm{\scriptsize 1}$,    
M.J.R.~Olsson$^\textrm{\scriptsize 37}$,    
A.~Olszewski$^\textrm{\scriptsize 84}$,    
J.~Olszowska$^\textrm{\scriptsize 84}$,    
D.C.~O'Neil$^\textrm{\scriptsize 151}$,    
A.~Onofre$^\textrm{\scriptsize 139a,139e}$,    
K.~Onogi$^\textrm{\scriptsize 116}$,    
P.U.E.~Onyisi$^\textrm{\scriptsize 11}$,    
H.~Oppen$^\textrm{\scriptsize 133}$,    
M.J.~Oreglia$^\textrm{\scriptsize 37}$,    
Y.~Oren$^\textrm{\scriptsize 161,*}$,    
D.~Orestano$^\textrm{\scriptsize 74a,74b}$,    
N.~Orlando$^\textrm{\scriptsize 62b}$,    
A.A.~O'Rourke$^\textrm{\scriptsize 45}$,    
R.S.~Orr$^\textrm{\scriptsize 167}$,    
B.~Osculati$^\textrm{\scriptsize 54b,54a,*}$,    
V.~O'Shea$^\textrm{\scriptsize 56}$,    
R.~Ospanov$^\textrm{\scriptsize 59a}$,    
G.~Otero~y~Garzon$^\textrm{\scriptsize 30}$,    
H.~Otono$^\textrm{\scriptsize 87}$,    
M.~Ouchrif$^\textrm{\scriptsize 35d}$,    
F.~Ould-Saada$^\textrm{\scriptsize 133}$,    
A.~Ouraou$^\textrm{\scriptsize 144}$,    
Q.~Ouyang$^\textrm{\scriptsize 15a}$,    
M.~Owen$^\textrm{\scriptsize 56}$,    
R.E.~Owen$^\textrm{\scriptsize 21}$,    
V.E.~Ozcan$^\textrm{\scriptsize 12c}$,    
N.~Ozturk$^\textrm{\scriptsize 8}$,    
K.~Pachal$^\textrm{\scriptsize 151}$,    
A.~Pacheco~Pages$^\textrm{\scriptsize 14}$,    
L.~Pacheco~Rodriguez$^\textrm{\scriptsize 144}$,    
C.~Padilla~Aranda$^\textrm{\scriptsize 14}$,    
S.~Pagan~Griso$^\textrm{\scriptsize 18}$,    
M.~Paganini$^\textrm{\scriptsize 183}$,    
G.~Palacino$^\textrm{\scriptsize 65}$,    
S.~Palazzo$^\textrm{\scriptsize 41b,41a}$,    
S.~Palestini$^\textrm{\scriptsize 36}$,    
M.~Palka$^\textrm{\scriptsize 83b}$,    
D.~Pallin$^\textrm{\scriptsize 38}$,    
I.~Panagoulias$^\textrm{\scriptsize 10}$,    
C.E.~Pandini$^\textrm{\scriptsize 53}$,    
J.G.~Panduro~Vazquez$^\textrm{\scriptsize 93}$,    
P.~Pani$^\textrm{\scriptsize 36}$,    
L.~Paolozzi$^\textrm{\scriptsize 53}$,    
T.D.~Papadopoulou$^\textrm{\scriptsize 10}$,    
K.~Papageorgiou$^\textrm{\scriptsize 9,i}$,    
A.~Paramonov$^\textrm{\scriptsize 6}$,    
D.~Paredes~Hernandez$^\textrm{\scriptsize 62b}$,    
B.~Parida$^\textrm{\scriptsize 59c}$,    
A.J.~Parker$^\textrm{\scriptsize 89}$,    
K.A.~Parker$^\textrm{\scriptsize 45}$,    
M.A.~Parker$^\textrm{\scriptsize 32}$,    
F.~Parodi$^\textrm{\scriptsize 54b,54a}$,    
J.A.~Parsons$^\textrm{\scriptsize 39}$,    
U.~Parzefall$^\textrm{\scriptsize 51}$,    
V.R.~Pascuzzi$^\textrm{\scriptsize 167}$,    
J.M.P.~Pasner$^\textrm{\scriptsize 145}$,    
E.~Pasqualucci$^\textrm{\scriptsize 72a}$,    
S.~Passaggio$^\textrm{\scriptsize 54b}$,    
F.~Pastore$^\textrm{\scriptsize 93}$,    
P.~Pasuwan$^\textrm{\scriptsize 44a,44b}$,    
S.~Pataraia$^\textrm{\scriptsize 99}$,    
J.R.~Pater$^\textrm{\scriptsize 100}$,    
A.~Pathak$^\textrm{\scriptsize 181}$,    
T.~Pauly$^\textrm{\scriptsize 36}$,    
B.~Pearson$^\textrm{\scriptsize 114}$,    
S.~Pedraza~Lopez$^\textrm{\scriptsize 174}$,    
R.~Pedro$^\textrm{\scriptsize 139a,139b}$,    
S.V.~Peleganchuk$^\textrm{\scriptsize 121b,121a}$,    
O.~Penc$^\textrm{\scriptsize 140}$,    
C.~Peng$^\textrm{\scriptsize 15a}$,    
H.~Peng$^\textrm{\scriptsize 59a}$,    
J.~Penwell$^\textrm{\scriptsize 65}$,    
B.S.~Peralva$^\textrm{\scriptsize 80a}$,    
M.M.~Perego$^\textrm{\scriptsize 144}$,    
A.P.~Pereira~Peixoto$^\textrm{\scriptsize 139a}$,    
D.V.~Perepelitsa$^\textrm{\scriptsize 29}$,    
F.~Peri$^\textrm{\scriptsize 19}$,    
L.~Perini$^\textrm{\scriptsize 68a,68b}$,    
H.~Pernegger$^\textrm{\scriptsize 36}$,    
S.~Perrella$^\textrm{\scriptsize 69a,69b}$,    
V.D.~Peshekhonov$^\textrm{\scriptsize 79,*}$,    
K.~Peters$^\textrm{\scriptsize 45}$,    
R.F.Y.~Peters$^\textrm{\scriptsize 100}$,    
B.A.~Petersen$^\textrm{\scriptsize 36}$,    
T.C.~Petersen$^\textrm{\scriptsize 40}$,    
E.~Petit$^\textrm{\scriptsize 57}$,    
A.~Petridis$^\textrm{\scriptsize 1}$,    
C.~Petridou$^\textrm{\scriptsize 162}$,    
P.~Petroff$^\textrm{\scriptsize 64}$,    
E.~Petrolo$^\textrm{\scriptsize 72a}$,    
M.~Petrov$^\textrm{\scriptsize 134}$,    
F.~Petrucci$^\textrm{\scriptsize 74a,74b}$,    
N.E.~Pettersson$^\textrm{\scriptsize 102}$,    
A.~Peyaud$^\textrm{\scriptsize 144}$,    
R.~Pezoa$^\textrm{\scriptsize 146c}$,    
T.~Pham$^\textrm{\scriptsize 104}$,    
F.H.~Phillips$^\textrm{\scriptsize 106}$,    
P.W.~Phillips$^\textrm{\scriptsize 143}$,    
G.~Piacquadio$^\textrm{\scriptsize 154}$,    
E.~Pianori$^\textrm{\scriptsize 178}$,    
A.~Picazio$^\textrm{\scriptsize 102}$,    
M.A.~Pickering$^\textrm{\scriptsize 134}$,    
R.~Piegaia$^\textrm{\scriptsize 30}$,    
J.E.~Pilcher$^\textrm{\scriptsize 37}$,    
A.D.~Pilkington$^\textrm{\scriptsize 100}$,    
M.~Pinamonti$^\textrm{\scriptsize 73a,73b}$,    
J.L.~Pinfold$^\textrm{\scriptsize 3}$,    
M.~Pitt$^\textrm{\scriptsize 180}$,    
M.-A.~Pleier$^\textrm{\scriptsize 29}$,    
V.~Pleskot$^\textrm{\scriptsize 142}$,    
E.~Plotnikova$^\textrm{\scriptsize 79}$,    
D.~Pluth$^\textrm{\scriptsize 78}$,    
P.~Podberezko$^\textrm{\scriptsize 121b,121a}$,    
R.~Poettgen$^\textrm{\scriptsize 96}$,    
R.~Poggi$^\textrm{\scriptsize 70a,70b}$,    
L.~Poggioli$^\textrm{\scriptsize 64}$,    
I.~Pogrebnyak$^\textrm{\scriptsize 106}$,    
D.~Pohl$^\textrm{\scriptsize 24}$,    
I.~Pokharel$^\textrm{\scriptsize 52}$,    
G.~Polesello$^\textrm{\scriptsize 70a}$,    
A.~Poley$^\textrm{\scriptsize 45}$,    
A.~Policicchio$^\textrm{\scriptsize 41b,41a}$,    
R.~Polifka$^\textrm{\scriptsize 36}$,    
A.~Polini$^\textrm{\scriptsize 23b}$,    
C.S.~Pollard$^\textrm{\scriptsize 45}$,    
V.~Polychronakos$^\textrm{\scriptsize 29}$,    
D.~Ponomarenko$^\textrm{\scriptsize 111}$,    
L.~Pontecorvo$^\textrm{\scriptsize 72a}$,    
G.A.~Popeneciu$^\textrm{\scriptsize 27d}$,    
D.M.~Portillo~Quintero$^\textrm{\scriptsize 135}$,    
S.~Pospisil$^\textrm{\scriptsize 141}$,    
K.~Potamianos$^\textrm{\scriptsize 45}$,    
I.N.~Potrap$^\textrm{\scriptsize 79}$,    
C.J.~Potter$^\textrm{\scriptsize 32}$,    
H.~Potti$^\textrm{\scriptsize 11}$,    
T.~Poulsen$^\textrm{\scriptsize 96}$,    
J.~Poveda$^\textrm{\scriptsize 36}$,    
M.E.~Pozo~Astigarraga$^\textrm{\scriptsize 36}$,    
P.~Pralavorio$^\textrm{\scriptsize 101}$,    
S.~Prell$^\textrm{\scriptsize 78}$,    
D.~Price$^\textrm{\scriptsize 100}$,    
M.~Primavera$^\textrm{\scriptsize 67a}$,    
S.~Prince$^\textrm{\scriptsize 103}$,    
N.~Proklova$^\textrm{\scriptsize 111}$,    
K.~Prokofiev$^\textrm{\scriptsize 62c}$,    
F.~Prokoshin$^\textrm{\scriptsize 146c}$,    
S.~Protopopescu$^\textrm{\scriptsize 29}$,    
J.~Proudfoot$^\textrm{\scriptsize 6}$,    
M.~Przybycien$^\textrm{\scriptsize 83a}$,    
A.~Puri$^\textrm{\scriptsize 173}$,    
P.~Puzo$^\textrm{\scriptsize 64}$,    
J.~Qian$^\textrm{\scriptsize 105}$,    
Y.~Qin$^\textrm{\scriptsize 100}$,    
A.~Quadt$^\textrm{\scriptsize 52}$,    
M.~Queitsch-Maitland$^\textrm{\scriptsize 45}$,    
A.~Qureshi$^\textrm{\scriptsize 1}$,    
S.K.~Radhakrishnan$^\textrm{\scriptsize 154}$,    
P.~Rados$^\textrm{\scriptsize 104}$,    
F.~Ragusa$^\textrm{\scriptsize 68a,68b}$,    
G.~Rahal$^\textrm{\scriptsize 97}$,    
J.A.~Raine$^\textrm{\scriptsize 100}$,    
S.~Rajagopalan$^\textrm{\scriptsize 29}$,    
T.~Rashid$^\textrm{\scriptsize 64}$,    
S.~Raspopov$^\textrm{\scriptsize 5}$,    
M.G.~Ratti$^\textrm{\scriptsize 68a,68b}$,    
D.M.~Rauch$^\textrm{\scriptsize 45}$,    
F.~Rauscher$^\textrm{\scriptsize 113}$,    
S.~Rave$^\textrm{\scriptsize 99}$,    
B.~Ravina$^\textrm{\scriptsize 148}$,    
I.~Ravinovich$^\textrm{\scriptsize 180}$,    
J.H.~Rawling$^\textrm{\scriptsize 100}$,    
M.~Raymond$^\textrm{\scriptsize 36}$,    
A.L.~Read$^\textrm{\scriptsize 133}$,    
N.P.~Readioff$^\textrm{\scriptsize 57}$,    
M.~Reale$^\textrm{\scriptsize 67a,67b}$,    
D.M.~Rebuzzi$^\textrm{\scriptsize 70a,70b}$,    
A.~Redelbach$^\textrm{\scriptsize 177}$,    
G.~Redlinger$^\textrm{\scriptsize 29}$,    
R.~Reece$^\textrm{\scriptsize 145}$,    
R.G.~Reed$^\textrm{\scriptsize 33e}$,    
K.~Reeves$^\textrm{\scriptsize 43}$,    
L.~Rehnisch$^\textrm{\scriptsize 19}$,    
J.~Reichert$^\textrm{\scriptsize 136}$,    
A.~Reiss$^\textrm{\scriptsize 99}$,    
C.~Rembser$^\textrm{\scriptsize 36}$,    
H.~Ren$^\textrm{\scriptsize 15a}$,    
M.~Rescigno$^\textrm{\scriptsize 72a}$,    
S.~Resconi$^\textrm{\scriptsize 68a}$,    
E.D.~Resseguie$^\textrm{\scriptsize 136}$,    
S.~Rettie$^\textrm{\scriptsize 175}$,    
E.~Reynolds$^\textrm{\scriptsize 21}$,    
O.L.~Rezanova$^\textrm{\scriptsize 121b,121a}$,    
P.~Reznicek$^\textrm{\scriptsize 142}$,    
R.~Richter$^\textrm{\scriptsize 114}$,    
S.~Richter$^\textrm{\scriptsize 94}$,    
E.~Richter-Was$^\textrm{\scriptsize 83b}$,    
O.~Ricken$^\textrm{\scriptsize 24}$,    
M.~Ridel$^\textrm{\scriptsize 135}$,    
P.~Rieck$^\textrm{\scriptsize 114}$,    
C.J.~Riegel$^\textrm{\scriptsize 182}$,    
O.~Rifki$^\textrm{\scriptsize 45}$,    
M.~Rijssenbeek$^\textrm{\scriptsize 154}$,    
A.~Rimoldi$^\textrm{\scriptsize 70a,70b}$,    
M.~Rimoldi$^\textrm{\scriptsize 20}$,    
L.~Rinaldi$^\textrm{\scriptsize 23b}$,    
G.~Ripellino$^\textrm{\scriptsize 153}$,    
B.~Risti\'{c}$^\textrm{\scriptsize 36}$,    
E.~Ritsch$^\textrm{\scriptsize 36}$,    
I.~Riu$^\textrm{\scriptsize 14}$,    
J.C.~Rivera~Vergara$^\textrm{\scriptsize 146a}$,    
F.~Rizatdinova$^\textrm{\scriptsize 129}$,    
E.~Rizvi$^\textrm{\scriptsize 92}$,    
C.~Rizzi$^\textrm{\scriptsize 14}$,    
R.T.~Roberts$^\textrm{\scriptsize 100}$,    
S.H.~Robertson$^\textrm{\scriptsize 103,ag}$,    
A.~Robichaud-Veronneau$^\textrm{\scriptsize 103}$,    
D.~Robinson$^\textrm{\scriptsize 32}$,    
J.E.M.~Robinson$^\textrm{\scriptsize 45}$,    
A.~Robson$^\textrm{\scriptsize 56}$,    
E.~Rocco$^\textrm{\scriptsize 99}$,    
C.~Roda$^\textrm{\scriptsize 71a,71b}$,    
Y.~Rodina$^\textrm{\scriptsize 101,ad}$,    
S.~Rodriguez~Bosca$^\textrm{\scriptsize 174}$,    
A.~Rodriguez~Perez$^\textrm{\scriptsize 14}$,    
D.~Rodriguez~Rodriguez$^\textrm{\scriptsize 174}$,    
A.M.~Rodr\'iguez~Vera$^\textrm{\scriptsize 168b}$,    
S.~Roe$^\textrm{\scriptsize 36}$,    
C.S.~Rogan$^\textrm{\scriptsize 58}$,    
O.~R{\o}hne$^\textrm{\scriptsize 133}$,    
R.~R\"ohrig$^\textrm{\scriptsize 114}$,    
C.P.A.~Roland$^\textrm{\scriptsize 65}$,    
J.~Roloff$^\textrm{\scriptsize 58}$,    
A.~Romaniouk$^\textrm{\scriptsize 111}$,    
M.~Romano$^\textrm{\scriptsize 23b,23a}$,    
E.~Romero~Adam$^\textrm{\scriptsize 174}$,    
N.~Rompotis$^\textrm{\scriptsize 90}$,    
M.~Ronzani$^\textrm{\scriptsize 124}$,    
L.~Roos$^\textrm{\scriptsize 135}$,    
S.~Rosati$^\textrm{\scriptsize 72a}$,    
K.~Rosbach$^\textrm{\scriptsize 51}$,    
P.~Rose$^\textrm{\scriptsize 145}$,    
N-A.~Rosien$^\textrm{\scriptsize 52}$,    
E.~Rossi$^\textrm{\scriptsize 69a,69b}$,    
L.P.~Rossi$^\textrm{\scriptsize 54b}$,    
L.~Rossini$^\textrm{\scriptsize 68a,68b}$,    
J.H.N.~Rosten$^\textrm{\scriptsize 32}$,    
R.~Rosten$^\textrm{\scriptsize 147}$,    
M.~Rotaru$^\textrm{\scriptsize 27b}$,    
J.~Rothberg$^\textrm{\scriptsize 147}$,    
D.~Rousseau$^\textrm{\scriptsize 64}$,    
D.~Roy$^\textrm{\scriptsize 33e}$,    
A.~Rozanov$^\textrm{\scriptsize 101}$,    
Y.~Rozen$^\textrm{\scriptsize 160}$,    
X.~Ruan$^\textrm{\scriptsize 33e}$,    
F.~Rubbo$^\textrm{\scriptsize 152}$,    
F.~R\"uhr$^\textrm{\scriptsize 51}$,    
A.~Ruiz-Martinez$^\textrm{\scriptsize 34}$,    
Z.~Rurikova$^\textrm{\scriptsize 51}$,    
N.A.~Rusakovich$^\textrm{\scriptsize 79}$,    
H.L.~Russell$^\textrm{\scriptsize 103}$,    
J.P.~Rutherfoord$^\textrm{\scriptsize 7}$,    
N.~Ruthmann$^\textrm{\scriptsize 36}$,    
E.M.~R{\"u}ttinger$^\textrm{\scriptsize 45,k}$,    
Y.F.~Ryabov$^\textrm{\scriptsize 137,*}$,    
M.~Rybar$^\textrm{\scriptsize 173}$,    
G.~Rybkin$^\textrm{\scriptsize 64}$,    
S.~Ryu$^\textrm{\scriptsize 6}$,    
A.~Ryzhov$^\textrm{\scriptsize 122}$,    
G.F.~Rzehorz$^\textrm{\scriptsize 52}$,    
P.~Sabatini$^\textrm{\scriptsize 52}$,    
G.~Sabato$^\textrm{\scriptsize 119}$,    
S.~Sacerdoti$^\textrm{\scriptsize 64}$,    
H.F-W.~Sadrozinski$^\textrm{\scriptsize 145}$,    
R.~Sadykov$^\textrm{\scriptsize 79}$,    
F.~Safai~Tehrani$^\textrm{\scriptsize 72a}$,    
P.~Saha$^\textrm{\scriptsize 120}$,    
M.~Sahinsoy$^\textrm{\scriptsize 60a}$,    
M.~Saimpert$^\textrm{\scriptsize 45}$,    
M.~Saito$^\textrm{\scriptsize 163}$,    
T.~Saito$^\textrm{\scriptsize 163}$,    
H.~Sakamoto$^\textrm{\scriptsize 163}$,    
A.~Sakharov$^\textrm{\scriptsize 124,am}$,    
D.~Salamani$^\textrm{\scriptsize 53}$,    
G.~Salamanna$^\textrm{\scriptsize 74a,74b}$,    
J.E.~Salazar~Loyola$^\textrm{\scriptsize 146c}$,    
D.~Salek$^\textrm{\scriptsize 119}$,    
P.H.~Sales~De~Bruin$^\textrm{\scriptsize 172}$,    
D.~Salihagic$^\textrm{\scriptsize 114,*}$,    
A.~Salnikov$^\textrm{\scriptsize 152}$,    
J.~Salt$^\textrm{\scriptsize 174}$,    
D.~Salvatore$^\textrm{\scriptsize 41b,41a}$,    
F.~Salvatore$^\textrm{\scriptsize 155}$,    
A.~Salvucci$^\textrm{\scriptsize 62a,62b,62c}$,    
A.~Salzburger$^\textrm{\scriptsize 36}$,    
D.~Sammel$^\textrm{\scriptsize 51}$,    
D.~Sampsonidis$^\textrm{\scriptsize 162}$,    
D.~Sampsonidou$^\textrm{\scriptsize 162}$,    
J.~S\'anchez$^\textrm{\scriptsize 174}$,    
A.~Sanchez~Pineda$^\textrm{\scriptsize 66a,66c}$,    
H.~Sandaker$^\textrm{\scriptsize 133}$,    
C.O.~Sander$^\textrm{\scriptsize 45}$,    
M.~Sandhoff$^\textrm{\scriptsize 182}$,    
C.~Sandoval$^\textrm{\scriptsize 22}$,    
D.P.C.~Sankey$^\textrm{\scriptsize 143}$,    
M.~Sannino$^\textrm{\scriptsize 54b,54a}$,    
Y.~Sano$^\textrm{\scriptsize 116}$,    
A.~Sansoni$^\textrm{\scriptsize 50}$,    
C.~Santoni$^\textrm{\scriptsize 38}$,    
H.~Santos$^\textrm{\scriptsize 139a}$,    
I.~Santoyo~Castillo$^\textrm{\scriptsize 155}$,    
A.~Sapronov$^\textrm{\scriptsize 79}$,    
J.G.~Saraiva$^\textrm{\scriptsize 139a,139d}$,    
O.~Sasaki$^\textrm{\scriptsize 81}$,    
K.~Sato$^\textrm{\scriptsize 169}$,    
E.~Sauvan$^\textrm{\scriptsize 5}$,    
P.~Savard$^\textrm{\scriptsize 167,ax}$,    
N.~Savic$^\textrm{\scriptsize 114}$,    
R.~Sawada$^\textrm{\scriptsize 163}$,    
C.~Sawyer$^\textrm{\scriptsize 143}$,    
L.~Sawyer$^\textrm{\scriptsize 95,ak}$,    
C.~Sbarra$^\textrm{\scriptsize 23b}$,    
A.~Sbrizzi$^\textrm{\scriptsize 23a}$,    
T.~Scanlon$^\textrm{\scriptsize 94}$,    
D.A.~Scannicchio$^\textrm{\scriptsize 171}$,    
J.~Schaarschmidt$^\textrm{\scriptsize 147}$,    
P.~Schacht$^\textrm{\scriptsize 114}$,    
B.M.~Schachtner$^\textrm{\scriptsize 113}$,    
D.~Schaefer$^\textrm{\scriptsize 37}$,    
L.~Schaefer$^\textrm{\scriptsize 136}$,    
J.~Schaeffer$^\textrm{\scriptsize 99}$,    
S.~Schaepe$^\textrm{\scriptsize 36}$,    
U.~Sch\"afer$^\textrm{\scriptsize 99}$,    
A.C.~Schaffer$^\textrm{\scriptsize 64}$,    
D.~Schaile$^\textrm{\scriptsize 113}$,    
R.D.~Schamberger$^\textrm{\scriptsize 154}$,    
N.~Scharmberg$^\textrm{\scriptsize 100}$,    
V.A.~Schegelsky$^\textrm{\scriptsize 137}$,    
D.~Scheirich$^\textrm{\scriptsize 142}$,    
F.~Schenck$^\textrm{\scriptsize 19}$,    
M.~Schernau$^\textrm{\scriptsize 171}$,    
C.~Schiavi$^\textrm{\scriptsize 54b,54a}$,    
S.~Schier$^\textrm{\scriptsize 145}$,    
L.K.~Schildgen$^\textrm{\scriptsize 24}$,    
Z.M.~Schillaci$^\textrm{\scriptsize 26}$,    
E.J.~Schioppa$^\textrm{\scriptsize 36}$,    
M.~Schioppa$^\textrm{\scriptsize 41b,41a}$,    
K.E.~Schleicher$^\textrm{\scriptsize 51}$,    
S.~Schlenker$^\textrm{\scriptsize 36}$,    
K.R.~Schmidt-Sommerfeld$^\textrm{\scriptsize 114}$,    
K.~Schmieden$^\textrm{\scriptsize 36}$,    
C.~Schmitt$^\textrm{\scriptsize 99}$,    
S.~Schmitt$^\textrm{\scriptsize 45}$,    
S.~Schmitz$^\textrm{\scriptsize 99}$,    
U.~Schnoor$^\textrm{\scriptsize 51}$,    
L.~Schoeffel$^\textrm{\scriptsize 144}$,    
A.~Schoening$^\textrm{\scriptsize 60b}$,    
E.~Schopf$^\textrm{\scriptsize 24}$,    
M.~Schott$^\textrm{\scriptsize 99}$,    
J.F.P.~Schouwenberg$^\textrm{\scriptsize 118}$,    
J.~Schovancova$^\textrm{\scriptsize 36}$,    
S.~Schramm$^\textrm{\scriptsize 53}$,    
N.~Schuh$^\textrm{\scriptsize 99}$,    
A.~Schulte$^\textrm{\scriptsize 99}$,    
H-C.~Schultz-Coulon$^\textrm{\scriptsize 60a}$,    
M.~Schumacher$^\textrm{\scriptsize 51}$,    
B.A.~Schumm$^\textrm{\scriptsize 145}$,    
Ph.~Schune$^\textrm{\scriptsize 144}$,    
A.~Schwartzman$^\textrm{\scriptsize 152}$,    
T.A.~Schwarz$^\textrm{\scriptsize 105}$,    
H.~Schweiger$^\textrm{\scriptsize 100}$,    
Ph.~Schwemling$^\textrm{\scriptsize 144}$,    
R.~Schwienhorst$^\textrm{\scriptsize 106}$,    
A.~Sciandra$^\textrm{\scriptsize 24}$,    
G.~Sciolla$^\textrm{\scriptsize 26}$,    
M.~Scornajenghi$^\textrm{\scriptsize 41b,41a}$,    
F.~Scuri$^\textrm{\scriptsize 71a}$,    
F.~Scutti$^\textrm{\scriptsize 104}$,    
L.M.~Scyboz$^\textrm{\scriptsize 114}$,    
J.~Searcy$^\textrm{\scriptsize 105}$,    
C.D.~Sebastiani$^\textrm{\scriptsize 72a,72b}$,    
P.~Seema$^\textrm{\scriptsize 24}$,    
S.C.~Seidel$^\textrm{\scriptsize 117}$,    
A.~Seiden$^\textrm{\scriptsize 145}$,    
J.M.~Seixas$^\textrm{\scriptsize 80b}$,    
G.~Sekhniaidze$^\textrm{\scriptsize 69a}$,    
K.~Sekhon$^\textrm{\scriptsize 105}$,    
S.J.~Sekula$^\textrm{\scriptsize 42}$,    
N.~Semprini-Cesari$^\textrm{\scriptsize 23b,23a}$,    
S.~Senkin$^\textrm{\scriptsize 38}$,    
C.~Serfon$^\textrm{\scriptsize 133}$,    
L.~Serin$^\textrm{\scriptsize 64}$,    
L.~Serkin$^\textrm{\scriptsize 66a,66b}$,    
M.~Sessa$^\textrm{\scriptsize 74a,74b}$,    
H.~Severini$^\textrm{\scriptsize 128}$,    
T.~\v{S}filigoj$^\textrm{\scriptsize 91}$,    
F.~Sforza$^\textrm{\scriptsize 170}$,    
A.~Sfyrla$^\textrm{\scriptsize 53}$,    
E.~Shabalina$^\textrm{\scriptsize 52}$,    
J.D.~Shahinian$^\textrm{\scriptsize 145}$,    
N.W.~Shaikh$^\textrm{\scriptsize 44a,44b}$,    
L.Y.~Shan$^\textrm{\scriptsize 15a}$,    
R.~Shang$^\textrm{\scriptsize 173}$,    
J.T.~Shank$^\textrm{\scriptsize 25}$,    
M.~Shapiro$^\textrm{\scriptsize 18}$,    
A.~Sharma$^\textrm{\scriptsize 134}$,    
A.S.~Sharma$^\textrm{\scriptsize 1}$,    
P.B.~Shatalov$^\textrm{\scriptsize 123}$,    
K.~Shaw$^\textrm{\scriptsize 66a,66b}$,    
S.M.~Shaw$^\textrm{\scriptsize 100}$,    
A.~Shcherbakova$^\textrm{\scriptsize 137}$,    
C.Y.~Shehu$^\textrm{\scriptsize 155}$,    
Y.~Shen$^\textrm{\scriptsize 128}$,    
N.~Sherafati$^\textrm{\scriptsize 34}$,    
A.D.~Sherman$^\textrm{\scriptsize 25}$,    
P.~Sherwood$^\textrm{\scriptsize 94}$,    
L.~Shi$^\textrm{\scriptsize 157,at}$,    
S.~Shimizu$^\textrm{\scriptsize 82}$,    
C.O.~Shimmin$^\textrm{\scriptsize 183}$,    
M.~Shimojima$^\textrm{\scriptsize 115}$,    
I.P.J.~Shipsey$^\textrm{\scriptsize 134}$,    
S.~Shirabe$^\textrm{\scriptsize 87}$,    
M.~Shiyakova$^\textrm{\scriptsize 79}$,    
J.~Shlomi$^\textrm{\scriptsize 180}$,    
A.~Shmeleva$^\textrm{\scriptsize 110}$,    
D.~Shoaleh~Saadi$^\textrm{\scriptsize 109}$,    
M.J.~Shochet$^\textrm{\scriptsize 37}$,    
J.~Shojaii$^\textrm{\scriptsize 104}$,    
D.R.~Shope$^\textrm{\scriptsize 128}$,    
S.~Shrestha$^\textrm{\scriptsize 126}$,    
E.~Shulga$^\textrm{\scriptsize 111}$,    
P.~Sicho$^\textrm{\scriptsize 140}$,    
A.M.~Sickles$^\textrm{\scriptsize 173}$,    
P.E.~Sidebo$^\textrm{\scriptsize 153}$,    
E.~Sideras~Haddad$^\textrm{\scriptsize 33e}$,    
O.~Sidiropoulou$^\textrm{\scriptsize 177}$,    
A.~Sidoti$^\textrm{\scriptsize 23b,23a}$,    
F.~Siegert$^\textrm{\scriptsize 47}$,    
Dj.~Sijacki$^\textrm{\scriptsize 16}$,    
J.~Silva$^\textrm{\scriptsize 139a}$,    
M.Jr.~Silva$^\textrm{\scriptsize 181}$,    
S.B.~Silverstein$^\textrm{\scriptsize 44a}$,    
L.~Simic$^\textrm{\scriptsize 79}$,    
S.~Simion$^\textrm{\scriptsize 64}$,    
E.~Simioni$^\textrm{\scriptsize 99}$,    
B.~Simmons$^\textrm{\scriptsize 94}$,    
M.~Simon$^\textrm{\scriptsize 99}$,    
P.~Sinervo$^\textrm{\scriptsize 167}$,    
N.B.~Sinev$^\textrm{\scriptsize 131}$,    
M.~Sioli$^\textrm{\scriptsize 23b,23a}$,    
G.~Siragusa$^\textrm{\scriptsize 177}$,    
I.~Siral$^\textrm{\scriptsize 105}$,    
S.Yu.~Sivoklokov$^\textrm{\scriptsize 112}$,    
J.~Sj\"{o}lin$^\textrm{\scriptsize 44a,44b}$,    
M.B.~Skinner$^\textrm{\scriptsize 89}$,    
P.~Skubic$^\textrm{\scriptsize 128}$,    
M.~Slater$^\textrm{\scriptsize 21}$,    
T.~Slavicek$^\textrm{\scriptsize 141}$,    
M.~Slawinska$^\textrm{\scriptsize 84}$,    
K.~Sliwa$^\textrm{\scriptsize 170}$,    
R.~Slovak$^\textrm{\scriptsize 142}$,    
V.~Smakhtin$^\textrm{\scriptsize 180}$,    
B.H.~Smart$^\textrm{\scriptsize 5}$,    
J.~Smiesko$^\textrm{\scriptsize 28a}$,    
N.~Smirnov$^\textrm{\scriptsize 111}$,    
S.Yu.~Smirnov$^\textrm{\scriptsize 111}$,    
Y.~Smirnov$^\textrm{\scriptsize 111}$,    
L.N.~Smirnova$^\textrm{\scriptsize 112,v}$,    
O.~Smirnova$^\textrm{\scriptsize 96}$,    
J.W.~Smith$^\textrm{\scriptsize 52}$,    
M.N.K.~Smith$^\textrm{\scriptsize 39}$,    
R.W.~Smith$^\textrm{\scriptsize 39}$,    
M.~Smizanska$^\textrm{\scriptsize 89}$,    
K.~Smolek$^\textrm{\scriptsize 141}$,    
A.A.~Snesarev$^\textrm{\scriptsize 110}$,    
I.M.~Snyder$^\textrm{\scriptsize 131}$,    
S.~Snyder$^\textrm{\scriptsize 29}$,    
R.~Sobie$^\textrm{\scriptsize 176,ag}$,    
F.~Socher$^\textrm{\scriptsize 47}$,    
A.M.~Soffa$^\textrm{\scriptsize 171}$,    
A.~Soffer$^\textrm{\scriptsize 161}$,    
A.~S{\o}gaard$^\textrm{\scriptsize 49}$,    
D.A.~Soh$^\textrm{\scriptsize 157}$,    
G.~Sokhrannyi$^\textrm{\scriptsize 91}$,    
C.A.~Solans~Sanchez$^\textrm{\scriptsize 36}$,    
M.~Solar$^\textrm{\scriptsize 141}$,    
E.Yu.~Soldatov$^\textrm{\scriptsize 111}$,    
U.~Soldevila$^\textrm{\scriptsize 174}$,    
A.A.~Solodkov$^\textrm{\scriptsize 122}$,    
A.~Soloshenko$^\textrm{\scriptsize 79}$,    
O.V.~Solovyanov$^\textrm{\scriptsize 122}$,    
V.~Solovyev$^\textrm{\scriptsize 137}$,    
P.~Sommer$^\textrm{\scriptsize 148}$,    
H.~Son$^\textrm{\scriptsize 170}$,    
W.~Song$^\textrm{\scriptsize 143}$,    
A.~Sopczak$^\textrm{\scriptsize 141}$,    
F.~Sopkova$^\textrm{\scriptsize 28b}$,    
D.~Sosa$^\textrm{\scriptsize 60b}$,    
C.L.~Sotiropoulou$^\textrm{\scriptsize 71a,71b}$,    
S.~Sottocornola$^\textrm{\scriptsize 70a,70b}$,    
R.~Soualah$^\textrm{\scriptsize 66a,66c,h}$,    
A.M.~Soukharev$^\textrm{\scriptsize 121b,121a}$,    
D.~South$^\textrm{\scriptsize 45}$,    
B.C.~Sowden$^\textrm{\scriptsize 93}$,    
S.~Spagnolo$^\textrm{\scriptsize 67a,67b}$,    
M.~Spalla$^\textrm{\scriptsize 114}$,    
M.~Spangenberg$^\textrm{\scriptsize 178}$,    
F.~Span\`o$^\textrm{\scriptsize 93}$,    
D.~Sperlich$^\textrm{\scriptsize 19}$,    
F.~Spettel$^\textrm{\scriptsize 114}$,    
T.M.~Spieker$^\textrm{\scriptsize 60a}$,    
R.~Spighi$^\textrm{\scriptsize 23b}$,    
G.~Spigo$^\textrm{\scriptsize 36}$,    
L.A.~Spiller$^\textrm{\scriptsize 104}$,    
M.~Spousta$^\textrm{\scriptsize 142}$,    
A.~Stabile$^\textrm{\scriptsize 68a,68b}$,    
R.~Stamen$^\textrm{\scriptsize 60a}$,    
S.~Stamm$^\textrm{\scriptsize 19}$,    
E.~Stanecka$^\textrm{\scriptsize 84}$,    
R.W.~Stanek$^\textrm{\scriptsize 6}$,    
C.~Stanescu$^\textrm{\scriptsize 74a}$,    
M.M.~Stanitzki$^\textrm{\scriptsize 45}$,    
B.~Stapf$^\textrm{\scriptsize 119}$,    
S.~Stapnes$^\textrm{\scriptsize 133}$,    
E.A.~Starchenko$^\textrm{\scriptsize 122}$,    
G.H.~Stark$^\textrm{\scriptsize 37}$,    
J.~Stark$^\textrm{\scriptsize 57}$,    
S.H.~Stark$^\textrm{\scriptsize 40}$,    
P.~Staroba$^\textrm{\scriptsize 140}$,    
P.~Starovoitov$^\textrm{\scriptsize 60a}$,    
S.~St\"arz$^\textrm{\scriptsize 36}$,    
R.~Staszewski$^\textrm{\scriptsize 84}$,    
M.~Stegler$^\textrm{\scriptsize 45}$,    
P.~Steinberg$^\textrm{\scriptsize 29}$,    
B.~Stelzer$^\textrm{\scriptsize 151}$,    
H.J.~Stelzer$^\textrm{\scriptsize 36}$,    
O.~Stelzer-Chilton$^\textrm{\scriptsize 168a}$,    
H.~Stenzel$^\textrm{\scriptsize 55}$,    
T.J.~Stevenson$^\textrm{\scriptsize 92}$,    
G.A.~Stewart$^\textrm{\scriptsize 36}$,    
M.C.~Stockton$^\textrm{\scriptsize 131}$,    
G.~Stoicea$^\textrm{\scriptsize 27b}$,    
P.~Stolte$^\textrm{\scriptsize 52}$,    
S.~Stonjek$^\textrm{\scriptsize 114}$,    
A.~Straessner$^\textrm{\scriptsize 47}$,    
J.~Strandberg$^\textrm{\scriptsize 153}$,    
S.~Strandberg$^\textrm{\scriptsize 44a,44b}$,    
M.~Strauss$^\textrm{\scriptsize 128}$,    
P.~Strizenec$^\textrm{\scriptsize 28b}$,    
R.~Str\"ohmer$^\textrm{\scriptsize 177}$,    
D.M.~Strom$^\textrm{\scriptsize 131}$,    
R.~Stroynowski$^\textrm{\scriptsize 42}$,    
A.~Strubig$^\textrm{\scriptsize 49}$,    
S.A.~Stucci$^\textrm{\scriptsize 29}$,    
B.~Stugu$^\textrm{\scriptsize 17}$,    
J.~Stupak$^\textrm{\scriptsize 128}$,    
N.A.~Styles$^\textrm{\scriptsize 45}$,    
D.~Su$^\textrm{\scriptsize 152}$,    
J.~Su$^\textrm{\scriptsize 138}$,    
S.~Suchek$^\textrm{\scriptsize 60a}$,    
Y.~Sugaya$^\textrm{\scriptsize 132}$,    
M.~Suk$^\textrm{\scriptsize 141}$,    
V.V.~Sulin$^\textrm{\scriptsize 110}$,    
D.M.S.~Sultan$^\textrm{\scriptsize 53}$,    
S.~Sultansoy$^\textrm{\scriptsize 4c}$,    
T.~Sumida$^\textrm{\scriptsize 85}$,    
S.~Sun$^\textrm{\scriptsize 105}$,    
X.~Sun$^\textrm{\scriptsize 3}$,    
K.~Suruliz$^\textrm{\scriptsize 155}$,    
C.J.E.~Suster$^\textrm{\scriptsize 156}$,    
M.R.~Sutton$^\textrm{\scriptsize 155}$,    
S.~Suzuki$^\textrm{\scriptsize 81}$,    
M.~Svatos$^\textrm{\scriptsize 140}$,    
M.~Swiatlowski$^\textrm{\scriptsize 37}$,    
S.P.~Swift$^\textrm{\scriptsize 2}$,    
A.~Sydorenko$^\textrm{\scriptsize 99}$,    
I.~Sykora$^\textrm{\scriptsize 28a}$,    
T.~Sykora$^\textrm{\scriptsize 142}$,    
D.~Ta$^\textrm{\scriptsize 99}$,    
K.~Tackmann$^\textrm{\scriptsize 45}$,    
J.~Taenzer$^\textrm{\scriptsize 161}$,    
A.~Taffard$^\textrm{\scriptsize 171}$,    
R.~Tafirout$^\textrm{\scriptsize 168a}$,    
E.~Tahirovic$^\textrm{\scriptsize 92}$,    
N.~Taiblum$^\textrm{\scriptsize 161}$,    
H.~Takai$^\textrm{\scriptsize 29}$,    
R.~Takashima$^\textrm{\scriptsize 86}$,    
E.H.~Takasugi$^\textrm{\scriptsize 114}$,    
K.~Takeda$^\textrm{\scriptsize 82}$,    
T.~Takeshita$^\textrm{\scriptsize 149}$,    
Y.~Takubo$^\textrm{\scriptsize 81}$,    
M.~Talby$^\textrm{\scriptsize 101}$,    
A.A.~Talyshev$^\textrm{\scriptsize 121b,121a}$,    
J.~Tanaka$^\textrm{\scriptsize 163}$,    
M.~Tanaka$^\textrm{\scriptsize 165}$,    
R.~Tanaka$^\textrm{\scriptsize 64}$,    
R.~Tanioka$^\textrm{\scriptsize 82}$,    
B.B.~Tannenwald$^\textrm{\scriptsize 126}$,    
S.~Tapia~Araya$^\textrm{\scriptsize 146c}$,    
S.~Tapprogge$^\textrm{\scriptsize 99}$,    
A.~Tarek~Abouelfadl~Mohamed$^\textrm{\scriptsize 135}$,    
S.~Tarem$^\textrm{\scriptsize 160}$,    
G.~Tarna$^\textrm{\scriptsize 27b,d}$,    
G.F.~Tartarelli$^\textrm{\scriptsize 68a}$,    
P.~Tas$^\textrm{\scriptsize 142}$,    
M.~Tasevsky$^\textrm{\scriptsize 140}$,    
T.~Tashiro$^\textrm{\scriptsize 85}$,    
E.~Tassi$^\textrm{\scriptsize 41b,41a}$,    
A.~Tavares~Delgado$^\textrm{\scriptsize 139a,139b}$,    
Y.~Tayalati$^\textrm{\scriptsize 35e}$,    
A.C.~Taylor$^\textrm{\scriptsize 117}$,    
A.J.~Taylor$^\textrm{\scriptsize 49}$,    
G.N.~Taylor$^\textrm{\scriptsize 104}$,    
P.T.E.~Taylor$^\textrm{\scriptsize 104}$,    
W.~Taylor$^\textrm{\scriptsize 168b}$,    
A.S.~Tee$^\textrm{\scriptsize 89}$,    
P.~Teixeira-Dias$^\textrm{\scriptsize 93}$,    
D.~Temple$^\textrm{\scriptsize 151}$,    
H.~Ten~Kate$^\textrm{\scriptsize 36}$,    
P.K.~Teng$^\textrm{\scriptsize 157}$,    
J.J.~Teoh$^\textrm{\scriptsize 132}$,    
F.~Tepel$^\textrm{\scriptsize 182}$,    
S.~Terada$^\textrm{\scriptsize 81}$,    
K.~Terashi$^\textrm{\scriptsize 163}$,    
J.~Terron$^\textrm{\scriptsize 98}$,    
S.~Terzo$^\textrm{\scriptsize 14}$,    
M.~Testa$^\textrm{\scriptsize 50}$,    
R.J.~Teuscher$^\textrm{\scriptsize 167,ag}$,    
S.J.~Thais$^\textrm{\scriptsize 183}$,    
T.~Theveneaux-Pelzer$^\textrm{\scriptsize 45}$,    
F.~Thiele$^\textrm{\scriptsize 40}$,    
J.P.~Thomas$^\textrm{\scriptsize 21}$,    
A.S.~Thompson$^\textrm{\scriptsize 56}$,    
P.D.~Thompson$^\textrm{\scriptsize 21}$,    
L.A.~Thomsen$^\textrm{\scriptsize 183}$,    
E.~Thomson$^\textrm{\scriptsize 136}$,    
Y.~Tian$^\textrm{\scriptsize 39}$,    
R.E.~Ticse~Torres$^\textrm{\scriptsize 52}$,    
V.O.~Tikhomirov$^\textrm{\scriptsize 110,ao}$,    
Yu.A.~Tikhonov$^\textrm{\scriptsize 121b,121a}$,    
S.~Timoshenko$^\textrm{\scriptsize 111}$,    
P.~Tipton$^\textrm{\scriptsize 183}$,    
S.~Tisserant$^\textrm{\scriptsize 101}$,    
K.~Todome$^\textrm{\scriptsize 165}$,    
S.~Todorova-Nova$^\textrm{\scriptsize 5}$,    
S.~Todt$^\textrm{\scriptsize 47}$,    
J.~Tojo$^\textrm{\scriptsize 87}$,    
S.~Tok\'ar$^\textrm{\scriptsize 28a}$,    
K.~Tokushuku$^\textrm{\scriptsize 81}$,    
E.~Tolley$^\textrm{\scriptsize 126}$,    
M.~Tomoto$^\textrm{\scriptsize 116}$,    
L.~Tompkins$^\textrm{\scriptsize 152}$,    
B.~Tong$^\textrm{\scriptsize 58}$,    
P.~Tornambe$^\textrm{\scriptsize 51}$,    
E.~Torrence$^\textrm{\scriptsize 131}$,    
H.~Torres$^\textrm{\scriptsize 47}$,    
E.~Torr\'o~Pastor$^\textrm{\scriptsize 147}$,    
C.~Tosciri$^\textrm{\scriptsize 134}$,    
J.~Toth$^\textrm{\scriptsize 101,af}$,    
F.~Touchard$^\textrm{\scriptsize 101}$,    
D.R.~Tovey$^\textrm{\scriptsize 148}$,    
C.J.~Treado$^\textrm{\scriptsize 124}$,    
T.~Trefzger$^\textrm{\scriptsize 177}$,    
F.~Tresoldi$^\textrm{\scriptsize 155}$,    
A.~Tricoli$^\textrm{\scriptsize 29}$,    
I.M.~Trigger$^\textrm{\scriptsize 168a}$,    
S.~Trincaz-Duvoid$^\textrm{\scriptsize 135}$,    
M.F.~Tripiana$^\textrm{\scriptsize 14}$,    
W.~Trischuk$^\textrm{\scriptsize 167}$,    
B.~Trocm\'e$^\textrm{\scriptsize 57}$,    
A.~Trofymov$^\textrm{\scriptsize 45}$,    
C.~Troncon$^\textrm{\scriptsize 68a}$,    
M.~Trovatelli$^\textrm{\scriptsize 176}$,    
F.~Trovato$^\textrm{\scriptsize 155}$,    
L.~Truong$^\textrm{\scriptsize 33c}$,    
M.~Trzebinski$^\textrm{\scriptsize 84}$,    
A.~Trzupek$^\textrm{\scriptsize 84}$,    
F.~Tsai$^\textrm{\scriptsize 45}$,    
K.W.~Tsang$^\textrm{\scriptsize 62a}$,    
J.C-L.~Tseng$^\textrm{\scriptsize 134}$,    
P.V.~Tsiareshka$^\textrm{\scriptsize 107}$,    
N.~Tsirintanis$^\textrm{\scriptsize 9}$,    
S.~Tsiskaridze$^\textrm{\scriptsize 14}$,    
V.~Tsiskaridze$^\textrm{\scriptsize 154}$,    
E.G.~Tskhadadze$^\textrm{\scriptsize 159a}$,    
I.I.~Tsukerman$^\textrm{\scriptsize 123}$,    
V.~Tsulaia$^\textrm{\scriptsize 18}$,    
S.~Tsuno$^\textrm{\scriptsize 81}$,    
D.~Tsybychev$^\textrm{\scriptsize 154}$,    
Y.~Tu$^\textrm{\scriptsize 62b}$,    
A.~Tudorache$^\textrm{\scriptsize 27b}$,    
V.~Tudorache$^\textrm{\scriptsize 27b}$,    
T.T.~Tulbure$^\textrm{\scriptsize 27a}$,    
A.N.~Tuna$^\textrm{\scriptsize 58}$,    
S.~Turchikhin$^\textrm{\scriptsize 79}$,    
D.~Turgeman$^\textrm{\scriptsize 180}$,    
I.~Turk~Cakir$^\textrm{\scriptsize 4b,w}$,    
R.T.~Turra$^\textrm{\scriptsize 68a}$,    
P.M.~Tuts$^\textrm{\scriptsize 39}$,    
G.~Ucchielli$^\textrm{\scriptsize 23b,23a}$,    
I.~Ueda$^\textrm{\scriptsize 81}$,    
M.~Ughetto$^\textrm{\scriptsize 44a,44b}$,    
F.~Ukegawa$^\textrm{\scriptsize 169}$,    
G.~Unal$^\textrm{\scriptsize 36}$,    
A.~Undrus$^\textrm{\scriptsize 29}$,    
G.~Unel$^\textrm{\scriptsize 171}$,    
F.C.~Ungaro$^\textrm{\scriptsize 104}$,    
Y.~Unno$^\textrm{\scriptsize 81}$,    
K.~Uno$^\textrm{\scriptsize 163}$,    
J.~Urban$^\textrm{\scriptsize 28b}$,    
P.~Urquijo$^\textrm{\scriptsize 104}$,    
P.~Urrejola$^\textrm{\scriptsize 99}$,    
G.~Usai$^\textrm{\scriptsize 8}$,    
J.~Usui$^\textrm{\scriptsize 81}$,    
L.~Vacavant$^\textrm{\scriptsize 101}$,    
V.~Vacek$^\textrm{\scriptsize 141}$,    
B.~Vachon$^\textrm{\scriptsize 103}$,    
K.O.H.~Vadla$^\textrm{\scriptsize 133}$,    
A.~Vaidya$^\textrm{\scriptsize 94}$,    
C.~Valderanis$^\textrm{\scriptsize 113}$,    
E.~Valdes~Santurio$^\textrm{\scriptsize 44a,44b}$,    
M.~Valente$^\textrm{\scriptsize 53}$,    
S.~Valentinetti$^\textrm{\scriptsize 23b,23a}$,    
A.~Valero$^\textrm{\scriptsize 174}$,    
L.~Val\'ery$^\textrm{\scriptsize 45}$,    
R.A.~Vallance$^\textrm{\scriptsize 21}$,    
A.~Vallier$^\textrm{\scriptsize 5}$,    
J.A.~Valls~Ferrer$^\textrm{\scriptsize 174}$,    
T.R.~Van~Daalen$^\textrm{\scriptsize 14}$,    
W.~Van~Den~Wollenberg$^\textrm{\scriptsize 119}$,    
H.~Van~der~Graaf$^\textrm{\scriptsize 119}$,    
P.~Van~Gemmeren$^\textrm{\scriptsize 6}$,    
J.~Van~Nieuwkoop$^\textrm{\scriptsize 151}$,    
I.~Van~Vulpen$^\textrm{\scriptsize 119}$,    
M.C.~van~Woerden$^\textrm{\scriptsize 119}$,    
M.~Vanadia$^\textrm{\scriptsize 73a,73b}$,    
W.~Vandelli$^\textrm{\scriptsize 36}$,    
A.~Vaniachine$^\textrm{\scriptsize 166}$,    
P.~Vankov$^\textrm{\scriptsize 119}$,    
G.~Vardanyan$^\textrm{\scriptsize 184}$,    
R.~Vari$^\textrm{\scriptsize 72a}$,    
E.W.~Varnes$^\textrm{\scriptsize 7}$,    
C.~Varni$^\textrm{\scriptsize 54b,54a}$,    
T.~Varol$^\textrm{\scriptsize 42}$,    
D.~Varouchas$^\textrm{\scriptsize 64}$,    
A.~Vartapetian$^\textrm{\scriptsize 8}$,    
K.E.~Varvell$^\textrm{\scriptsize 156}$,    
G.A.~Vasquez$^\textrm{\scriptsize 146c}$,    
J.G.~Vasquez$^\textrm{\scriptsize 183}$,    
F.~Vazeille$^\textrm{\scriptsize 38}$,    
D.~Vazquez~Furelos$^\textrm{\scriptsize 14}$,    
T.~Vazquez~Schroeder$^\textrm{\scriptsize 103}$,    
J.~Veatch$^\textrm{\scriptsize 52}$,    
V.~Vecchio$^\textrm{\scriptsize 74a,74b}$,    
L.M.~Veloce$^\textrm{\scriptsize 167}$,    
F.~Veloso$^\textrm{\scriptsize 139a,139c}$,    
S.~Veneziano$^\textrm{\scriptsize 72a}$,    
A.~Ventura$^\textrm{\scriptsize 67a,67b}$,    
M.~Venturi$^\textrm{\scriptsize 176}$,    
N.~Venturi$^\textrm{\scriptsize 36}$,    
V.~Vercesi$^\textrm{\scriptsize 70a}$,    
M.~Verducci$^\textrm{\scriptsize 74a,74b}$,    
W.~Verkerke$^\textrm{\scriptsize 119}$,    
A.T.~Vermeulen$^\textrm{\scriptsize 119}$,    
J.C.~Vermeulen$^\textrm{\scriptsize 119}$,    
M.C.~Vetterli$^\textrm{\scriptsize 151,ax}$,    
N.~Viaux~Maira$^\textrm{\scriptsize 146c}$,    
O.~Viazlo$^\textrm{\scriptsize 96}$,    
I.~Vichou$^\textrm{\scriptsize 173,*}$,    
T.~Vickey$^\textrm{\scriptsize 148}$,    
O.E.~Vickey~Boeriu$^\textrm{\scriptsize 148}$,    
G.H.A.~Viehhauser$^\textrm{\scriptsize 134}$,    
S.~Viel$^\textrm{\scriptsize 18}$,    
L.~Vigani$^\textrm{\scriptsize 134}$,    
M.~Villa$^\textrm{\scriptsize 23b,23a}$,    
M.~Villaplana~Perez$^\textrm{\scriptsize 68a,68b}$,    
E.~Vilucchi$^\textrm{\scriptsize 50}$,    
M.G.~Vincter$^\textrm{\scriptsize 34}$,    
V.B.~Vinogradov$^\textrm{\scriptsize 79}$,    
A.~Vishwakarma$^\textrm{\scriptsize 45}$,    
C.~Vittori$^\textrm{\scriptsize 23b,23a}$,    
I.~Vivarelli$^\textrm{\scriptsize 155}$,    
S.~Vlachos$^\textrm{\scriptsize 10}$,    
M.~Vogel$^\textrm{\scriptsize 182}$,    
P.~Vokac$^\textrm{\scriptsize 141}$,    
G.~Volpi$^\textrm{\scriptsize 14}$,    
S.E.~von~Buddenbrock$^\textrm{\scriptsize 33e}$,    
E.~Von~Toerne$^\textrm{\scriptsize 24}$,    
V.~Vorobel$^\textrm{\scriptsize 142}$,    
K.~Vorobev$^\textrm{\scriptsize 111}$,    
M.~Vos$^\textrm{\scriptsize 174}$,    
J.H.~Vossebeld$^\textrm{\scriptsize 90}$,    
N.~Vranjes$^\textrm{\scriptsize 16}$,    
M.~Vranjes~Milosavljevic$^\textrm{\scriptsize 16}$,    
V.~Vrba$^\textrm{\scriptsize 141}$,    
M.~Vreeswijk$^\textrm{\scriptsize 119}$,    
R.~Vuillermet$^\textrm{\scriptsize 36}$,    
I.~Vukotic$^\textrm{\scriptsize 37}$,    
P.~Wagner$^\textrm{\scriptsize 24}$,    
W.~Wagner$^\textrm{\scriptsize 182}$,    
J.~Wagner-Kuhr$^\textrm{\scriptsize 113}$,    
H.~Wahlberg$^\textrm{\scriptsize 88}$,    
S.~Wahrmund$^\textrm{\scriptsize 47}$,    
K.~Wakamiya$^\textrm{\scriptsize 82}$,    
J.~Walder$^\textrm{\scriptsize 89}$,    
R.~Walker$^\textrm{\scriptsize 113}$,    
W.~Walkowiak$^\textrm{\scriptsize 150}$,    
V.~Wallangen$^\textrm{\scriptsize 44a,44b}$,    
A.M.~Wang$^\textrm{\scriptsize 58}$,    
C.~Wang$^\textrm{\scriptsize 59b,d}$,    
F.~Wang$^\textrm{\scriptsize 181}$,    
H.~Wang$^\textrm{\scriptsize 18}$,    
H.~Wang$^\textrm{\scriptsize 3}$,    
J.~Wang$^\textrm{\scriptsize 156}$,    
J.~Wang$^\textrm{\scriptsize 60b}$,    
P.~Wang$^\textrm{\scriptsize 42}$,    
Q.~Wang$^\textrm{\scriptsize 128}$,    
R.-J.~Wang$^\textrm{\scriptsize 135}$,    
R.~Wang$^\textrm{\scriptsize 59a}$,    
R.~Wang$^\textrm{\scriptsize 6}$,    
S.M.~Wang$^\textrm{\scriptsize 157}$,    
T.~Wang$^\textrm{\scriptsize 39}$,    
W.~Wang$^\textrm{\scriptsize 157,q}$,    
W.X.~Wang$^\textrm{\scriptsize 59a,ah}$,    
Y.~Wang$^\textrm{\scriptsize 59a,al}$,    
Z.~Wang$^\textrm{\scriptsize 59c}$,    
C.~Wanotayaroj$^\textrm{\scriptsize 45}$,    
A.~Warburton$^\textrm{\scriptsize 103}$,    
C.P.~Ward$^\textrm{\scriptsize 32}$,    
D.R.~Wardrope$^\textrm{\scriptsize 94}$,    
A.~Washbrook$^\textrm{\scriptsize 49}$,    
P.M.~Watkins$^\textrm{\scriptsize 21}$,    
A.T.~Watson$^\textrm{\scriptsize 21}$,    
M.F.~Watson$^\textrm{\scriptsize 21}$,    
G.~Watts$^\textrm{\scriptsize 147}$,    
S.~Watts$^\textrm{\scriptsize 100}$,    
B.M.~Waugh$^\textrm{\scriptsize 94}$,    
A.F.~Webb$^\textrm{\scriptsize 11}$,    
S.~Webb$^\textrm{\scriptsize 99}$,    
C.~Weber$^\textrm{\scriptsize 183}$,    
M.S.~Weber$^\textrm{\scriptsize 20}$,    
S.A.~Weber$^\textrm{\scriptsize 34}$,    
S.M.~Weber$^\textrm{\scriptsize 60a}$,    
J.S.~Webster$^\textrm{\scriptsize 6}$,    
A.R.~Weidberg$^\textrm{\scriptsize 134}$,    
B.~Weinert$^\textrm{\scriptsize 65}$,    
J.~Weingarten$^\textrm{\scriptsize 52}$,    
M.~Weirich$^\textrm{\scriptsize 99}$,    
C.~Weiser$^\textrm{\scriptsize 51}$,    
P.S.~Wells$^\textrm{\scriptsize 36}$,    
T.~Wenaus$^\textrm{\scriptsize 29}$,    
T.~Wengler$^\textrm{\scriptsize 36}$,    
S.~Wenig$^\textrm{\scriptsize 36}$,    
N.~Wermes$^\textrm{\scriptsize 24}$,    
M.D.~Werner$^\textrm{\scriptsize 78}$,    
P.~Werner$^\textrm{\scriptsize 36}$,    
M.~Wessels$^\textrm{\scriptsize 60a}$,    
T.D.~Weston$^\textrm{\scriptsize 20}$,    
K.~Whalen$^\textrm{\scriptsize 131}$,    
N.L.~Whallon$^\textrm{\scriptsize 147}$,    
A.M.~Wharton$^\textrm{\scriptsize 89}$,    
A.S.~White$^\textrm{\scriptsize 105}$,    
A.~White$^\textrm{\scriptsize 8}$,    
M.J.~White$^\textrm{\scriptsize 1}$,    
R.~White$^\textrm{\scriptsize 146c}$,    
D.~Whiteson$^\textrm{\scriptsize 171}$,    
B.W.~Whitmore$^\textrm{\scriptsize 89}$,    
F.J.~Wickens$^\textrm{\scriptsize 143}$,    
W.~Wiedenmann$^\textrm{\scriptsize 181}$,    
M.~Wielers$^\textrm{\scriptsize 143}$,    
C.~Wiglesworth$^\textrm{\scriptsize 40}$,    
L.A.M.~Wiik-Fuchs$^\textrm{\scriptsize 51}$,    
A.~Wildauer$^\textrm{\scriptsize 114}$,    
F.~Wilk$^\textrm{\scriptsize 100}$,    
H.G.~Wilkens$^\textrm{\scriptsize 36}$,    
H.H.~Williams$^\textrm{\scriptsize 136}$,    
S.~Williams$^\textrm{\scriptsize 32}$,    
C.~Willis$^\textrm{\scriptsize 106}$,    
S.~Willocq$^\textrm{\scriptsize 102}$,    
J.A.~Wilson$^\textrm{\scriptsize 21}$,    
I.~Wingerter-Seez$^\textrm{\scriptsize 5}$,    
E.~Winkels$^\textrm{\scriptsize 155}$,    
F.~Winklmeier$^\textrm{\scriptsize 131}$,    
O.J.~Winston$^\textrm{\scriptsize 155}$,    
B.T.~Winter$^\textrm{\scriptsize 24}$,    
M.~Wittgen$^\textrm{\scriptsize 152}$,    
M.~Wobisch$^\textrm{\scriptsize 95}$,    
A.~Wolf$^\textrm{\scriptsize 99}$,    
T.M.H.~Wolf$^\textrm{\scriptsize 119}$,    
R.~Wolff$^\textrm{\scriptsize 101}$,    
M.W.~Wolter$^\textrm{\scriptsize 84}$,    
H.~Wolters$^\textrm{\scriptsize 139a,139c}$,    
V.W.S.~Wong$^\textrm{\scriptsize 175}$,    
N.L.~Woods$^\textrm{\scriptsize 145}$,    
S.D.~Worm$^\textrm{\scriptsize 21}$,    
B.K.~Wosiek$^\textrm{\scriptsize 84}$,    
K.W.~Wo\'{z}niak$^\textrm{\scriptsize 84}$,    
K.~Wraight$^\textrm{\scriptsize 56}$,    
M.~Wu$^\textrm{\scriptsize 37}$,    
S.L.~Wu$^\textrm{\scriptsize 181}$,    
X.~Wu$^\textrm{\scriptsize 53}$,    
Y.~Wu$^\textrm{\scriptsize 59a}$,    
T.R.~Wyatt$^\textrm{\scriptsize 100}$,    
B.M.~Wynne$^\textrm{\scriptsize 49}$,    
S.~Xella$^\textrm{\scriptsize 40}$,    
Z.~Xi$^\textrm{\scriptsize 105}$,    
L.~Xia$^\textrm{\scriptsize 15b}$,    
D.~Xu$^\textrm{\scriptsize 15a}$,    
H.~Xu$^\textrm{\scriptsize 59a,d}$,    
L.~Xu$^\textrm{\scriptsize 29}$,    
T.~Xu$^\textrm{\scriptsize 144}$,    
W.~Xu$^\textrm{\scriptsize 105}$,    
B.~Yabsley$^\textrm{\scriptsize 156}$,    
S.~Yacoob$^\textrm{\scriptsize 33a}$,    
K.~Yajima$^\textrm{\scriptsize 132}$,    
D.P.~Yallup$^\textrm{\scriptsize 94}$,    
D.~Yamaguchi$^\textrm{\scriptsize 165}$,    
Y.~Yamaguchi$^\textrm{\scriptsize 165}$,    
A.~Yamamoto$^\textrm{\scriptsize 81}$,    
T.~Yamanaka$^\textrm{\scriptsize 163}$,    
F.~Yamane$^\textrm{\scriptsize 82}$,    
M.~Yamatani$^\textrm{\scriptsize 163}$,    
T.~Yamazaki$^\textrm{\scriptsize 163}$,    
Y.~Yamazaki$^\textrm{\scriptsize 82}$,    
Z.~Yan$^\textrm{\scriptsize 25}$,    
H.J.~Yang$^\textrm{\scriptsize 59c,59d}$,    
H.T.~Yang$^\textrm{\scriptsize 18}$,    
S.~Yang$^\textrm{\scriptsize 77}$,    
Y.~Yang$^\textrm{\scriptsize 163}$,    
Y.~Yang$^\textrm{\scriptsize 157}$,    
Z.~Yang$^\textrm{\scriptsize 17}$,    
W-M.~Yao$^\textrm{\scriptsize 18}$,    
Y.C.~Yap$^\textrm{\scriptsize 45}$,    
Y.~Yasu$^\textrm{\scriptsize 81}$,    
E.~Yatsenko$^\textrm{\scriptsize 5}$,    
K.H.~Yau~Wong$^\textrm{\scriptsize 24}$,    
J.~Ye$^\textrm{\scriptsize 42}$,    
S.~Ye$^\textrm{\scriptsize 29}$,    
I.~Yeletskikh$^\textrm{\scriptsize 79}$,    
E.~Yigitbasi$^\textrm{\scriptsize 25}$,    
E.~Yildirim$^\textrm{\scriptsize 99}$,    
K.~Yorita$^\textrm{\scriptsize 179}$,    
K.~Yoshihara$^\textrm{\scriptsize 136}$,    
C.J.S.~Young$^\textrm{\scriptsize 36}$,    
C.~Young$^\textrm{\scriptsize 152}$,    
J.~Yu$^\textrm{\scriptsize 78}$,    
J.~Yu$^\textrm{\scriptsize 8}$,    
X.~Yue$^\textrm{\scriptsize 60a}$,    
S.P.Y.~Yuen$^\textrm{\scriptsize 24}$,    
I.~Yusuff$^\textrm{\scriptsize 32}$,    
B.~Zabinski$^\textrm{\scriptsize 84}$,    
G.~Zacharis$^\textrm{\scriptsize 10}$,    
R.~Zaidan$^\textrm{\scriptsize 14}$,    
A.M.~Zaitsev$^\textrm{\scriptsize 122,an}$,    
N.~Zakharchuk$^\textrm{\scriptsize 45}$,    
J.~Zalieckas$^\textrm{\scriptsize 17}$,    
S.~Zambito$^\textrm{\scriptsize 58}$,    
D.~Zanzi$^\textrm{\scriptsize 36}$,    
C.~Zeitnitz$^\textrm{\scriptsize 182}$,    
G.~Zemaityte$^\textrm{\scriptsize 134}$,    
J.C.~Zeng$^\textrm{\scriptsize 173}$,    
Q.~Zeng$^\textrm{\scriptsize 152}$,    
O.~Zenin$^\textrm{\scriptsize 122}$,    
T.~\v{Z}eni\v{s}$^\textrm{\scriptsize 28a}$,    
D.~Zerwas$^\textrm{\scriptsize 64}$,    
M.~Zgubi\v{c}$^\textrm{\scriptsize 134}$,    
D.F.~Zhang$^\textrm{\scriptsize 59b}$,    
D.~Zhang$^\textrm{\scriptsize 105}$,    
F.~Zhang$^\textrm{\scriptsize 181}$,    
G.~Zhang$^\textrm{\scriptsize 59a,ah}$,    
H.~Zhang$^\textrm{\scriptsize 15c}$,    
J.~Zhang$^\textrm{\scriptsize 6}$,    
L.~Zhang$^\textrm{\scriptsize 51}$,    
L.~Zhang$^\textrm{\scriptsize 59a}$,    
M.~Zhang$^\textrm{\scriptsize 173}$,    
P.~Zhang$^\textrm{\scriptsize 15c}$,    
R.~Zhang$^\textrm{\scriptsize 59a,d}$,    
R.~Zhang$^\textrm{\scriptsize 24}$,    
X.~Zhang$^\textrm{\scriptsize 59b}$,    
Y.~Zhang$^\textrm{\scriptsize 15a,15d}$,    
Z.~Zhang$^\textrm{\scriptsize 64}$,    
X.~Zhao$^\textrm{\scriptsize 42}$,    
Y.~Zhao$^\textrm{\scriptsize 59b,64,ab}$,    
Z.~Zhao$^\textrm{\scriptsize 59a}$,    
A.~Zhemchugov$^\textrm{\scriptsize 79}$,    
B.~Zhou$^\textrm{\scriptsize 105}$,    
C.~Zhou$^\textrm{\scriptsize 181}$,    
L.~Zhou$^\textrm{\scriptsize 42}$,    
M.S.~Zhou$^\textrm{\scriptsize 15a,15d}$,    
M.~Zhou$^\textrm{\scriptsize 154}$,    
N.~Zhou$^\textrm{\scriptsize 59c}$,    
Y.~Zhou$^\textrm{\scriptsize 7}$,    
C.G.~Zhu$^\textrm{\scriptsize 59b}$,    
H.L.~Zhu$^\textrm{\scriptsize 59a}$,    
H.~Zhu$^\textrm{\scriptsize 15a}$,    
J.~Zhu$^\textrm{\scriptsize 105}$,    
Y.~Zhu$^\textrm{\scriptsize 59a}$,    
X.~Zhuang$^\textrm{\scriptsize 15a}$,    
K.~Zhukov$^\textrm{\scriptsize 110}$,    
V.~Zhulanov$^\textrm{\scriptsize 121b,121a}$,    
A.~Zibell$^\textrm{\scriptsize 177}$,    
D.~Zieminska$^\textrm{\scriptsize 65}$,    
N.I.~Zimine$^\textrm{\scriptsize 79}$,    
S.~Zimmermann$^\textrm{\scriptsize 51}$,    
Z.~Zinonos$^\textrm{\scriptsize 114}$,    
M.~Zinser$^\textrm{\scriptsize 99}$,    
M.~Ziolkowski$^\textrm{\scriptsize 150}$,    
L.~\v{Z}ivkovi\'{c}$^\textrm{\scriptsize 16}$,    
G.~Zobernig$^\textrm{\scriptsize 181}$,    
A.~Zoccoli$^\textrm{\scriptsize 23b,23a}$,    
K.~Zoch$^\textrm{\scriptsize 52}$,    
T.G.~Zorbas$^\textrm{\scriptsize 148}$,    
R.~Zou$^\textrm{\scriptsize 37}$,    
M.~Zur~Nedden$^\textrm{\scriptsize 19}$,    
L.~Zwalinski$^\textrm{\scriptsize 36}$.    
\bigskip
\\

$^{1}$Department of Physics, University of Adelaide, Adelaide; Australia.\\
$^{2}$Physics Department, SUNY Albany, Albany NY; United States of America.\\
$^{3}$Department of Physics, University of Alberta, Edmonton AB; Canada.\\
$^{4}$$^{(a)}$Department of Physics, Ankara University, Ankara;$^{(b)}$Istanbul Aydin University, Istanbul;$^{(c)}$Division of Physics, TOBB University of Economics and Technology, Ankara; Turkey.\\
$^{5}$LAPP, Universit\'e Grenoble Alpes, Universit\'e Savoie Mont Blanc, CNRS/IN2P3, Annecy; France.\\
$^{6}$High Energy Physics Division, Argonne National Laboratory, Argonne IL; United States of America.\\
$^{7}$Department of Physics, University of Arizona, Tucson AZ; United States of America.\\
$^{8}$Department of Physics, University of Texas at Arlington, Arlington TX; United States of America.\\
$^{9}$Physics Department, National and Kapodistrian University of Athens, Athens; Greece.\\
$^{10}$Physics Department, National Technical University of Athens, Zografou; Greece.\\
$^{11}$Department of Physics, University of Texas at Austin, Austin TX; United States of America.\\
$^{12}$$^{(a)}$Bahcesehir University, Faculty of Engineering and Natural Sciences, Istanbul;$^{(b)}$Istanbul Bilgi University, Faculty of Engineering and Natural Sciences, Istanbul;$^{(c)}$Department of Physics, Bogazici University, Istanbul;$^{(d)}$Department of Physics Engineering, Gaziantep University, Gaziantep; Turkey.\\
$^{13}$Institute of Physics, Azerbaijan Academy of Sciences, Baku; Azerbaijan.\\
$^{14}$Institut de F\'isica d'Altes Energies (IFAE), Barcelona Institute of Science and Technology, Barcelona; Spain.\\
$^{15}$$^{(a)}$Institute of High Energy Physics, Chinese Academy of Sciences, Beijing;$^{(b)}$Physics Department, Tsinghua University, Beijing;$^{(c)}$Department of Physics, Nanjing University, Nanjing;$^{(d)}$University of Chinese Academy of Science (UCAS), Beijing; China.\\
$^{16}$Institute of Physics, University of Belgrade, Belgrade; Serbia.\\
$^{17}$Department for Physics and Technology, University of Bergen, Bergen; Norway.\\
$^{18}$Physics Division, Lawrence Berkeley National Laboratory and University of California, Berkeley CA; United States of America.\\
$^{19}$Institut f\"{u}r Physik, Humboldt Universit\"{a}t zu Berlin, Berlin; Germany.\\
$^{20}$Albert Einstein Center for Fundamental Physics and Laboratory for High Energy Physics, University of Bern, Bern; Switzerland.\\
$^{21}$School of Physics and Astronomy, University of Birmingham, Birmingham; United Kingdom.\\
$^{22}$Facultad de Ciencias y Centro de Investigaci\'ones, Universidad Antonio Nari\~no, Bogota; Colombia.\\
$^{23}$$^{(a)}$INFN Bologna and Universita' di Bologna, Dipartimento di Fisica;$^{(b)}$INFN Sezione di Bologna; Italy.\\
$^{24}$Physikalisches Institut, Universit\"{a}t Bonn, Bonn; Germany.\\
$^{25}$Department of Physics, Boston University, Boston MA; United States of America.\\
$^{26}$Department of Physics, Brandeis University, Waltham MA; United States of America.\\
$^{27}$$^{(a)}$Transilvania University of Brasov, Brasov;$^{(b)}$Horia Hulubei National Institute of Physics and Nuclear Engineering, Bucharest;$^{(c)}$Department of Physics, Alexandru Ioan Cuza University of Iasi, Iasi;$^{(d)}$National Institute for Research and Development of Isotopic and Molecular Technologies, Physics Department, Cluj-Napoca;$^{(e)}$University Politehnica Bucharest, Bucharest;$^{(f)}$West University in Timisoara, Timisoara; Romania.\\
$^{28}$$^{(a)}$Faculty of Mathematics, Physics and Informatics, Comenius University, Bratislava;$^{(b)}$Department of Subnuclear Physics, Institute of Experimental Physics of the Slovak Academy of Sciences, Kosice; Slovak Republic.\\
$^{29}$Physics Department, Brookhaven National Laboratory, Upton NY; United States of America.\\
$^{30}$Departamento de F\'isica, Universidad de Buenos Aires, Buenos Aires; Argentina.\\
$^{31}$California State University, CA; United States of America.\\
$^{32}$Cavendish Laboratory, University of Cambridge, Cambridge; United Kingdom.\\
$^{33}$$^{(a)}$Department of Physics, University of Cape Town, Cape Town;$^{(b)}$iThemba Labs, Western Cape;$^{(c)}$Department of Mechanical Engineering Science, University of Johannesburg, Johannesburg;$^{(d)}$University of South Africa, Department of Physics, Pretoria;$^{(e)}$School of Physics, University of the Witwatersrand, Johannesburg; South Africa.\\
$^{34}$Department of Physics, Carleton University, Ottawa ON; Canada.\\
$^{35}$$^{(a)}$Facult\'e des Sciences Ain Chock, R\'eseau Universitaire de Physique des Hautes Energies - Universit\'e Hassan II, Casablanca;$^{(b)}$Facult\'{e} des Sciences, Universit\'{e} Ibn-Tofail, K\'{e}nitra;$^{(c)}$Facult\'e des Sciences Semlalia, Universit\'e Cadi Ayyad, LPHEA-Marrakech;$^{(d)}$Facult\'e des Sciences, Universit\'e Mohamed Premier and LPTPM, Oujda;$^{(e)}$Facult\'e des sciences, Universit\'e Mohammed V, Rabat; Morocco.\\
$^{36}$CERN, Geneva; Switzerland.\\
$^{37}$Enrico Fermi Institute, University of Chicago, Chicago IL; United States of America.\\
$^{38}$LPC, Universit\'e Clermont Auvergne, CNRS/IN2P3, Clermont-Ferrand; France.\\
$^{39}$Nevis Laboratory, Columbia University, Irvington NY; United States of America.\\
$^{40}$Niels Bohr Institute, University of Copenhagen, Copenhagen; Denmark.\\
$^{41}$$^{(a)}$Dipartimento di Fisica, Universit\`a della Calabria, Rende;$^{(b)}$INFN Gruppo Collegato di Cosenza, Laboratori Nazionali di Frascati; Italy.\\
$^{42}$Physics Department, Southern Methodist University, Dallas TX; United States of America.\\
$^{43}$Physics Department, University of Texas at Dallas, Richardson TX; United States of America.\\
$^{44}$$^{(a)}$Department of Physics, Stockholm University;$^{(b)}$Oskar Klein Centre, Stockholm; Sweden.\\
$^{45}$Deutsches Elektronen-Synchrotron DESY, Hamburg and Zeuthen; Germany.\\
$^{46}$Lehrstuhl f{\"u}r Experimentelle Physik IV, Technische Universit{\"a}t Dortmund, Dortmund; Germany.\\
$^{47}$Institut f\"{u}r Kern-~und Teilchenphysik, Technische Universit\"{a}t Dresden, Dresden; Germany.\\
$^{48}$Department of Physics, Duke University, Durham NC; United States of America.\\
$^{49}$SUPA - School of Physics and Astronomy, University of Edinburgh, Edinburgh; United Kingdom.\\
$^{50}$INFN e Laboratori Nazionali di Frascati, Frascati; Italy.\\
$^{51}$Physikalisches Institut, Albert-Ludwigs-Universit\"{a}t Freiburg, Freiburg; Germany.\\
$^{52}$II. Physikalisches Institut, Georg-August-Universit\"{a}t G\"ottingen, G\"ottingen; Germany.\\
$^{53}$D\'epartement de Physique Nucl\'eaire et Corpusculaire, Universit\'e de Gen\`eve, Gen\`eve; Switzerland.\\
$^{54}$$^{(a)}$Dipartimento di Fisica, Universit\`a di Genova, Genova;$^{(b)}$INFN Sezione di Genova; Italy.\\
$^{55}$II. Physikalisches Institut, Justus-Liebig-Universit{\"a}t Giessen, Giessen; Germany.\\
$^{56}$SUPA - School of Physics and Astronomy, University of Glasgow, Glasgow; United Kingdom.\\
$^{57}$LPSC, Universit\'e Grenoble Alpes, CNRS/IN2P3, Grenoble INP, Grenoble; France.\\
$^{58}$Laboratory for Particle Physics and Cosmology, Harvard University, Cambridge MA; United States of America.\\
$^{59}$$^{(a)}$Department of Modern Physics and State Key Laboratory of Particle Detection and Electronics, University of Science and Technology of China, Hefei;$^{(b)}$Institute of Frontier and Interdisciplinary Science and Key Laboratory of Particle Physics and Particle Irradiation (MOE), Shandong University, Qingdao;$^{(c)}$School of Physics and Astronomy, Shanghai Jiao Tong University, KLPPAC-MoE, SKLPPC, Shanghai;$^{(d)}$Tsung-Dao Lee Institute, Shanghai; China.\\
$^{60}$$^{(a)}$Kirchhoff-Institut f\"{u}r Physik, Ruprecht-Karls-Universit\"{a}t Heidelberg, Heidelberg;$^{(b)}$Physikalisches Institut, Ruprecht-Karls-Universit\"{a}t Heidelberg, Heidelberg; Germany.\\
$^{61}$Faculty of Applied Information Science, Hiroshima Institute of Technology, Hiroshima; Japan.\\
$^{62}$$^{(a)}$Department of Physics, Chinese University of Hong Kong, Shatin, N.T., Hong Kong;$^{(b)}$Department of Physics, University of Hong Kong, Hong Kong;$^{(c)}$Department of Physics and Institute for Advanced Study, Hong Kong University of Science and Technology, Clear Water Bay, Kowloon, Hong Kong; China.\\
$^{63}$Department of Physics, National Tsing Hua University, Hsinchu; Taiwan.\\
$^{64}$IJCLab, Universit\'e Paris-Saclay, CNRS/IN2P3, 91405, Orsay; France.\\
$^{65}$Department of Physics, Indiana University, Bloomington IN; United States of America.\\
$^{66}$$^{(a)}$INFN Gruppo Collegato di Udine, Sezione di Trieste, Udine;$^{(b)}$ICTP, Trieste;$^{(c)}$Dipartimento Politecnico di Ingegneria e Architettura, Universit\`a di Udine, Udine; Italy.\\
$^{67}$$^{(a)}$INFN Sezione di Lecce;$^{(b)}$Dipartimento di Matematica e Fisica, Universit\`a del Salento, Lecce; Italy.\\
$^{68}$$^{(a)}$INFN Sezione di Milano;$^{(b)}$Dipartimento di Fisica, Universit\`a di Milano, Milano; Italy.\\
$^{69}$$^{(a)}$INFN Sezione di Napoli;$^{(b)}$Dipartimento di Fisica, Universit\`a di Napoli, Napoli; Italy.\\
$^{70}$$^{(a)}$INFN Sezione di Pavia;$^{(b)}$Dipartimento di Fisica, Universit\`a di Pavia, Pavia; Italy.\\
$^{71}$$^{(a)}$INFN Sezione di Pisa;$^{(b)}$Dipartimento di Fisica E. Fermi, Universit\`a di Pisa, Pisa; Italy.\\
$^{72}$$^{(a)}$INFN Sezione di Roma;$^{(b)}$Dipartimento di Fisica, Sapienza Universit\`a di Roma, Roma; Italy.\\
$^{73}$$^{(a)}$INFN Sezione di Roma Tor Vergata;$^{(b)}$Dipartimento di Fisica, Universit\`a di Roma Tor Vergata, Roma; Italy.\\
$^{74}$$^{(a)}$INFN Sezione di Roma Tre;$^{(b)}$Dipartimento di Matematica e Fisica, Universit\`a Roma Tre, Roma; Italy.\\
$^{75}$$^{(a)}$INFN-TIFPA;$^{(b)}$Universit\`a degli Studi di Trento, Trento; Italy.\\
$^{76}$Institut f\"{u}r Astro-~und Teilchenphysik, Leopold-Franzens-Universit\"{a}t, Innsbruck; Austria.\\
$^{77}$University of Iowa, Iowa City IA; United States of America.\\
$^{78}$Department of Physics and Astronomy, Iowa State University, Ames IA; United States of America.\\
$^{79}$Joint Institute for Nuclear Research, Dubna; Russia.\\
$^{80}$$^{(a)}$Departamento de Engenharia El\'etrica, Universidade Federal de Juiz de Fora (UFJF), Juiz de Fora;$^{(b)}$Universidade Federal do Rio De Janeiro COPPE/EE/IF, Rio de Janeiro;$^{(c)}$Universidade Federal de S\~ao Jo\~ao del Rei (UFSJ), S\~ao Jo\~ao del Rei;$^{(d)}$Instituto de F\'isica, Universidade de S\~ao Paulo, S\~ao Paulo; Brazil.\\
$^{81}$KEK, High Energy Accelerator Research Organization, Tsukuba; Japan.\\
$^{82}$Graduate School of Science, Kobe University, Kobe; Japan.\\
$^{83}$$^{(a)}$AGH University of Science and Technology, Faculty of Physics and Applied Computer Science, Krakow;$^{(b)}$Marian Smoluchowski Institute of Physics, Jagiellonian University, Krakow; Poland.\\
$^{84}$Institute of Nuclear Physics Polish Academy of Sciences, Krakow; Poland.\\
$^{85}$Faculty of Science, Kyoto University, Kyoto; Japan.\\
$^{86}$Kyoto University of Education, Kyoto; Japan.\\
$^{87}$Research Center for Advanced Particle Physics and Department of Physics, Kyushu University, Fukuoka ; Japan.\\
$^{88}$Instituto de F\'{i}sica La Plata, Universidad Nacional de La Plata and CONICET, La Plata; Argentina.\\
$^{89}$Physics Department, Lancaster University, Lancaster; United Kingdom.\\
$^{90}$Oliver Lodge Laboratory, University of Liverpool, Liverpool; United Kingdom.\\
$^{91}$Department of Experimental Particle Physics, Jo\v{z}ef Stefan Institute and Department of Physics, University of Ljubljana, Ljubljana; Slovenia.\\
$^{92}$School of Physics and Astronomy, Queen Mary University of London, London; United Kingdom.\\
$^{93}$Department of Physics, Royal Holloway University of London, Egham; United Kingdom.\\
$^{94}$Department of Physics and Astronomy, University College London, London; United Kingdom.\\
$^{95}$Louisiana Tech University, Ruston LA; United States of America.\\
$^{96}$Fysiska institutionen, Lunds universitet, Lund; Sweden.\\
$^{97}$Centre de Calcul de l'Institut National de Physique Nucl\'eaire et de Physique des Particules (IN2P3), Villeurbanne; France.\\
$^{98}$Departamento de F\'isica Teorica C-15 and CIAFF, Universidad Aut\'onoma de Madrid, Madrid; Spain.\\
$^{99}$Institut f\"{u}r Physik, Universit\"{a}t Mainz, Mainz; Germany.\\
$^{100}$School of Physics and Astronomy, University of Manchester, Manchester; United Kingdom.\\
$^{101}$CPPM, Aix-Marseille Universit\'e, CNRS/IN2P3, Marseille; France.\\
$^{102}$Department of Physics, University of Massachusetts, Amherst MA; United States of America.\\
$^{103}$Department of Physics, McGill University, Montreal QC; Canada.\\
$^{104}$School of Physics, University of Melbourne, Victoria; Australia.\\
$^{105}$Department of Physics, University of Michigan, Ann Arbor MI; United States of America.\\
$^{106}$Department of Physics and Astronomy, Michigan State University, East Lansing MI; United States of America.\\
$^{107}$B.I. Stepanov Institute of Physics, National Academy of Sciences of Belarus, Minsk; Belarus.\\
$^{108}$Research Institute for Nuclear Problems of Byelorussian State University, Minsk; Belarus.\\
$^{109}$Group of Particle Physics, University of Montreal, Montreal QC; Canada.\\
$^{110}$P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow; Russia.\\
$^{111}$National Research Nuclear University MEPhI, Moscow; Russia.\\
$^{112}$D.V. Skobeltsyn Institute of Nuclear Physics, M.V. Lomonosov Moscow State University, Moscow; Russia.\\
$^{113}$Fakult\"at f\"ur Physik, Ludwig-Maximilians-Universit\"at M\"unchen, M\"unchen; Germany.\\
$^{114}$Max-Planck-Institut f\"ur Physik (Werner-Heisenberg-Institut), M\"unchen; Germany.\\
$^{115}$Nagasaki Institute of Applied Science, Nagasaki; Japan.\\
$^{116}$Graduate School of Science and Kobayashi-Maskawa Institute, Nagoya University, Nagoya; Japan.\\
$^{117}$Department of Physics and Astronomy, University of New Mexico, Albuquerque NM; United States of America.\\
$^{118}$Institute for Mathematics, Astrophysics and Particle Physics, Radboud University Nijmegen/Nikhef, Nijmegen; Netherlands.\\
$^{119}$Nikhef National Institute for Subatomic Physics and University of Amsterdam, Amsterdam; Netherlands.\\
$^{120}$Department of Physics, Northern Illinois University, DeKalb IL; United States of America.\\
$^{121}$$^{(a)}$Budker Institute of Nuclear Physics and NSU, SB RAS, Novosibirsk;$^{(b)}$Novosibirsk State University Novosibirsk; Russia.\\
$^{122}$Institute for High Energy Physics of the National Research Centre Kurchatov Institute, Protvino; Russia.\\
$^{123}$Institute for Theoretical and Experimental Physics named by A.I. Alikhanov of National Research Centre "Kurchatov Institute", Moscow; Russia.\\
$^{124}$Department of Physics, New York University, New York NY; United States of America.\\
$^{125}$Ochanomizu University, Otsuka, Bunkyo-ku, Tokyo; Japan.\\
$^{126}$Ohio State University, Columbus OH; United States of America.\\
$^{127}$Faculty of Science, Okayama University, Okayama; Japan.\\
$^{128}$Homer L. Dodge Department of Physics and Astronomy, University of Oklahoma, Norman OK; United States of America.\\
$^{129}$Department of Physics, Oklahoma State University, Stillwater OK; United States of America.\\
$^{130}$Palack\'y University, RCPTM, Joint Laboratory of Optics, Olomouc; Czech Republic.\\
$^{131}$Center for High Energy Physics, University of Oregon, Eugene OR; United States of America.\\
$^{132}$Graduate School of Science, Osaka University, Osaka; Japan.\\
$^{133}$Department of Physics, University of Oslo, Oslo; Norway.\\
$^{134}$Department of Physics, Oxford University, Oxford; United Kingdom.\\
$^{135}$LPNHE, Sorbonne Universit\'e, Universit\'e de Paris, CNRS/IN2P3, Paris; France.\\
$^{136}$Department of Physics, University of Pennsylvania, Philadelphia PA; United States of America.\\
$^{137}$Konstantinov Nuclear Physics Institute of National Research Centre "Kurchatov Institute", PNPI, St. Petersburg; Russia.\\
$^{138}$Department of Physics and Astronomy, University of Pittsburgh, Pittsburgh PA; United States of America.\\
$^{139}$$^{(a)}$Laborat\'orio de Instrumenta\c{c}\~ao e F\'isica Experimental de Part\'iculas - LIP, Lisboa;$^{(b)}$Departamento de F\'isica, Faculdade de Ci\^{e}ncias, Universidade de Lisboa, Lisboa;$^{(c)}$Departamento de F\'isica, Universidade de Coimbra, Coimbra;$^{(d)}$Centro de F\'isica Nuclear da Universidade de Lisboa, Lisboa;$^{(e)}$Departamento de F\'isica, Universidade do Minho, Braga;$^{(f)}$Departamento de Física Teórica y del Cosmos, Universidad de Granada, Granada (Spain);$^{(g)}$Dep F\'isica and CEFITEC of Faculdade de Ci\^{e}ncias e Tecnologia, Universidade Nova de Lisboa, Caparica;$^{(h)}$Instituto Superior T\'ecnico, Universidade de Lisboa, Lisboa; Portugal.\\
$^{140}$Institute of Physics of the Czech Academy of Sciences, Prague; Czech Republic.\\
$^{141}$Czech Technical University in Prague, Prague; Czech Republic.\\
$^{142}$Charles University, Faculty of Mathematics and Physics, Prague; Czech Republic.\\
$^{143}$Particle Physics Department, Rutherford Appleton Laboratory, Didcot; United Kingdom.\\
$^{144}$IRFU, CEA, Universit\'e Paris-Saclay, Gif-sur-Yvette; France.\\
$^{145}$Santa Cruz Institute for Particle Physics, University of California Santa Cruz, Santa Cruz CA; United States of America.\\
$^{146}$$^{(a)}$Departamento de F\'isica, Pontificia Universidad Cat\'olica de Chile, Santiago;$^{(b)}$Universidad Andres Bello, Department of Physics, Santiago;$^{(c)}$Departamento de F\'isica, Universidad T\'ecnica Federico Santa Mar\'ia, Valpara\'iso; Chile.\\
$^{147}$Department of Physics, University of Washington, Seattle WA; United States of America.\\
$^{148}$Department of Physics and Astronomy, University of Sheffield, Sheffield; United Kingdom.\\
$^{149}$Department of Physics, Shinshu University, Nagano; Japan.\\
$^{150}$Department Physik, Universit\"{a}t Siegen, Siegen; Germany.\\
$^{151}$Department of Physics, Simon Fraser University, Burnaby BC; Canada.\\
$^{152}$SLAC National Accelerator Laboratory, Stanford CA; United States of America.\\
$^{153}$Physics Department, Royal Institute of Technology, Stockholm; Sweden.\\
$^{154}$Departments of Physics and Astronomy, Stony Brook University, Stony Brook NY; United States of America.\\
$^{155}$Department of Physics and Astronomy, University of Sussex, Brighton; United Kingdom.\\
$^{156}$School of Physics, University of Sydney, Sydney; Australia.\\
$^{157}$Institute of Physics, Academia Sinica, Taipei; Taiwan.\\
$^{158}$Academia Sinica Grid Computing, Institute of Physics, Academia Sinica, Taipei; Taiwan.\\
$^{159}$$^{(a)}$E. Andronikashvili Institute of Physics, Iv. Javakhishvili Tbilisi State University, Tbilisi;$^{(b)}$High Energy Physics Institute, Tbilisi State University, Tbilisi; Georgia.\\
$^{160}$Department of Physics, Technion, Israel Institute of Technology, Haifa; Israel.\\
$^{161}$Raymond and Beverly Sackler School of Physics and Astronomy, Tel Aviv University, Tel Aviv; Israel.\\
$^{162}$Department of Physics, Aristotle University of Thessaloniki, Thessaloniki; Greece.\\
$^{163}$International Center for Elementary Particle Physics and Department of Physics, University of Tokyo, Tokyo; Japan.\\
$^{164}$Graduate School of Science and Technology, Tokyo Metropolitan University, Tokyo; Japan.\\
$^{165}$Department of Physics, Tokyo Institute of Technology, Tokyo; Japan.\\
$^{166}$Tomsk State University, Tomsk; Russia.\\
$^{167}$Department of Physics, University of Toronto, Toronto ON; Canada.\\
$^{168}$$^{(a)}$TRIUMF, Vancouver BC;$^{(b)}$Department of Physics and Astronomy, York University, Toronto ON; Canada.\\
$^{169}$Division of Physics and Tomonaga Center for the History of the Universe, Faculty of Pure and Applied Sciences, University of Tsukuba, Tsukuba; Japan.\\
$^{170}$Department of Physics and Astronomy, Tufts University, Medford MA; United States of America.\\
$^{171}$Department of Physics and Astronomy, University of California Irvine, Irvine CA; United States of America.\\
$^{172}$Department of Physics and Astronomy, University of Uppsala, Uppsala; Sweden.\\
$^{173}$Department of Physics, University of Illinois, Urbana IL; United States of America.\\
$^{174}$Instituto de F\'isica Corpuscular (IFIC), Centro Mixto Universidad de Valencia - CSIC, Valencia; Spain.\\
$^{175}$Department of Physics, University of British Columbia, Vancouver BC; Canada.\\
$^{176}$Department of Physics and Astronomy, University of Victoria, Victoria BC; Canada.\\
$^{177}$Fakult\"at f\"ur Physik und Astronomie, Julius-Maximilians-Universit\"at W\"urzburg, W\"urzburg; Germany.\\
$^{178}$Department of Physics, University of Warwick, Coventry; United Kingdom.\\
$^{179}$Waseda University, Tokyo; Japan.\\
$^{180}$Department of Particle Physics, Weizmann Institute of Science, Rehovot; Israel.\\
$^{181}$Department of Physics, University of Wisconsin, Madison WI; United States of America.\\
$^{182}$Fakult{\"a}t f{\"u}r Mathematik und Naturwissenschaften, Fachgruppe Physik, Bergische Universit\"{a}t Wuppertal, Wuppertal; Germany.\\
$^{183}$Department of Physics, Yale University, New Haven CT; United States of America.\\
$^{184}$Yerevan Physics Institute, Yerevan; Armenia.\\

$^{a}$ Also at Borough of Manhattan Community College, City University of New York, New York NY; United States of America.\\
$^{b}$ Also at Centre for High Performance Computing, CSIR Campus, Rosebank, Cape Town; South Africa.\\
$^{c}$ Also at CERN, Geneva; Switzerland.\\
$^{d}$ Also at CPPM, Aix-Marseille Universit\'e, CNRS/IN2P3, Marseille; France.\\
$^{e}$ Also at D\'epartement de Physique Nucl\'eaire et Corpusculaire, Universit\'e de Gen\`eve, Gen\`eve; Switzerland.\\
$^{f}$ Also at Departament de Fisica de la Universitat Autonoma de Barcelona, Barcelona; Spain.\\
$^{g}$ Also at Departamento de Física Teórica y del Cosmos, Universidad de Granada, Granada (Spain); Spain.\\
$^{h}$ Also at Department of Applied Physics and Astronomy, University of Sharjah, Sharjah; United Arab Emirates.\\
$^{i}$ Also at Department of Financial and Management Engineering, University of the Aegean, Chios; Greece.\\
$^{j}$ Also at Department of Physics and Astronomy, University of Louisville, Louisville, KY; United States of America.\\
$^{k}$ Also at Department of Physics and Astronomy, University of Sheffield, Sheffield; United Kingdom.\\
$^{l}$ Also at Department of Physics, Ben Gurion University of the Negev, Beer Sheva; Israel.\\
$^{m}$ Also at Department of Physics, California State University, East Bay; United States of America.\\
$^{n}$ Also at Department of Physics, California State University, Fresno; United States of America.\\
$^{o}$ Also at Department of Physics, California State University, Sacramento; United States of America.\\
$^{p}$ Also at Department of Physics, King's College London, London; United Kingdom.\\
$^{q}$ Also at Department of Physics, Nanjing University, Nanjing; China.\\
$^{r}$ Also at Department of Physics, St. Petersburg State Polytechnical University, St. Petersburg; Russia.\\
$^{s}$ Also at Department of Physics, University of Fribourg, Fribourg; Switzerland.\\
$^{t}$ Also at Department of Physics, University of Michigan, Ann Arbor MI; United States of America.\\
$^{u}$ Also at Dipartimento di Fisica E. Fermi, Universit\`a di Pisa, Pisa; Italy.\\
$^{v}$ Also at Faculty of Physics, M.V. Lomonosov Moscow State University, Moscow; Russia.\\
$^{w}$ Also at Giresun University, Faculty of Engineering, Giresun; Turkey.\\
$^{x}$ Also at Graduate School of Science, Osaka University, Osaka; Japan.\\
$^{y}$ Also at Hellenic Open University, Patras; Greece.\\
$^{z}$ Also at Horia Hulubei National Institute of Physics and Nuclear Engineering, Bucharest; Romania.\\
$^{aa}$ Also at II. Physikalisches Institut, Georg-August-Universit\"{a}t G\"ottingen, G\"ottingen; Germany.\\
$^{ab}$ Also at IJCLab, Universit\'e Paris-Saclay, CNRS/IN2P3, 91405, Orsay; France.\\
$^{ac}$ Also at Institucio Catalana de Recerca i Estudis Avancats, ICREA, Barcelona; Spain.\\
$^{ad}$ Also at Institut de F\'isica d'Altes Energies (IFAE), Barcelona Institute of Science and Technology, Barcelona; Spain.\\
$^{ae}$ Also at Institute for Mathematics, Astrophysics and Particle Physics, Radboud University Nijmegen/Nikhef, Nijmegen; Netherlands.\\
$^{af}$ Also at Institute for Particle and Nuclear Physics, Wigner Research Centre for Physics, Budapest; Hungary.\\
$^{ag}$ Also at Institute of Particle Physics (IPP), Vancouver; Canada.\\
$^{ah}$ Also at Institute of Physics, Academia Sinica, Taipei; Taiwan.\\
$^{ai}$ Also at Institute of Physics, Azerbaijan Academy of Sciences, Baku; Azerbaijan.\\
$^{aj}$ Also at Institute of Theoretical Physics, Ilia State University, Tbilisi; Georgia.\\
$^{ak}$ Also at Louisiana Tech University, Ruston LA; United States of America.\\
$^{al}$ Also at LPNHE, Sorbonne Universit\'e, Universit\'e de Paris, CNRS/IN2P3, Paris; France.\\
$^{am}$ Also at Manhattan College, New York NY; United States of America.\\
$^{an}$ Also at Moscow Institute of Physics and Technology State University, Dolgoprudny; Russia.\\
$^{ao}$ Also at National Research Nuclear University MEPhI, Moscow; Russia.\\
$^{ap}$ Also at Near East University, Nicosia, North Cyprus, Mersin; Turkey.\\
$^{aq}$ Also at Ochadai Academic Production, Ochanomizu University, Tokyo; Japan.\\
$^{ar}$ Also at Physics Department, An-Najah National University, Nablus; Palestine.\\
$^{as}$ Also at Physikalisches Institut, Albert-Ludwigs-Universit\"{a}t Freiburg, Freiburg; Germany.\\
$^{at}$ Also at School of Physics, Sun Yat-sen University, Guangzhou; China.\\
$^{au}$ Also at The City College of New York, New York NY; United States of America.\\
$^{av}$ Also at The Collaborative Innovation Center of Quantum Matter (CICQM), Beijing; China.\\
$^{aw}$ Also at Tomsk State University, Tomsk, and Moscow Institute of Physics and Technology State University, Dolgoprudny; Russia.\\
$^{ax}$ Also at TRIUMF, Vancouver BC; Canada.\\
$^{ay}$ Also at Universita di Napoli Parthenope, Napoli; Italy.\\
$^{*}$ Deceased

\end{flushleft}

% Created with Glance <Atlas.Glance@cern.ch>

